COMPASS: A Unified Decision-Intelligence System for Navigating Performance Trade-off in HPC

HPC systems expose many configuration parameters that jointly drive competing objectives. Existing tools such as autotuners recommend good configurations but do not identify minimal changes for a near-miss configuration to meet a performance objective, and they often ignore domain-specific constraints. To address this gap, we introduce COMPASS -- a modular, programmable engine that uses operational traces to generate HPC configuration recommendations and guide tuning decisions. This paper: (1) formalizes configuration questions into query patterns; (2) develops an interactive decision-making engine that formulates these queries as Machine Learning (ML) tasks; (3) quantifies the trustworthiness of its recommendations by providing evidence and quantifying uncertainty, and -- when confidence is low -- provides guidance on which configurations to run next. We validate COMPASS using analytical ground truth, reconstruction accuracy, reproduction of published findings, and when possible, running on real hardware. When integrated with an open-source HPC scheduling simulator, COMPASS cuts average job turnaround time by 65.93% and node usage by 80.93% relative to the state-of-the-art. Moreover, COMPASS achieves up to 100x faster training and 80x faster inference than state-of-the-art generative methods, and scales to traces with 1.3B samples and 126GB of data.

==> Sections/RQ_50_papers.tex <==
A Comprehensive Analysis of Process Energy
Consumption on Multi-Socket Systems with
GPUs

1) Recommend a process configuration that minimizes energy consumption while ensuring completion in under 500 seconds on the dual-socket AMD EPYC CPU system.

2) "Given a baseline where a GPU matrix multiplication job uses standard CUDA cores, how should I change the implementation to achieve a 10\% reduction in GPU card power consumption?"

3) "Given a baseline configuration with 32 threads executing vector arithmetic, what would be the impact on power consumption if I increase the thread count to 64?"

4) "If I switch the memory operations from scalar to vector instructions for a process currently using 50\% of CPU cores, how much would the CPU power consumption change?"


===========


Extracting Practical, Actionable Energy Insights from
Supercomputer Telemetry and Logs

5) If a job on Polaris accelerates its GPU memory utilization from 10\% to 30\% of runtime, how will this likely affect its instantaneous power consumption?

6) How much idle GPU power could be saved if software-controlled P-states were enabled, given that the average job uses only a quarter of available GPU power and 50\% of draw is idle?

7) What is the impact on total node energy if the number of allocated GPUs per job is increased from 1 to 4?



========

Fresco: A Public Multi-Institutional Dataset for Understanding HPC System Behavior and Dependability

8) Based on historical runs, which resource allocation (CPU, memory, GPU) is recommended for training workloads to achieve the shortest job completion time on Stampede

9) Recommend an optimal node configuration to minimize the failure rate for long-duration jobs on the Anvil cluster

10) What if I double the walltime request for given jobs on Stampede, what change should I expect in their overall completion rate?

11) If my goal is to reduce instantaneous power consumption by 20\% for GPU-based tasks on Anvil, which resource or scheduling parameter should we optimize?



“A Comprehensive Analysis of Process Energy Consumption on Multi‑…” – mathematical models predicting CPU & GPU power & energy consumption per process (1.9\% CPU error, 9.7% GPU) 
Department of Computer Science
+3
atlarge-research.com
+3
Boston University
+3
arXiv

[arXiv link]
EfiMon: A Process Analyser for Granular Power Consumption – regression-based tool estimating per-process energy in shared environments (2.2–4.4% error) 
arXiv

[arXiv link]
Power-Aware Scheduling for Multi-Center HPC Electric Cost – uses GNNs to predict per-job power across clusters, integrated with scheduling framework, evaluated on PM100 dataset 
Wikipedia
+5
arXiv
+5
arXiv
+5

[arXiv link]
Extracting Practical, Actionable Energy Insights from Supercomputer… – GPU telemetry + scheduler logs from Polaris system, dataset linking workload behavior to power 
arXiv
+1
arXiv
+1

[arXiv link]
Measuring the Energy Consumption and Efficiency of DNN Training – introduces the BUTTER‑E dataset: 63 k runs, 30 k configurations of neural nets with watt-meter readings 
arXiv

[arXiv link]
Prediction of Performance and Power Consumption of GPGPU Applications – static-analysis ML models predicting GPU kernel power & runtime; datasets from PTX code 
arXiv
+1
Wikipedia
+1

[arXiv link]
Understanding Energy Consumption of HPC-Scale AI – benchmark‑tracker tool for measuring energy/time of DL workloads; includes dataset & tools 
arXiv

[arXiv link]
�� Runtime/Performance & Energy Trends
Energy Efficiency Trends in HPC – survey + data-driven insights on hardware, scheduling, power management 
arXiv
+2
arXiv
+2
arXiv
+2

[arXiv link]
Maximizing Energy Efficiency of HPC Workloads with FaaS (GreenFaaS) – synthetic workload energy/runtime dataset showing 45 % energy-delay reduction
arXiv
+9
arXiv
+9
arXiv
+9

[arXiv link]
Precise Energy Consumption Measurements of Heterogeneous AI Workloads – evaluation of node-level energy usage (multi‑node GPU/CPU) 
arXiv
+1
Department of Computer Science
+1

[arXiv link]
�� Anomaly & Performance-State Classification
Runtime Performance Anomaly Diagnosis in Production HPC – active-learning classification framework diagnosing anomaly types at runtime (F1 ≈ 0.82)
arXiv
+2
Boston University
+2
emreates.github.io
+2

[PDF]
RUAD: Unsupervised Anomaly Detection in HPC – time-series LSTM model on Marconi100 logs, AUC ≈ 0.77 
arXiv
+1
ScienceDirect
+1

[arXiv link]
Data Characterization and Anomaly Detection for HPC Datacenters – PROMETHEUS dataset from 343 nodes with node-/GPU- level telemetry
atlarge-research.com

[PDF]
Anomaly Detection and Anticipation in HPC Systems – model to classify node states using labeled supercomputer data 
ResearchGate
Diagnosing Performance Variations in HPC Applications – statistical-feature classifier (kNN, RF) for performance anomalies (OS jitter, memory leaks, etc.)
emreates.github.io
+1
Boston University
+1
Unsupervised KPIs‑Based Clustering of Jobs in HPC Data Centers – clusters jobs based on KPIs to identify behavior classes (unsupervised) 
arXiv
Modeling HPC System Log Messages for Early Job State Prediction – log-based classification of job outcomes (failed/completed) 
Department of Computer Science
+1
arXiv
+1
�� Workload Classification & Benchmarks
MIT Supercloud Workload Classification Challenge – CPU/GPU job logs designed for classification challenge 
arXiv
+1
Department of Computer Science
+1
HPC AI500: Benchmark Suite for Scientific DL Workloads – includes performance, accuracy, power & cost metrics across 14 DL benchmarks 
arXiv
+1
arXiv
+1
�� Benchmarks & Tools (with public data)
A Job Power Consumption Dataset of a Large‑scale Production System (ACM) – ~230 K jobs with power consumption records 
dl.acm.org


==> Sections/RQ_list.tex <==
// For each dataset, make note of (1) the features they dropped (2) features they used (3) Target columns (4) What metric did they use to demonstrate that they are the best? We have to beat them at that metric.

For example we have a sample where the number of gpus are 4 , power consumption is 500

1) what is the power consumption if we double the number of gpus.

2) 
Modify X = {num_gpus: 4 -> ?} to achieve Y = {power: 500W -> 450W}

what-if we change X = { num gpus :  4-> 8}, how would that affect Y = {power: ?}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
PM-100:
[Done]
X = cores_per_task, num_cores_req, num_nodes_req, num_gpus_req, mem_req, time_limit
Y = run_time, node_power_consumption, cpu_power_consumption, mem_power_consumption, job_state, 
Recommendation for a user: should not include partition.

% >>> df["job_state"].unique()
% array(['CANCELLED', 'FAILED', 'COMPLETED', 'TIMEOUT', 'OUT_OF_MEMORY',
%        'NODE_FAIL'], dtype=object)

1. \textcolor{blue}{Recommend a configuration where}
X = [cores_per_task: ?, num_cores_req: ?, num_nodes_req: ?, num_gpus_req: ?, time_limit: ?, num_gpus: 4] %Meaning, only these features need to be recommended.
\textcolor{blue}{to achieve}
Y = [run_time: minimum, cpu_power_consumption: minimum, job_state: completed]
%Multi-objective optimization -- find a stisficing one that is neither minimum for runtime not for cpu. but good for both.

2. Discover what impacts 
Y = [runtime, node_poower_consumption, cpu_power_consumption].

3. Modify X = {} to achieve
Y = {} such that x_i changes minimally.

4. What-if we change 
X_cond = {}, how would that affect
Y = {} such that the rest of the features not mentioned changes minimally.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Fugaku:
1. Recommend a configuration where 
X =  ['cnumr': 64, 'nnumr': 1, 'mszl':?, 'freq_req':?, 'jobenv_req':?]
to achieve
Y = [econ: optimal, job_state: completed]

2. Discover what impacts 
\(Y = [\text{econ}, \text{duration}] \)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% 3. What if we change the configuration X = [num_task: 122 → 128, allreduce_size: 5M → 6.4M], how would that affect Y = [runtime]? 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


SC'19 dataset:
1. Recommend a configuration where 
X = [app: CoMD]
to achieve
Y = [perf_variation: minimum]


% NOTE: Recommend a configuration for application=FT (check in the SC'19 paper which one had the 4x variation) to achieve the minimum ``abs\_variation" (You will need to calculate the abs\_variation column for that dataset)
% -- average for every application, and then difference between that application's samples and that that_application's_average_value value.

2. Discover what impacts 
Y = [perf_variation].


3. What if we change the configuration X = [num\_task: 122 → 128, power\_cap: 115W → 82W], how would that affect Y = [runtime]?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

DATASET: Monet dataset from the Blue Waters
% X = [
%     "Time",
%     "Z-_SAMPLE_GEMINI_LINK_CREDIT_STALL (% x1e6)",
%     "Z+_SAMPLE_GEMINI_LINK_CREDIT_STALL (% x1e6)",
%     "Y-_SAMPLE_GEMINI_LINK_CREDIT_STALL (% x1e6)",
%     "Y+_SAMPLE_GEMINI_LINK_CREDIT_STALL (% x1e6)",
%     "X-_SAMPLE_GEMINI_LINK_CREDIT_STALL (% x1e6)",
%     "X+_SAMPLE_GEMINI_LINK_CREDIT_STALL (% x1e6)",
%     "Z-_SAMPLE_GEMINI_LINK_INQ_STALL (% x1e6)",
%     "Z+_SAMPLE_GEMINI_LINK_INQ_STALL (% x1e6)",
%     "Y-_SAMPLE_GEMINI_LINK_INQ_STALL (% x1e6)",
%     "Y+_SAMPLE_GEMINI_LINK_INQ_STALL (% x1e6)",
%     "X-_SAMPLE_GEMINI_LINK_INQ_STALL (% x1e6)",
%     "X+_SAMPLE_GEMINI_LINK_INQ_STALL (% x1e6)",
%     "nettopo_mesh_coord_Z",
%     "nettopo_mesh_coord_Y",
%     "nettopo_mesh_coord_X"
% ]

% y = [
%     "Z-_SAMPLE_GEMINI_LINK_USED_BW (% x1e6)",
%     "Z+_SAMPLE_GEMINI_LINK_USED_BW (% x1e6)",
%     "Y-_SAMPLE_GEMINI_LINK_USED_BW (% x1e6)",
%     "Y+_SAMPLE_GEMINI_LINK_USED_BW (% x1e6)",
%     "X-_SAMPLE_GEMINI_LINK_USED_BW (% x1e6)",
%     "X+_SAMPLE_GEMINI_LINK_USED_BW (% x1e6)"
% ]
% # Column Description
% | Column Name                                  | Column Description                 |
% |----------------------------------------------|------------------------------------|
% | **#Time**                                        | *UNIX Epoch time* in seconds  |
% | ***dir*_SAMPLE_GEMINI_LINK_CREDIT_STALL (% x1e6)** | *Credit Stall* which can be defined as the stall time associated with sending flits between different switches.                    |
% | ***dir*_SAMPLE_GEMINI_LINK_INQ_STALL (% x1e6)**    | *Inq Stall* which can be defined as the stall time associated with sending flits within the same switch                         |
% | ***dir*_SAMPLE_GEMINI_LINK_USED_BW (% x1e6)**      | *Bandwidth Utilization* which is the percentage of maximum link bandwidth used during the measurement interval           |
% | **nettopo_mesh_coord_Z**                         | *Z coordinate* in the torus topology                    |
% | **nettopo_mesh_coord_Y**                         | *Y coordinate* in the torus topology                       |
% | **nettopo_mesh_coord_X**                         | *X coordinate* in the torus topology    
X = [nettopo_mesh_coord_X, nettopo_mesh_coord_Z, nettopo_mesh_coord_Y]

Y = [dirX+_SAMPLE_GEMINI_LINK_CREDIT_STALL = minimum, dirX+_SAMPLE_GEMINI_LINK_INQ_STALL = minimum, dirX+_SAMPLE_GEMINI_LINK_USED_BW =  minimum]


1. Recommend a configuration where 
X = [nettopo_mesh_coord_X, nettopo_mesh_coord_Z, nettopo_mesh_coord_Y]
to achieve
Y = [dirY+_SAMPLE_GEMINI_LINK_CREDIT_STALL = minimum]



2. Discover what impacts
Y = [dirX+_SAMPLE_GEMINI_LINK_CREDIT_STALL, dirX+_SAMPLE_GEMINI_LINK_INQ_STALL, dirX+_SAMPLE_GEMINI_LINK_USED_BW]

% Recommend me a configuration where X is [var: min\_initial\_value] and we have minimum bandwidth for Z direction.

% 1. Recommend a configuration where 
% X = [app: CoMD]
% to achieve
% Y = [abs\_variation: minimum]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Lassen Supercomputing dataset
1. Recommend a configuration where 
X = [region: 0, var: initial\_value]
to achieve
Y = [abs\_variation: minimum]

dataset details:
X = ['isolated_cores', 'num_nodes_x', 'num_processors_x', 'num_gpus_x', 'projected_memory_x', 'type', 'job_type', 'time_limit', 'smt_mode', 'core_blink', 'power_cap', 'power_shifting_ratio', 'num_nodes_y', 'num_processors_y', 'num_gpus_y', 'num_tasks', 'projected_memory_y', 'omp_thread_limit']
Y = ['energy', 'gpu_usage', 'gpfs_read', 'gpfs_write', 'total_s_time']
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DATASET: BUTTER-E: Department of Energy - BUTTER-E - Energy Consumption Data for the BUTTER Empirical Deep Learning Dataset:
[Done]
Recommendation for a user:  X = size, depth, shape, learning_rate, batch_size, optimizer, is_gpu; Y = energy, runtime, power, 

Things to drop: run_id, experiment_id, slurm_job_id, start_time, update_time, node, filter_1, filter_2, filter_3, filter_3_stdevs, filter, start_time_int, start_offset, num_reps, std_power, std_energy, energy_overhead, non_overhead_energy, runtime_overhead, non_overhead_runtime
Recommendation for a job scheduler: node %names of the nodes.

% Target Variable	Description
% energy	Total energy consumption per run
% run_time	Wall-clock duration of the run
% non_overhead_energy	Energy minus estimated idle/overhead energy
% non_overhead_runtime	Runtime minus estimated overhead
% std_power, std_energy	Variability measures that could serve as stability/efficiency targets

1a. Recommend a configuration where
X = [depth: ?, optimizer: ?, learning_rate: ?, batch_size: ?, dataset: 'mnist', is_gpu: True]
to achieve

% 1b. Recommend a configuration where
% X = [depth: ?, size: ?, dataset: 'connect4', is_gpu: True]
% to achieve
% Y = [run_time: minimum, job_state: 'completed']

% 1c. Recommend optimizer and batch size for stable energy profile
% Recommend a configuration where
% X = [optimizer: ?, batch_size: ?, dataset: 'splice', shape: 'rectangle']
% to achieve
% Y = [std_energy: minimum, job_state: 'completed']

2. Discover what impacts
Y = [energy, run_time, std_power, std_energy]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

1000-genome dataset
1. Recommend a configuration where 
X = [region: 0, var: inital\_value]
to achieve
Y = [abs\_variation: minimum]


PoSeiDon - Datasets
1. Recommend a configuration where 
X = [region: 0, var: inital\_value]
to achieve
Y = [abs\_variation: minimum]


MPI application phases https://zenodo.org/records/2635656
1. Recommend a configuration where 
X = [region: 0, var: inital\_value]
to achieve
Y = [abs\_variation: minimum]

% The dataset from Zenodo is designed to train machine learning models to predict the duration of computation or communication phases in MPI-based HPC applications.

% Each CSV file (e.g., adagio\_cmp\_1098432-512p.csv) corresponds to a specific application run and phase type (here, "cmp" for computation).

% Features typically include hardware counters, application-level metrics, and system state variables collected at the start of each phase. These may involve:

% CPU frequency

% Number of active cores

% Memory usage

% Cache statistics

% Application-specific parameters (e.g., process rank, phase ID)

% The target column is the duration of the current phase (computation or communication), measured in microseconds or milliseconds.

% No information from previous phases is used as input; all features are from the current phase only.

% The dataset supports supervised learning, where the model learns to map the features to the phase duration.

% Multiple files exist for different applications and runs, enabling generalization across workloads.

% The data structure is tabular, with each row representing a single phase instance.

% The main goal is to enable accurate, real-time prediction of phase duration for energy optimization in HPC systems.

% The dataset is directly linked to the methodology described in the COUNTDOWN Slack paper, focusing on phase-level prediction for power management.


I/O dataset: https://zenodo.org/records/1345780
1. Recommend a configuration where 
X = [region: 0, var: inital\_value]
to achieve
Y = [abs\_variation: minimum]



MPI dataset: https://zenodo.org/records/14812022
1. Recommend a configuration where 
X = [region: 0, var: inital\_value]
to achieve
Y = [abs\_variation: minimum]


HotCloudPerf'23 ML Job Failures Analysis:
1. Recommend a configuration where 
X = [region: 0, var: inital\_value]
to achieve
Y = [abs\_variation: minimum]

% We can use classification accuracy compared to use a standard XGBoost method?
% My synthesized data makes an XGBoost model more accurate? We are successful if an XGBoost/LightGBM/or any established model become more accurate if they use our synthesized data+original data OR only our synthesized data then they become more accurate or less UQ error.


GitHub - ACAT-SCUT/Awesome-CloudComputing-Datasets
1. Recommend a configuration where 
X = [region: 0, var: inital\_value]
to achieve
Y = [abs\_variation: minimum]


MIT supercomputing dataset
1. Recommend a configuration where 
X = [region: 0, var: inital\_value]
to achieve
Y = [abs\_variation: minimum]


https://portal.nersc.gov/cfs/m888/dcamps/hamlib/
1. Recommend a configuration where 
X = [region: 0, var: inital\_value]
to achieve
Y = [abs\_variation: minimum]

Google borg dataset  https://github.com/google/cluster-data
1. Recommend a configuration where 
X = [region: 0, var: inital\_value]
to achieve
Y = [abs\_variation: minimum]



==> Sections/background.tex <==
% \tzi{Describe counterfactual analysis and its mathematical formulation, DiCE and its math formulation, Recommendation and how it is different from counterfactual, and causal analysis. No more than 0.5 - 1 page.}
% 
% \subsection{Counterfactual analysis and explanation}

% Counterfactual reasoning addresses questions of the form ``What would the outcome have been if the value of a particular parameter had been set differently?" Formally, given an input configuration $x \in R^d$ and a predictive model 
% $f : R^d \rightarrow R^k$, the goal is to find a perturbed configuration $x'$ such that the model prediction changes in a desired way--e.g., achieving a target performance value $y^*$.

% % \vspace{0.2in} 
% \begin{equation*} 
% \eqnmarkbox[Green]{cf_instance}{\mathbf{x}'} = \arg\min_{\mathbf{x}'} \left[ \eqnmarkbox[WildStrawberry]{pred_loss}{\mathcal{L}_{\text{pred}}(f(\mathbf{x}'), \mathbf{y}^*)} + \lambda_1 \eqnmarkbox[YellowOrange]{distance}{\mathcal{L}_{\text{dist}}(\mathbf{x}, \mathbf{x}')} \right] \end{equation*} %\vspace{0.2in}
% \annotate[yshift=0.4em]{above,right}{cf_instance}{Counterfactual\\ configuration} \annotate[yshift=0.4em]{above,right}{pred_loss}{Loss measuring deviation\\ from target outcome} \annotate[yshift=-1.0em]{below,left}{distance}{Penalty for deviating\\ from original configuration}

% \noindent This formulation captures both counterfactual generation and explanation: it identifies minimal, plausible changes to the input that would yield the desired outcome. An extension to this formulation is the generation of diverse counterfactuals--multiple distinct configurations that satisfy the same target but reveal different pathways to improvement. This involves augmenting the objective with a diversity term:

% \vspace{0.2in} \begin{equation} \eqnmarkbox[Green]{cf_diverse_loss}{\mathcal{L}(\mathbf{x}, {\mathbf{x}'j})} = \lambda_1 \eqnmarkbox[WildStrawberry]{pred_term}{\mathcal{L}{\text{pred}}} + \lambda_2 \eqnmarkbox[OliveGreen]{dist_term}{\mathcal{L}{\text{dist}}} + \lambda_3 \eqnmarkbox[RoyalBlue]{div_term}{\mathcal{L}{\text{div}}} \label{eqn:counterfactual_diverse} \end{equation} \vspace{0.2in}

% \annotate[yshift=0.4em]{above,right}{cf_diverse_loss}{Loss for generating diverse counterfactuals} \annotate[yshift=0.4em]{above,right}{pred_term}{Ensures target performance is achieved} \annotate[yshift=0.4em]{above,right}{dist_term}{Maintains proximity to original} \annotate[yshift=0.4em]{above,right}{div_term}{Promotes diversity among candidates}

% \noindent Together, these formulations enable the system to explain why certain changes improve performance by identifying multiple valid and interpretable feasible alternatives within user-specified constraints.

% \subsection{Recommendation and Satisficing Optimization}

% \noindent In contrast to counterfactuals--where an initial desirable full or partial configuration is known, %and outcomes are explored—
% recommendation begins with a desired outcome and returns one or more feasible configurations that achieve it. The system searches over a constrained configuration space $\mathcal{C}$ for candidates that optimize one or more objectives.

% % \vspace{0.2in} 
% % \begin{equation*} 
% % \eqnmarkbox[Green]{recommended_config}{\mathbf{x}^} = \arg\min_{\mathbf{x}' \in \mathcal{C}} \eqnmarkbox[WildStrawberry]{multi_loss}{\mathcal{L}_{\text{multi}}(f(\mathbf{x}'), \mathbf{y}^)} \end{equation*}

% % \annotate[yshift=0.4em]{above,left}{recommended_config}{Recommended configuration} 
% % \annotate[yshift=0.4em]{above,right}{multi_loss}{Multi-objective loss (e.g., runtime, power)} 
% % \annotate[yshift=-0.4em]{below,left}{\mathcal{C}}{Feasible configuration space}

% \noindent If users provide constraints or thresholds across multiple performance metrics, the system formulates the query as a satisficing problem--identifying configurations that may not be globally optimal but lie within a trade-off region.

% \subsection{Conditional and Unconditional Generation}
% Recommender systems use a variety of techniques to predict user preferences and deliver personalized recommendations. These include Collaborative Filtering~\cite{schafer2007collaborative}, Matrix Factorization~\cite{koren2009matrix}, and more recently, Self-supervised Learning Models~\cite{yu2023self}. While effective, these methods rely heavily on user-specific historical data, which limits their generalization in data-scarce environments. Additionally, traditional approaches such as neighborhood-based collaborative filtering become computationally expensive when applied to heterogeneous data~\cite{chen2020efficient}.

% To address these challenges, generative models have emerged as a popular strategy for synthetic data generation~\cite{deldjoo2024recommendation}. By learning from available system metrics, these models can simulate realistic performance profiles, filling in missing data regions and improving generalization to unseen scenarios. Synthetic generation can take two forms: (1) Unconditional generation samples directly from the learned distribution of system configurations and performance outcomes, making it especially useful for new users with no historical data. (2) Conditional generation allows crafting synthetic samples based on prior knowledge to simulate what-if scenarios, enabling exploration of different performance trade-offs using existing datasets.
% % Synthesis is the more general operation where there is no masked quantity. And then say how conditional and unconditional generation maps to a range of use cases such as (1) recommendation for user with no experience (2) counterfactual generation for query-driven explanation and exploration for users who want to explore the parameter space, or auto-tuners, or educational tool for students and scientists who want to interactively explore and learn from telemetry data. 


\subsection{Structural Causal Modeling}
Structural Causal Models (SCMs)~\cite{bongers2021foundations} offer a rigorous mathematical framework for modeling cause-and-effect relationships, which enables robust reasoning about what-if scenarios. The models describe the relationships through various structural equations that link variables via directed causal pathways, providing a visual representation using Directed Acyclic Graphs (DAGs). This reasoning capability is crucial for the decision-making process to generate recommendations or what-if scenarios where causal relationships are more critical than correlation. For instance, user queries to a recommendation system--for example, a user investigates how increasing the number of compute nodes \texttt{num\_node} from a base configuration to a certain number might influence \texttt{node\_power\_consumption}. While observational data might suggest a correlation between \texttt{num\_node} and \texttt{node\_power\_consumption}, it cannot conclusively confirm whether the change in node count causes the observed change in power draw. %especially since other system-level factors such as job distribution and hardware heterogeneity may also play a role.

The observational data might show correlation between threads and execution time, but this alone can't confirm that only increasing the threads causes the speedup. In real-world HPC systems, speedup of a simulation depends on various other factors such as processor affinity and background system load. Leveraging the power of SCM, we can analyze the effect of changing the number of nodes by keeping other variables constant. This helps us in a crucial way; by visualizing the DAG generated by SCM, we can gain interpretable insights into how the other parameters such as \texttt{threads\_per\_core}, \texttt{memory\_bandwidth}, etc. can contribute to altering the target variables passively. Instead of relying on surface-level correlations only, such a structural discovery provides a transparent view of underlying mechanisms, supporting informed decision-making in \gls{hpc} configurations.
% Structural Causal Models(SCMs) ~\cite{bongers2021foundations} offer a rigorous mathematical framework for modeling cause-and-effect relationships, which enables robust reasoning about what-if scenarios. The models describe the relationships through various structural equations that link variables via directed causal pathways, providing a visual representation using Directed Acyclic Graph (DAG). This reasoning capability is crucial for the decision-making process to generate recommendations or what-if scenarios where causal relationships are more critical than correlation. For instance, user queries to a recommendation system - For instance, a user investigates how increasing the number of compute nodes \texttt{num\_node} from a base configuration to a certain number might influence \texttt{node\_power\_consumption}. While observational data might suggest a correlation between \texttt{num\_node} and \texttt{node\_power\_consumption}, it cannot conclusively confirm whether the change in node count causes the observed change in power draw—especially since other system-level factors such as job distribution and hardware heterogeneity may also play a role.. The observational data might show correlation between threads and execution time, but this alone can't confirm that only increasing the threads doesn't cause the speedup. In real-world HPC systems, speedup of a simulation depends on various other factors such as processor affinity and background system load. Leveraging the power of SCM, we can analyze the effect of changing the number of nodes by keeping other variables constant. This helps us in a crucial way; by visualizing the DAG generated by SCM, we can gain interpretable insights into how the other parameters such as \texttt{threads\_per\_core}, \texttt{memory\_bandwidth} etc. can contribute to altering the target variables passively. Instead of relying on surface-level correlations only, such a structural discovery provides a transparent view of underlying mechanisms, supporting informed decision-making in high performance computing (HPC) configurations.

% There are many ways to evaluate the quality of the recommendations and counterfactuals. Some common ways people have evaluated are by experimentation, or using the data to train predictive models and evaluating the predictive models' accuracy to solve downstream tasks, or designing distance measures to evaluate the distance between the distributions and subspace distance~\cite{banday2024perfgen}.


==> Sections/c3g_loss_equation.tex <==
\begin{figure*}[t]
% \centering
% \footnotesize
\tiny
\setlength{\tabcolsep}{35pt} % tighten column padding
% \renewcommand{\arraystretch}{1.15} % tighten row height (tune if needed)
\begin{tabular}{p{\textwidth}}
% -------------------- Row 1: Full-width master objective --------------------
% \centering
\begin{minipage}{\columnwidth}
% \centering
\begin{equation}
\label{eqn:c3g_cf_loss}
\eqnmarkbox[Green]{cf_loss}{
\{\mathbf{x}'_1,\ldots,\mathbf{x}'_N\}
}
=
\arg\min_{\{\mathbf{x}'_i \in \mathcal{X}_{\mathrm{valid}}\}}
\left[
\lambda_{\mathrm{valid}}\,
\eqnmarkbox[WildStrawberry]{validity}{
\mathcal{L}_{\mathrm{valid}}\!\big(\{\mathbf{x}'_i\},y^{\star},f_{\theta}\big)
}
+
\lambda_{\mathrm{prox}}\,
\eqnmarkbox[YellowOrange]{proximity}{
\sum_{i=1}^d \mathcal{L}_{\mathrm{prox}}(\mathbf{x}'_i,\mathbf{x})
}
+
\lambda_{\mathrm{cons}}\,
\eqnmarkbox[RoyalBlue]{cons}{
\sum_{i=1}^N \Phi(\mathbf{x}'_i)
}
-
\lambda_{\mathrm{div}}\,
\eqnmarkbox[Blue]{diversity}{
\mathcal{L}_{\mathrm{div}}\!\big(\{\mathbf{x}'_i\}\big)
}
\right].
\end{equation}

\annotate[yshift=0.9em]{above,right}{cf_loss}{Configuration set}
\annotate[yshift=-0.5em]{below,left}{validity}{Target satisfaction}
\annotate[yshift=0.4em]{above,left}{proximity}{Minimal change from \(\mathbf{x}\)}
\annotate[yshift=0.5em]{above,right}{cons}{Domain constraints}
\annotate[yshift=0.4em]{above,right}{diversity}{Distinct recourses}
\end{minipage}
% \\[0.5em]
\end{tabular}
% -------------------- Row 2: 4 side-by-side definitions --------------------
\footnotesize
\resizebox{\textwidth}{!}{
\begin{tabular}{p{0.3\textwidth} p{0.2\textwidth} p{0.2\textwidth} p{0.2\textwidth}}
\centering
\begin{minipage}{0.3\textwidth}
\centering
\begin{equation}
\label{eqn:valid-loss}
\mathcal{L}_{\mathrm{valid}}\!\big(\{\mathbf{x}'_i\},y^{\star},f_{\theta}\big)
=
\frac{1}{N}\sum_{i=1}^N
\Big[
\frac{(y_{\max} - y_{\min})}{2} - f_{\theta}(\mathbf{x}'_i\big)
\Big]
% +
% \Big[
% \big(f_{\theta}(\mathbf{x}'_i)-\epsilon\big) - y_{\max}
% \Big]_+ 
\end{equation}
\textbf{Validity}\\
\end{minipage}
&
\begin{minipage}{0.2\textwidth}
\centering
\begin{equation}
\label{eqn:prox-loss}
\mathcal{L}_{\mathrm{prox}}(\mathbf{x}'_i,\mathbf{x})
=
\sum_{j=1}^d w_j\,|x'_{i,j}-x_j|
\end{equation}
\textbf{Proximity}\\
\end{minipage}
&
\begin{minipage}{0.2\textwidth}
\centering
\begin{equation}
\label{eqn:cons-loss}
\Phi(\mathbf{x}'_i)
=
\sum_{k} \phi_k(\mathbf{x}'_i)
\end{equation}
\textbf{Constraints}\\
\end{minipage}
&
\begin{minipage}{0.2\textwidth}
\centering
\begin{equation}
\label{eqn:diversity-loss}
\mathcal{L}_{\mathrm{div}}\!\big(\{\mathbf{x}'_i\}\big)
=
\frac{2}{d(d-1)}
\sum_{1\le i<j\le d}
d_{\mathrm{CF}}(\mathbf{x}'_i,\mathbf{x}'_j)
\end{equation}
\textbf{Diversity}\\
\end{minipage}
\\
\end{tabular}
}
% \vspace{-0.5em}
\caption{Unified \(C^3G\) objective (top) and explicit definitions of each loss component (bottom).}
\label{fig:c3g_objective}
% \vspace{-0.8em}
\end{figure*}


==> Sections/c3g_unification_proof.tex <==
% ============================================================
%  C3G Query-Type Unification  —  drop-in subsection for SC paper
%  Citation keys: wachter2017, mothilal2020, verma2020, gupta2024gfi,
%                 korikov2021, korikov2021ijcai
%  Adjust \proposition / \proofsketch macros to match your theorem env.
% ============================================================

% --- Suggested macro definitions (add to preamble if not already present) ---
% \newtheorem{proposition}{Proposition}[section]
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{remark}{Remark}[section]
% \newcommand{\proofsketch}{\noindent\textit{Proof sketch.}\;}
% ----------------------------------------------------------------------------

\subsection{Formal Reduction of Query Types to a Common Optimization Problem}
\label{sec:c3g-unification}

We now formalize the sense in which the C3G loss unifies the three COMPASS
query types, making the relationship to forward and inverse problems precise.
The purpose of this subsection is not to claim novelty—counterfactual
optimization as an inverse problem is well established
\cite{wachter2018counterfactual,mothilal2020,korikov2021}—but to verify that the
\emph{same} parameterized problem subsumes all three query modes, so that the
single implementation presented in Section~\ref{sec:implementation} is
architecturally sufficient.

\paragraph{General problem statement.}
Let $f:\mathcal{X}\!\to\!\mathcal{Y}$ be a frozen surrogate, let
$\mathbf{x}_0\!\in\!\mathcal{X}$ be an initialization point, let
$[y_{\min},y_{\max}]\subset\mathcal{Y}$ with slack $\epsilon\!\ge\!0$ define a
target range $y^{\star}$, let $\mathcal{C}$ be a feasible set encoding domain
and equality constraints, and let
$\boldsymbol{\lambda}=(\lambda_{\mathrm{prox}},\lambda_{\mathrm{cons}},\lambda_{\mathrm{div}})\in\mathbb{R}_{\ge0}^{3}$.
Define the \emph{C3G problem}

\begin{equation}
  P(\mathbf{x}_0,\,y^{\star},\,\mathcal{C},\,\boldsymbol{\lambda})
  \;=\;
  \argmin_{\{\mathbf{x}'_i\}\,\subseteq\,\mathcal{X}_{\mathrm{valid}}\cap\mathcal{C}}
  \Bigl[
    \mathcal{L}_{\mathrm{valid}}(\{\mathbf{x}'_i\},y^{\star},f)
    +\lambda_{\mathrm{prox}}\!\sum_{i=1}^{N}\|\mathbf{x}'_i-\mathbf{x}_0\|_1
    +\lambda_{\mathrm{cons}}\!\sum_{i=1}^{N}\Phi(\mathbf{x}'_i)
    -\lambda_{\mathrm{div}}\,\mathcal{L}_{\mathrm{div}}(\{\mathbf{x}'_i\})
  \Bigr],
  \label{eq:c3g-general}
\end{equation}

\noindent where $\mathcal{L}_{\mathrm{valid}}$ is the hinge-based range validity
loss (zero when $f(\mathbf{x}'_i)\in[y_{\min}-\epsilon,\,y_{\max}+\epsilon]$),
$\Phi$ aggregates domain-constraint violation penalties, and
$\mathcal{L}_{\mathrm{div}}$ is the pairwise diversity reward.
Let $\mathcal{C}_{\mathrm{dom}}$ denote the base domain feasibility set, and
for an index set $S\!\subseteq\![d]$ with prescribed values
$\{v_j\}_{j\in S}$ write
$\mathcal{C}_{S}=\mathcal{C}_{\mathrm{dom}}\cap\{x'_j=v_j:j\in S\}$.

\begin{proposition}[Recommend as $P$]
\label{prop:recommend}
The \emph{recommend} query with target $y^{\star}$ is the instance
$P(\mathbf{x}_0,\,y^{\star},\,\mathcal{C}_{\mathrm{dom}},\,\boldsymbol{\lambda})$
where $\mathbf{x}_0\sim p_{\mathrm{filt}}(\mathcal{D})$ (sampled uniformly
from training configurations that satisfy $\mathcal{C}_{\mathrm{dom}}$) and
$\lambda_{\mathrm{prox}}=\lambda^{\mathrm{rec}}_{\mathrm{prox}}\approx 0$.
\end{proposition}

\proofsketch
Because $\lambda_{\mathrm{prox}}$ is negligibly small, the proximity term
exerts negligible regularisation; the optimizer is free to traverse
$\mathcal{X}_{\mathrm{valid}}$ guided almost entirely by
$\mathcal{L}_{\mathrm{valid}}$.  The result is therefore governed by the
equation $f(\mathbf{x}'_i)\approx y^{\star}$, which is precisely an
\emph{inverse problem}: given target output, recover a compatible input
\cite{gupta2024gfi,wachter2018counterfactual}.  The diversity term
$\mathcal{L}_{\mathrm{div}}$ spreads the $N$ solutions across
$\mathcal{X}$, directly extending the DiCE formulation of \cite{mothilal2020}
to a range-valued target.\hfill$\square$

\begin{proposition}[Reconfigure as $P$]
\label{prop:reconfigure}
The \emph{reconfigure} query for a user-provided baseline
$\mathbf{x}_{\mathrm{user}}$ and target $y^{\star}$ is the instance
$P(\mathbf{x}_{\mathrm{user}},\,y^{\star},\,\mathcal{C}_{\mathrm{dom}},\,\boldsymbol{\lambda})$
with all three weights strictly positive:
$\lambda_{\mathrm{prox}},\lambda_{\mathrm{cons}},\lambda_{\mathrm{div}}>0$.
\end{proposition}

\proofsketch
Setting $\mathbf{x}_0=\mathbf{x}_{\mathrm{user}}$ and activating the
proximity term instantiates the canonical counterfactual objective of
Wachter~et~al.\ \cite{wachter2018counterfactual},
$\min_{\mathbf{x}'}\ell(f(\mathbf{x}'),y^{\star})+\lambda\|\mathbf{x}'-\mathbf{x}\|$,
embedded within the set-valued extension of \cite{mothilal2020}.  The
optimizer must simultaneously minimise prediction error and the $\ell_1$
distance to $\mathbf{x}_{\mathrm{user}}$, producing minimal-edit
counterfactuals—algorithmic recourse in the sense of
\cite{korikov2021}.\hfill$\square$

\begin{proposition}[What-if as $P$]
\label{prop:whatif}
The \emph{what-if} query in which features $S\!\subseteq\![d]$ are fixed to
values $\{v_j\}_{j\in S}$ is the instance
$P(\mathbf{x}_{\mathrm{user}},\,y^{\star},\,\mathcal{C}_{S},\,\boldsymbol{\lambda})$
with $\lambda_{\mathrm{prox}}\!=\!0$ (or $\lambda_{\mathrm{prox}}\!\to\!0$)
and $\mathcal{C}_{S}=\mathcal{C}_{\mathrm{dom}}\cup\{x'_j=v_j:j\in S\}$.
\end{proposition}

\proofsketch
The equality constraints in $\mathcal{C}_{S}$ enforce the user-specified
interventions; with $\lambda_{\mathrm{prox}}=0$ there is no incentive to
remain near $\mathbf{x}_{\mathrm{user}}$, so the loss reduces to
$\mathcal{L}_{\mathrm{valid}}$ subject to the fixed-feature constraints.
The optimizer evaluates $f(\mathbf{x}')$ after enforcing the
intervention, making this a \emph{forward} prediction under intervention:
the counterfactual degenerates to a constrained surrogate evaluation, which
\cite{verma2020} identify as the ``what-if'' subclass of counterfactual
reasoning, and which \cite{gupta2024gfi} show is the forward direction of
the same latent optimization that governs inverse inference.\hfill$\square$

\begin{remark}[Forward/inverse duality]
Propositions~\ref{prop:recommend}--\ref{prop:whatif} reflect the
forward/inverse duality studied in \cite{gupta2024gfi}: recommend and
reconfigure are inverse instances of $P$ (output $y^{\star}$ is given; inputs
are optimised), whereas what-if is the forward instance ($\mathbf{x}'$ is
largely fixed by $\mathcal{C}_{S}$; the value $f(\mathbf{x}')$ is read
off).  The same loss landscape accommodates both directions because
$\mathcal{L}_{\mathrm{valid}}$ is differentiable everywhere and provides a
non-zero gradient signal regardless of which decision variables are free.
\end{remark}

\begin{corollary}[Architectural unification]
\label{cor:single-impl}
Because all three query types are instances of $P$ (Eq.~\eqref{eq:c3g-general}),
a single implementation of the C3G optimizer—one loss-evaluation loop,
one gradient-free solver, one constraint-projection step—handles all three
modes without modification.  The modes differ exclusively in
\emph{(a)}~how $\mathbf{x}_0$ is initialised (sampled from filtered data vs.\
copied from the user baseline) and
\emph{(b)}~which equality constraints populate $\mathcal{C}$ (none, or
$\{x'_j=v_j:j\in S\}$).
All other components—the validity hinge, the proximity $\ell_1$ term, the
domain-penalty aggregator $\Phi$, and the diversity reward—execute
identically on every call.  The unification is therefore not merely
conceptual but \emph{architectural}: query routing reduces to parameter
instantiation of $P$, with no query-type-specific code paths required.
\end{corollary}


==> Sections/card.tex <==
\newtcolorbox{datasetcard}{
  enhanced,
  breakable,
  colback=white,
  colframe=black!10,
  arc=3mm,              % rounded corners
  boxrule=0.5pt,
  left=8pt,right=8pt,top=8pt,bottom=8pt,
  drop shadow=black!25, % shadow
}

% A helper environment for consistent label/value layout inside the card
\newenvironment{cardcontent}
{\begin{tabularx}{\linewidth}{@{}>{\bfseries}l @{\hspace{8pt}} X@{}}}
{\end{tabularx}}




\begin{datasetcard}
\begin{cardcontent}
\usericon\; Question: &
What is $12 + 7$? \\
\roboticon\; Answer: &
The result is $19$. \\
\calcicon\; Metrics: &
Accuracy: 1.00 \quad | \quad Error: 0 \quad | \quad Notes: Correct \\
\end{cardcontent}
\end{datasetcard}

\vspace{8pt}

\begin{datasetcard}
\begin{cardcontent}
\usericon\; Question: &
Explain Newton's second law in one sentence. \\
\roboticon\; Answer: &
It states that the net force on an object equals mass times acceleration ($F = ma$). \\
\calcicon\; Metrics: &
Rubric: 4/5 \quad | \quad Hallucination: No \quad | \quad Notes: Good, concise \\
\end{cardcontent}
\end{datasetcard}

\vspace{8pt}

\begin{datasetcard}
\begin{cardcontent}
\usericon\; Question: &
Summarize the paragraph in 2 lines. \\
\roboticon\; Answer: &
(Answer text here, potentially longer and wrapping automatically.) \\
\calcicon\; Metrics: &
ROUGE-L: 0.61 \quad | \quad Length: 2 lines \quad | \quad Pass: Yes \\
\end{cardcontent}
\end{datasetcard}

==> Sections/causal.tex <==
% \tzi{too generic. revise.}
Structural Causal Models (SCMs) enable~\sysname to reason about how changes to system configurations influence performance outcomes beyond what correlations can capture. An SCM defines a set of variables (e.g., cores, memory, runtime) as a directed acyclic graph (DAG), where each variable is computed by a function of its causal parents and an exogenous noise term. These noise terms account for system randomness and unmeasured effects, such as scheduling delays or background contentions. In~\sysname, we use SCMs to evaluate whether a generated configuration is causally plausible, to quantify the sensitivity of performance to resource changes, and to identify which inputs most influence a target metric.

Through SCMs,~\sysname can simulate what happens when the value of a configuration parameter is changed. %we intervene—e.g., setting GPU count to 4—by modifying the corresponding equation while keeping the rest of the system intact. 
This lets us preserve realistic dependencies while exploring counterfactual scenarios. For linear models, we compute causal influence using path coefficients that reflect how much a change in input affects the output. In nonlinear cases, we use gradients to capture local sensitivity near a baseline configuration. This analysis is used in~\sysname to explain why a certain parameter matters and how much it contributes to observed variation in runtime, energy, or other metrics.

In practical terms, SCMs help us do three things. \banooqa{First, %we filter out any counterfactual or recommended configuration that violates known causal structure--such as changing interdependent parameters in isolation. Second, 
we generate explanations by computing causal attribution scores and reporting which features have the largest effect on a given outcome. %Third, 
Second, we perform uncertainty-aware validation by simulating what would happen under the same unobserved noise, ensuring that outputs remain consistent with past data. Third, we plot the median and standard deviations of the estimate effects of recommendations/suggestions alongside the median and standard deviations of the estimate effects of the data to verify that the causal estimates remain consistent and that no additional uncertainty has been introduced.}

Consider a simple HPC setup with variables \texttt{Cores}, \texttt{Mem}, and \texttt{Runtime}. If the DAG encodes that both cores and memory affect runtime, the structural equation for runtime might look like \( \texttt{Runtime} = \beta_{\text{core}} \cdot \texttt{Cores} + \beta_{\text{mem}} \cdot \texttt{Mem} + \epsilon \), where \( \epsilon \) captures background noise. Any configuration synthesized by~\sysname is valid only if it respects this relationship, stays within reasonable changes based on historical variation, and maintains the observed variability from the real system. These checks allow~\sysname to reject unrealistic recommendations, improve interpretability, and ensure that decision support outputs remain trustworthy and grounded in how the HPC system actually behaves.
% \tzi{SCM}
% Existing methods for evaluating counterfactuals and recommendations typically rely on predictive accuracy~\cite{}, distributional similarity~\cite{}, or even custom distance measures that compute subspace distance~\cite{banday2024perfgen}. However, these approaches lack mechanisms to verify whether the generated outputs are causally plausible. A recommendation may achieve the target performance in a predictive sense, but still violate known causal relationships in the system — for instance, by altering mutually dependent variables independently. To address this gap in evaluation methodology, we propose to leverage Structural Causal Models (SCMs)~\cite{} as a framework for evaluating the causal consistency of generated configurations. %By learning a causal graph from historical data, SCMs capture the directionality and dependencies between configuration parameters and performance metrics. 
% Mathematically, an SCM is defined as a tuple 
% \(
% \mathcal{M} = \langle {\mathcal{G}}, {\mathbf{f}}, {P_U} \rangle
% \), where $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ is a DAG representing the causal graph, $\mathbf{f} = \{f_i\}$ is a set of structural functions for each variable, $P_U$ is a distribution that models how likely it is that performance metrics will be affected by unobserved randomness. %Modeling this uncertainty explicitly allows us to reason not just about expected values, but about the distribution of possible outcomes given an intervention.

% % Explicitly modeling \( P_U \) allows us to simulate interventions while holding these noise factors fixed, enabling counterfactual reasoning about what would happen to the same job under a different configuration. This makes SCMs well-suited for evaluating and validating counterfactuals and recommendations in a causally coherent manner.



% %is a probability distribution over exogenous (noise) variables.
% % \vspace{0.2in}
% % \annotate[yshift=0.4em]{above,right}{graph}{Causal graph with nodes (variables) and edges (causal relations)}
% % \annotate[yshift=0.4em]{above,right}{struct_eqns}{Functions defining each variable based on its parents in the graph}
% % \annotate[yshift=0.4em]{above,right}{exog}{Unobserved factors accounting for randomness}


% %enable simulation of interventions (via do-calculus), where we can estimate the effect of setting a variable (e.g., \texttt{GPU=1}) while holding confounders constant. 
% SCM framework provides simulation capability that allows evaluating whether counterfactuals are causally consistent with known system behavior, and enables validating recommendations as configurations that are not seen in the data but should be feasible under the learned causal structure. %Compared to feature-space techniques such as DiCE, which optimize for outcome validity and diversity without explicit causal constraints, SCMs offer a principled way to assess and improve the trustworthiness of generated decisions. Moreover, combining both approaches allows us to explore trade-offs: DiCE offers search diversity, while SCM-based validation enforces structural realism. In this work, we use SCMs both to evaluate counterfactuals independently and to simulate interventions that support robust, interpretable recommendation generation.
% This principled approach enables an additional layer of stringent evaluation that improves the trustworthiness of~\sysname.


==> Sections/causal_graphs_table.tex <==
\begin{figure}[t]
\centering
\captionsetup{justification=centering, font=small}
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
\setlength{\floatsep}{0pt}
\setlength{\textfloatsep}{0pt}
\setlength{\tabcolsep}{0pt}  % horizontal gap between columns
\renewcommand{\arraystretch}{0.0}  % vertical spacing between rows

\resizebox{\textwidth}{!}{
\begin{tabular}{>{\centering\arraybackslash}p{0.5\linewidth} >{\centering\arraybackslash}p{0.5\linewidth}}

% Row 1
\begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{Figs/causal-graphs/pm100/pm100_mpc_cpc_graph.pdf}
    \caption{PM-100 NPC}
\end{subfigure} &
\begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{Figs/causal-graphs/sc19/comd.pdf}
    \caption{CoMD}
\end{subfigure} \\

% Row 3
\begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{Figs/causal-graphs/sc19/ft.pdf}
    \caption{FT}
\end{subfigure} &

\begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{Figs/causal-graphs/fugaku/final_cg.pdf}
    \caption{F-Data}
\end{subfigure} \\

\begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{Figs/causal-graphs/monet/monet_cg.pdf}
    \caption{Monet}
\end{subfigure} &
% Row 2
% \begin{subfigure}[b]{\linewidth}
%     \includegraphics[width=\linewidth]{Figs/causal-graphs/sc19/kripke.pdf}
%     \caption{Kripke}
% \end{subfigure} \\

% Row 4
\begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{Figs/causal-graphs/butter-e/butter_graph_stds.pdf}
    \caption{BUTTER-E}
\end{subfigure}\\
% \begin{subfigure}[b]{\linewidth}
%     \includegraphics[width=\linewidth]{Figs/causal-graphs/monet/monet_cg.pdf}
%     \caption{HotCloudPerf}
% \end{subfigure}

\end{tabular}
}
\caption{A subset of the causal graphs.}
\label{fig:causal-graphs-4x2}
\end{figure}

==> Sections/compass_begreat_dice_tabcf_bofire_reconstrunction.tex <==
\begin{table*}[!t]
\caption{\whatif reconstruction error. lower MAPE indicates better performance. Entries marked with \ding{56} indicate that training did not complete within the imposed time budget ($≤$ 30 mins), and thus no
configurations were generated}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{\sysname} & \textbf{\begreat} & \textbf{\bofire} & \textbf{DiCE} & \textbf{\tabcf} \\ \hline
Monet &\ding{213} & \ding{213} & \ding{213} & \ding{213} & \ding{56} \\ \hline
PM-100 & 0.2438 & \ding{213} & \ding{213} & 0.1885 & \ding{56} \\ \hline
BUTTER-E & 0.1946 & \ding{213} & \ding{213} &  0.1671 & \ding{56}  \\ \hline
CoMD & 1.5676 & \ding{213} & \ding{213} & 1.0804 & \ding{56} \\ \hline
FT & 0.8610 & \ding{213} & \ding{213} & 0.7909 & \ding{56} \\ \hline
\textcolor{blue}{HotPerfCloud$\uparrow$} & \ding{213} & \ding{213} & \ding{213} & \ding{213} & \ding{56} \\ \hline
\end{tabular}
\label{tab:what_if_experiments}
\end{table*}

==> Sections/counterfactual.tex <==
Figure~\ref{fig:overview} illustrates that counterfactual analysis is the backbone that powers different types of queries. 
Counterfactual analysis enables users to reason about alternative %system behaviors 
behaviors by generating new configurations that minimally differ from a given baseline and that would lead to a different performance outcome. 
It uses a pre-trained predictive model $f: \mathcal{X} \rightarrow \mathcal{Y}$, which can estimate performance metrics given a configuration $\mathcal{X}$. Based on the formulation proposed by Wachter et al.~\cite{wachter2017counterfactual}, once trained, the model’s parameters are held fixed during counterfactual generation. This constraint ensures that any change in output is caused solely by changes in the input configuration. %—not by retraining or model drift.
While in this work, we choose XGBoost~\cite{chen2015xgboost,chen2016xgboost} to train the model from the input tabular data because XGBoost has been widely used successfully; the choice of the predictive model can be selected by the users.

Counterfactual analysis requires users to specify an original configuration $\mathcal{X}$, and a desired $y^*$ target performance constraint, which can be single or multi-objective. $\mathcal{X}'_i$ is a counterfactual configuration and $f(\mathcal{X}'_i)$ is the predicted value. If the user does not specify $\mathcal{y}^*$, then~\sysname assumes that the user wants to achieve an optimal value for the identified performance target metrics for the dataset in question (\tzi{or is this recommendation?}). Although, in the prototype implementation of~\sysname, we use counterfactual analysis as the synthesis engine for all types of queries, the backend synthesizer engine can be extended or replaced to deploy many other synthesis engines such as~\gls{llms}, Generative Adversarial Network~\cite{creswell2018generative}, among many others. The rationale is that with minor modification, counterfactual analysis can be used as the unified engine for generation. While counterfactual analysis is the most suitable tool for the Exploratory (both kinds) and Modification queries, other generative methods are incapable of serving these three types of queries. However, counterfactual analysis can be extended to ask the prescriptive queries by assuming either a random initial baseline configuration or \tzi{what else?}. Thus this tool provides a unified backend for all types of queries and our choice of the backend.

\subsubsection{Recommendation}
\label{sec:recommend}
\input{Sections/recommend}

\subsubsection{Exploratory Analysis}
\label{sec:exploratory}
Counterfactual analysis can be formulated as an optimization problem over the input space that balances \tzi{three} different objectives: (1) validity: each generated configuration $\mathbf{x}'_i$ must lead the model $f$ to predict the desired target $\mathbf{y}^*$; (2) proximity: the configuration should change only what is necessary; inputs should stay close to the original $\mathbf{x}$, making changes actionable; and (3) diversity: the set of counterfactuals should represent distinct adjustment strategies, not minor variations of the same one. Equation~\ref{eqn:cf_loss} mathematically presents the loss function that is minimized to identify $N$ alternate configurations, where $N$ is specified by users or by default~\sysname generates \tzi{$5$} counterfactuals. 
% At the heart of this process lies a trained predictive model, \( f: \mathcal{X} \rightarrow \mathcal{Y} \), which estimates performance metrics (e.g., runtime, energy) given a configuration \( \mathbf{x} \). Once trained, the model’s parameters are held fixed during counterfactual generation. This constraint ensures that any change in output is caused solely by changes in the input configuration—not by retraining or model drift. This aligns with the principle from Wachter et al.~\cite{wachter2017counterfactual}, where counterfactual reasoning is framed as an optimization over the input space:
\vspace{0.2in}
\begin{equation}
\footnotesize
\resizebox{\columnwidth}{!}{
\eqnmarkbox[Green]{cf_loss}{\{\mathbf{x}'_1, \ldots, \mathbf{x}'_N\}} = \arg\min_{\{\mathbf{x}'_i\}} \left[
% \sum_{i=1}^N \eqnmarkbox[WildStrawberry]{validity}{\mathcal{L}(f(\mathbf{x}'_i), \mathbf{y}^*)} +
\sum_{i=1}^N \eqnmarkbox[WildStrawberry]{validity}{\mathcal{L}_{\text{valid}}(f(\mathbf{x}'_i), \mathbf{y}^*)} +
% \sum_{i=1}^N \eqnmarkbox[WildStrawberry]{validity}{\frac{1}{N} \sum_{i=1}^{N} (f(\mathbf{x}'_i) - \mathbf{y}^*)^2} +
\lambda_1 \eqnmarkbox[YellowOrange]{proximity}{\mathcal{L}_{\text{prox}}(\mathbf{x}, \mathbf{x}'_i)} -
\lambda_2 \eqnmarkbox[RoyalBlue]{diversity}{diversity}%{\text{det}(K)}
\right]
}
\label{eqn:cf_loss}
\end{equation}
\annotate[yshift=0.7em]{above,right}{cf_loss}{Optimal counterfactual set}
\annotate[yshift=0.50em]{above,right}{validity}{Ensures prediction is close\\ to specified target}
\annotate[yshift=-0.2em,xshift=-0.0em]{below,left}{proximity}{Penalizes large deviations\\ from the given config}
\resizebox{\columnwidth}{!}{
\annotate[yshift=-0.3em]{below,left}{diversity}{Promotes\\ distinct solutions}
}

% \vspace{0.15in}
% \noindent The optimization balances three objectives:
% \begin{itemize}[leftmargin=1.5em]
%     \item \textbf{Validity:} Each generated configuration \( \mathbf{x}'_i \) must lead the model \( f \) to predict the desired target \( \mathbf{y}^* \).
%     \item \textbf{Proximity:} The configuration should change only what is necessary; inputs should stay close to the original \( \mathbf{x} \), making changes actionable.
%     \item \textbf{Diversity:} The set of counterfactuals should represent distinct adjustment strategies, not minor variations of the same one.
% \end{itemize}
Where, %\textbf{Prediction Loss:} This term 
prediction loss, $    \mathcal{L}_{\text{valid}}(f(\mathbf{x}'_i), \mathbf{y}^*) = \frac{1}{N} \sum_{i=1}^{N} (f(\mathbf{x}'_i) - \mathbf{y}^*)^2$, ensures that the predicted performance of each generated configuration closely matches the user-defined performance goal. Next, proximity loss, $\mathcal{L}_{\text{prox}}(\mathbf{x}, \mathbf{x}') = \sum_{k=1}^{d} \frac{|\mathbf{x}_k - \mathbf{x}'_k|}{\text{MAD}_k}$, penalizes unnecessary deviations from the original configuration to preserve realism and make suggestions actionable in practice. Here, each feature difference normalized by its Median Absolute Deviation (MAD) to account for variability across features and ensure scale-invariant comparisons. Finally, the diversity loss term, $    \text{diversity} = \text{det}(K), \quad K_{ij} = \frac{1}{1 + \|\mathbf{x}'_i - \mathbf{x}'_j\|}$, promotes variation among counterfactuals. It computes a similarity matrix \( K \), where each entry $K_{ij}$ is the pair-wise distance between counterfactuals. The determinant \( \det(K) \) quantifies how diverse the generated samples are, a higher values indicate that the counterfactuals are spread out. %, not clustered, and represent distinct configuration options.
% encourages the generation of distinct counterfactuals by penalizing redundancy. It constructs a similarity matrix \( K \) where each entry \( K_{ij} = \frac{1}{1 + \|x'_i - x'_j\|} \) captures how similar a pair of counterfactuals \( x'_i \) and \( x'_j \) are. The determinant of this matrix, \( \det(K) \), serves as a compact measure of spread--larger values imply that the counterfactuals span a wider and more varied space of configurations, thus offering users a diverse set of feasible alternatives.



% \vspace{0.15in}
% \paragraph*{Component Losses}
% \begin{enumerate}[leftmargin=1.5em]
%     \item \textbf{Prediction Loss:}
%     \begin{equation*}
%     \mathcal{L}_{\text{valid}} = \frac{1}{N} \sum_{i=1}^{N} (f(\mathbf{x}'_i) - \mathbf{y}^*)^2
%     \end{equation*}

%     \item \textbf{Proximity Loss:}
%     \begin{equation*}
%     \mathcal{L}_{\text{prox}}(\mathbf{x}, \mathbf{x}') = \sum_{k=1}^{d} \frac{|\mathbf{x}_k - \mathbf{x}'_k|}{\text{MAD}_k}
%     \end{equation*}
%     where MAD is the median absolute deviation, used to normalize changes across features with different scales.

%     \item \textbf{Diversity Term:}
%     \begin{equation*}
%     \text{diversity} = \text{det}(K), \quad K_{ij} = \frac{1}{1 + \|\mathbf{x}'_i - \mathbf{x}'_j\|}
%     \end{equation*}
%     Maximizing this kernel matrix determinant encourages dissimilar solutions.
% \end{enumerate}

% \vspace{0.3em}
% \subsection{Example: HPC Resource Optimization via Counterfactuals}

% Suppose a user wants to improve job runtime using alternative resource configurations.

% \begin{itemize}[leftmargin=1.5em]
%     \item \textbf{Original Configuration:} \( \mathbf{x} = \{ \texttt{cores} = 64,~ \texttt{memory} = 128~\text{GB} \} \), with \( f(\mathbf{x}) = 1.2 \) hours
%     \item \textbf{Target Outcome:} \( \mathbf{y}^* = 1.0 \) hour
%     \item \textbf{Constraints:} cores ≤ 72, memory ≤ 256 GB
%     \item \textbf{MAD:} cores = 16, memory = 32 GB
% \end{itemize}

% Using Equation~\ref{eqn:cf_loss}, \sysname generates:

% \begin{align*}
% \mathbf{x}'_1 &= \{68~\texttt{cores},~128~\texttt{GB}\} \quad \text{(add cores)} \\
% \mathbf{x}'_2 &= \{64~\texttt{cores},~144~\texttt{GB}\} \quad \text{(add memory)}
% \end{align*}

% \noindent These results are:
% \begin{itemize}[leftmargin=1.5em]
%     \item Predictively valid (\( f(\mathbf{x}') \leq 1.0 \) hr)
%     \item Close to the original (within 15\%)
%     \item Feasible under system constraints
%     \item Diverse in their strategies (different resources adjusted)
% \end{itemize}


% \subsection{Methodological Framework}
% Counterfactual analysis generates alternative configurations, which are diverse and feasible inputs that minimally differ from a given instance to achieve a specified performance goal. In~\sysname, counterfactual analysis is formulated as a constrained optimization problem that balances three competing objectives: prediction validity, input proximity, and solution diversity. 

% \vspace{0.15in} \begin{equation} \eqnmarkbox[GreenYellow]{cf_loss}{{\mathbf{x}'_1, \ldots, \mathbf{x}'N}} = \arg\min{{\mathbf{x}'i}} \left[ \sum{i=1}^N \eqnmarkbox[WildStrawberry]{validity}{\mathcal{L}(f(\mathbf{x}'i), \mathbf{y}^*)} + \lambda_1 \eqnmarkbox[YellowOrange]{proximity}{\mathcal{L}{\text{prox}}(\mathbf{x}, \mathbf{x}'_i)} - \lambda_2 \eqnmarkbox[RoyalBlue]{diversity}{\text{det}(K)} \right] \label{eqn:cf_loss} \end{equation}

% \annotate[yshift=0.4em]{above,right}{cf_loss}{Optimal counterfactual set} \annotate[yshift=0.6em]{above,right}{validity}{Ensures prediction meets target} \annotate[yshift=-1.2em,xshift=0.5em]{below,left}{proximity}{Penalizes large deviations from original} \annotate[yshift=0.5em]{above,left}{diversity}{Promotes distinct solutions via kernel matrix}

% \vspace{0.1in} \noindent \textbf{Where:} \begin{itemize}[leftmargin=1.5em] \item $f: \mathcal{X} \rightarrow \mathcal{Y}$ is the trained predictive model \item $\mathbf{x} \in \mathcal{X}$ is the original configuration \item $\mathbf{y}^* \in \mathcal{Y}$ is the desired performance vector \item $K_{ij} = \frac{1}{1 + |\mathbf{x}'_i - \mathbf{x}'_j|}$ is the similarity kernel used to encourage diversity \end{itemize}

% \paragraph*{Component Losses}

% \vspace{-0.25em} \begin{enumerate}[leftmargin=1.5em] \item \textbf{Validity:} Ensures generated configurations achieve the desired outcome. 
% \begin{equation} \mathcal{L}{\text{valid}} = \frac{1}{N} \sum{i=1}^{N} (f(\mathbf{x}'_i) - \mathbf{y}^)^2 
% \end{equation}

% \item \textbf{Proximity:} Measures deviation from the original input using MAD-normalized distance. \begin{equation*} \mathcal{L}{\text{prox}}(\mathbf{x}, \mathbf{x}') = \sum{k=1}^{d} \frac{|\mathbf{x}_k - \mathbf{x}'_k|}{\text{MAD}_k} \end{equation*}

% \item \textbf{Diversity:} Rewards diverse counterfactuals by maximizing the determinant of the similarity kernel. \begin{equation*} \text{diversity} = \text{det}(K), \quad K_{ij} = \frac{1}{1 + |\mathbf{x}'_i - \mathbf{x}'_j|} \end{equation*} \end{enumerate}

% \vspace{0.3em} \subsection{Example: HPC Resource Optimization via Counterfactuals}

% We consider an HPC job where the objective is to reduce execution time through configuration adjustments.

% \begin{itemize}[leftmargin=1.5em] \item \textbf{Original Configuration:} $\mathbf{x} = {\texttt{cores} = 64,~ \texttt{memory} = 128~\text{GB}}$ with $f(\mathbf{x}) = 1.2$ hours. \item \textbf{Target Outcome:} $\mathbf{y}^* = 1.0$ hour. \item \textbf{Constraints:} cores $\leq 72$, memory $\leq 256$ GB. \item \textbf{Normalization:} MAD${\texttt{cores}} = 16$, MAD${\texttt{memory}} = 32$ GB. \end{itemize}

% Applying the counterfactual formulation in Equation~\ref{eqn:cf_loss}, \sysname generates:

% \begin{align*} \mathbf{x}'_1 &= {68~\texttt{cores}, 128~\texttt{GB}} \quad \text{(increased CPU)} \ \mathbf{x}'_2 &= {64~\texttt{cores}, 144~\texttt{GB}} \quad \text{(increased memory)} \end{align*}

% \paragraph*{Interpretation:} \begin{itemize}[leftmargin=1.5em] \item Both candidates achieve $f(\mathbf{x}') \leq 1.0$ hour (validity). \item Changes are within 15% of the original (proximity). \item Solutions illustrate different resource strategies (diversity). \item All configurations comply with cluster constraints (feasibility). \end{itemize}

% \noindent This formulation forms the basis of~\sysname’s counterfactual engine and underpins the exploratory and modification queries used in operational decision-making.

% Counterfactual analysis~\cite{} enables users to explore alternative scenarios and understand how different outcomes could have occurred under different conditions. Such explorations increase trustworthiness, transparency, and make AI/ML models interpretable. Specifically,~\sysname leverages counterfactual analysis to propose hypothetical configurations based on a given configuration and a predictive model. Those hypothetical configurations show how minimal changes are needed to alter a model's decision. For instance, given a predictive model $f$ and an input feature vector $X$, the corresponding prediction of the given $x$ is $y' = f(x)$. The goal of a counterfactual generation engine is to generate $n$ meaningful counterfactual configurations $X'$ by perturbing specific features within this given input $X$. The modified output $X'$ is then provided back to the predictive model $f$; it yields a distinctly different output $y'' = f(x')$. This improves the given predictive model in four different ways: (1) We can evaluate the sensitivity and variability of a model by analyzing how small changes in $x$ can affect the output, (2) The transition from $x$ to $x'$ and the corresponding changes from $f(x)$ to $f(x')$ make the predictive model's decision-making process visible and understandable. (3) The adaptation from $x$ to $x'$ can define a narrative of how different outcomes can be achieved, which is interpretable for humans. (4) $x'$ offers actionable guidance on what might be done in real world scenarios. 

% Wachter et al.~\cite{wachter2017counterfactual} address the methodology for determining counterfactuals from a predictive model and given sample. The function $f_w$ represents a predictive model parameterized by weight $w$. The weights w are optimized during the training phase of the predictive model. In the process of generating counterfactuals, $f_w$ is used to evaluate how modifications of an input $x'$ alter the predicted outcome, generating a new target $y'$, keeping the $w$ parameter constant in the generation process. Constant $w$ ensures that changes in the prediction are solely from the adjustment to the given input to the predictive model. To express the minimality, they introduce a distance function $d(x_i, x')$ to quantify the divergence of $x'$ and $x_i$. A factor $\lambda$ is introduced to trade off the prediction and closeness to the original instance. The overall optimization algorithm is as follows:

% \begin{equation}
%     \arg \min_{x'} \max_\lambda (\lambda(f_w(x') - y')^2 + d(x_i, x'))
%     \label{eq:wachter}
% \end{equation}

% However, the equation ~\ref{eq:wachter} lacks some key aspects of counterfactual generation. We first assume that our pipeline is responsible for generating $N$ counterfactuals ${x_1, x_2, ... x_n}$ from the given sample $x$. To generate meaningful and actionable counterfactuals, (1) we need to include diversity in the generated counterfactuals so that the pipeline provided offers a variety of actionable configurations, (2) our goal is to minimize changes from the original sample so that they can be placed close to the desired range, (3) the suggested actionable configurations must be feasible with real-world constraints. 

% So the optimized loss function for the counterfactual generation pipeline will be:

% \begin{equation}
%     CF(x) = arg \min_{x1,x2, ..xn}(Loss + \lambda_{1} * Proximity + \lambda_{2} * Diversity)
% \end{equation}

% Where, Loss is computed from the actual loss of the given machine learning predictive model, $\lambda_1$ and $\lambda_2$ are both parameters to control the proximity and diversity.

% \begin{equation*}
%     Loss = \frac{1}{N} * \sum_{i=1}^{N} \mathcal{L(f(x_i), x)}
% \end{equation*}

% Proximity is how close the generated counterfactual configurations are to the given sample.

% \begin{equation*}
%     Proximity = \frac{1}{k} * \sum_{i=1}^{N} \Delta(x_i, x)
% \end{equation*}

% We calculate the diversity using the  determinant of the kernel matrix given the counterfactuals.

% \begin{equation*}
%     Diversity = \det(M) 
% \end{equation*}

% where 

% \begin{equation*}
%     M(i, j) = \frac{1}{1 + \Delta(x_i, x_j)}
% \end{equation*}



% % %
% % Counterfactual analysis simulates hypothetical changes to an existing configuration. Given an original configuration $\mathbf{x}$ and a target outcome $\mathbf{y}^*$, \sysname generates a new configuration $\mathbf{x}'$ that would lead to the desired outcome under the predictive model:

% % \begin{equation*}
% % \mathbf{x}' = \arg\min_{\mathbf{x}'} \left[ \mathcal{L}_{\text{pred}}(f(\mathbf{x}'), \mathbf{y}^*) + \lambda_1 \mathcal{L}_{\text{dist}}(\mathbf{x}, \mathbf{x}') \right]
% % \end{equation*}

% % Where $\mathcal{L}_{\text{pred}}$ penalizes deviation from the target outcome, and $\mathcal{L}_{\text{dist}}$ penalizes large changes to the original configuration.

% % To support deeper exploration, \sysname extends this to generate \emph{Top-K counterfactuals} and \emph{Pareto frontiers} across multiple objectives:

% % \begin{equation*}
% % \mathcal{L}_{\text{diverse}} = \lambda_1 \mathcal{L}_{\text{pred}} + \lambda_2 \mathcal{L}_{\text{dist}} + \lambda_3 \mathcal{L}_{\text{div}}(\{\mathbf{x}'_j\})
% % \end{equation*}

% % This loss promotes diversity among counterfactuals that all meet the performance target. \sysname uses this to explore trade-offs between objectives such as energy efficiency and runtime.

% % %%%%%%%%%%%%%%%%%%
% % Counterfactual reasoning addresses questions of the form ``What would the outcome have been if the value of a particular parameter had been set differently?" Formally, given an input configuration $x \in R^d$ and a predictive model 
% % $f : R^d \rightarrow R^k$, the goal is to find a perturbed configuration $x'$ such that the model prediction changes in a desired way--e.g., achieving a target performance value $y^*$.

% % \vspace{0.2in} 
% % \begin{equation*} 
% % \eqnmarkbox[Green]{cf_instance}{\mathbf{x}'} = \arg\min_{\mathbf{x}'} \left[ \eqnmarkbox[WildStrawberry]{pred_loss}{\mathcal{L}_{\text{pred}}(f(\mathbf{x}'), \mathbf{y}^*)} + \lambda_1 \eqnmarkbox[YellowOrange]{distance}{\mathcal{L}_{\text{dist}}(\mathbf{x}, \mathbf{x}')} \right] \end{equation*} %\vspace{0.2in}
% % \annotate[yshift=0.4em]{above,right}{cf_instance}{Counterfactual\\ configuration} \annotate[yshift=0.4em]{above,right}{pred_loss}{Loss measuring deviation\\ from target outcome} \annotate[yshift=-1.0em]{below,left}{distance}{Penalty for deviating\\ from original configuration}

% % \noindent This formulation captures both counterfactual generation and explanation: it identifies minimal, plausible changes to the input that would yield the desired outcome. An extension to this formulation is the generation of diverse counterfactuals--multiple distinct configurations that satisfy the same target but reveal different pathways to improvement. This involves augmenting the objective with a diversity term:

% % \vspace{0.2in} \begin{equation} \eqnmarkbox[Green]{cf_diverse_loss}{\mathcal{L}(\mathbf{x}, {\mathbf{x}'j})} = \lambda_1 \eqnmarkbox[WildStrawberry]{pred_term}{\mathcal{L}{\text{pred}}} + \lambda_2 \eqnmarkbox[OliveGreen]{dist_term}{\mathcal{L}{\text{dist}}} + \lambda_3 \eqnmarkbox[RoyalBlue]{div_term}{\mathcal{L}{\text{div}}} \label{eqn:counterfactual_diverse} 
% % \end{equation} 
% % \annotate[yshift=0.4em]{above,right}{cf_diverse_loss}{Loss for generating\\ diverse counterfactuals} \annotate[yshift=0.8em]{above,left}{pred_term}{Ensures target performance\\ is achieved} 
% % \annotate[yshift=0.4em]{below,right}{dist_term}{Maintains proximity to original} 
% % \annotate[yshift=-0.4em]{below,left}{div_term}{Promotes diversity\\ among candidates}

% % \noindent Together, these formulations enable the system to explain why certain changes improve performance by identifying multiple valid and interpretable feasible alternatives within user-specified constraints.

% % \tzi{@ankur -- please describe the math and underlying theory of what DiCE uses.}

\textbf{How to use:} An~\gls{hpc}-specific example to put counterfactual analysis to perspective would be of a user wanting to reduce the runtime of an~\gls{hpc} job. The user would specify in~\sysname that the original configuration uses $64$ cores and $128$~GB memory, resulting in a predicted runtime of 1.2 hours. The user specifies a performance target of $1.0$ hour and provides system constraints such as $cores \le 72$ and $memory \le 256~GB$. \sysname uses Equation~\ref{eqn:cf_loss} to generate two valid counterfactuals: (1) increase cores to $68$ while keeping memory fixed, or (2) increase memory to $144~GB$ while keeping cores unchanged. Both satisfy the performance goal, remain within allowed bounds, and reflect distinct resource allocation strategies.

Counterfactual analysis supports two query templates from Table~\ref{tab:query-taxonomy}. The user may ask an inverse optimization query such as \textit{``What changes would reduce runtime to 1 hour?"} Alternatively, they may ask a forward what-if query: \textit{``What would happen to runtime if I increase memory to 144~GB?"}.~\sysname can answer both queries using the same counterfactual generation methodology.

==> Sections/counterfactual2.tex <==
\sysname uses counterfactual analysis as a unified backbone to power multiple types of decision-support queries. It allows users to simulate how system behavior would change under different configuration choices. Unlike predictive models that only forecast outcomes for given inputs, counterfactuals enable the generation of new inputs that satisfy user-defined outcomes. This inversion of reasoning--from predicting effects to searching for causes--makes counterfactual analysis the precise tool for exploratory and modification (three out of four) queries. %simulation, optimization, and failure prevention. 
It fills a key gap left by standard supervised learning: while models such as XGBoost~\cite{chen2015xgboost} can forecast performance (e.g., runtime), regular predictive methods cannot suggest what inputs would lead to desired outcomes. Counterfactuals fill this gap by solving the inverse problem where they optimize input perturbations under user constraints, with guarantees of proximity, diversity, and target satisfaction. This is especially valuable for~\gls{hpc} stakeholders who need to understand, not just predict, how to improve job outcomes or avoid performance anomalies. In~\sysname, we implement counterfactual generation over a fixed predictive model $f: \mathcal{X} \rightarrow \mathcal{Y}$, trained using XGBoost. Once trained, the model weights remain fixed during counterfactual generation, following the approach of Wachter et al.~\cite{wachter2017counterfactual}. Freezing model parameters ensures that all observed changes in predicted output yield from the modified input configuration, not from model retraining or parameter change.

\subsubsection{Mathematical Formulation}
\label{sec:cf-formulation}

Counterfactual analysis requires a baseline configuration to start from, which is $\mathbf{x} \in \mathbb{R}^d$. Given a target outcome $\mathbf{y}^* \in \mathbb{R}^k$, and a pre-trained predictive model $f$,~\sysname generates a set of $N$ counterfactuals $\{\mathbf{x}'_1, \ldots, \mathbf{x}'_N\}$ by solving the constrained optimization in Equation~\ref{eqn:cf_loss}. Users can specify $N$ in the config file or GUI. By default~\sysname uses $N=20$.
%
\vspace{0.2in}
\begin{equation}
\footnotesize
\resizebox{\columnwidth}{!}{$
\eqnmarkbox[Green]{cf_loss}{\{\mathbf{x}'_1, \ldots, \mathbf{x}'_N\}} = \arg\min_{\{\mathbf{x}'_i\}} \left[
\sum_{i=1}^N \eqnmarkbox[WildStrawberry]{validity}{\mathcal{L}_{\text{valid}}(f(\mathbf{x}'_i), \mathbf{y}^*)} +
\lambda_1 
\eqnmarkbox[YellowOrange]{proximity}{\mathcal{L}_{\text{prox}}(\mathbf{x}, \mathbf{x}'_i)} -
\lambda_2 \eqnmarkbox[RoyalBlue]{diversity}{diversity}
\right]
$}
\label{eqn:cf_loss}
\end{equation}
\annotate[yshift=0.9em]{above,right}{cf_loss}{Optimal counterfactual set}
\annotate[yshift=0.50em]{above,right}{validity}{Ensures prediction is close\\ to specified target}
\annotate[xshift=-2.0ex]{below,left}{proximity}{Penalizes large deviations \\ from a given config}
% \resizebox{\columnwidth}{!}{
\annotate[]{below,left}{diversity}{Promotes\\ distinct solutions}
% }
\vspace{0.2in}

%
The first term, $\mathcal{L}_{\text{valid}}(f(\mathbf{x}'_i), \mathbf{y}^*) = \frac{1}{N} \sum_{i=1}^N (f(\mathbf{x}'_i) - \mathbf{y}^*)^2$, ensures that the predicted outcome for each synthesized configuration closely matches the user-defined target $\mathbf{y}^*$. \\
%
The second term, $\mathcal{L}_{\text{prox}}(\mathbf{x}, \mathbf{x}') = \sum_{k=1}^{d} \frac{|\mathbf{x}_k - \mathbf{x}'_k|}{\text{MAD}_k}$, penalizes unnecessary deviations from the original configuration to preserve realism and make suggestions actionable in practice. Here, each feature difference is normalized by its Median Absolute Deviation (MAD) to account for variability across features and ensure scale-invariant comparisons.

% $\mathcal{L}_{\text{prox}}(\mathbf{x}, \ma_____thbf{x}'_i) = \sum_{k=1}^d \frac{|\mathbf{x}_k - \mathbf{x}'_{i,k}|}{\text{MAD}_k}$, minimizes unnecessary changes by penalizing deviations from the original configuration $\mathbf{x}$. Here, $\text{MAD}_k$ is the Median Absolute Deviation of feature $k$, computed from historical job data, and serves to normalize feature changes relative to their natural variability. 

The third term, $\text{diversity} = \text{det}(K), \quad K_{ij} = \frac{1}{1 + \|\mathbf{x}'_i - \mathbf{x}'_j\|}$, encourages variation among counterfactuals. It computes a similarity matrix \( K \), where each entry $K_{ij}$ is the pair-wise distance between counterfactual samples $x'_i$ and $x'_j$. The determinant \( \det(K) \) quantifies how diverse the generated samples are, a higher values indicate that the counterfactuals are spread out.

% encourages solution diversity by maximizing the determinant of a similarity kernel matrix $K$, where each entry is defined as $K_{ij} = \frac{1}{1 + \|\mathbf{x}'_i - \mathbf{x}'_j\|}$. This diversity term ensures that the synthesized counterfactuals are not minor perturbations of each other but instead span a broader space of distinct yet valid configuration options.

% \subsubsection{Applicability to Query Types}
% \label{sec:cf-queries}
% \tzi{@Ankur -- revise this section to explain in details how counterfactuals are being mapped to the recommendation task.}

% \ankur{I didn;t get where to put this: For recommendation query, we assume user will not provide the framework any query sample to explore. Hence, by analyzing the given constraints and user query, we introduce a heuristic to find optimal samples from the given samples. Our goal is to find the best K optimal configurations which gains better performance. After splitting train and test set from the given dataset, we filter which test samples meet the user queries as those samples will be truly unseen to the generative pipeline. Then we calculate distance of the  samples to the user queries and constraints. The lower the distance, we assume the optimal sample it is. We then invoke our generation pipeline with the optimal samples.}

% This formulation directly supports three of the four generative query types in~\sysname. For exploratory queries—both forward and inverse—counterfactuals enable users to simulate alternative scenarios or discover which changes would meet a target objective. A forward what-if query modifies a single parameter (e.g., node count) and evaluates its effect on outcomes such as runtime or power. An inverse optimization query asks which set of changes could reduce runtime or energy below a specified threshold. In both cases, the user provides either a modified $\mathbf{x}'$ or a target $\mathbf{y}^*$, and~\sysname uses Equation~\ref{eqn:cf_loss} to return multiple feasible configurations. For modification queries, where the goal is to avoid job failure or anomalous performance, the target outcome becomes a class label (e.g., failure = 0), and the predictive model $f$ is a binary classifier. The counterfactual engine identifies minimal changes to the original configuration that would alter the model’s decision, subject to feasibility and realism constraints. Although counterfactuals are not naturally suited for prescriptive queries,~\sysname adapts the same engine by generating multiple candidate baselines from the feasible configuration space and optimizing toward user-defined targets. While not globally optimal, this satisficing search enables the system to return configurations that meet multiple performance objectives without needing expert domain knowledge. Other generative methods like GANs or LLMs can propose configurations but cannot guarantee outcome validity or minimal changes, making them less suitable for query types that require traceable, causal adjustments.

% \subsubsection{Example: Runtime Reduction via Exploratory Counterfactuals}
% \label{sec:cf-example}

% Consider an HPC user whose job runs with 64 cores and 128~GB of memory, resulting in a predicted runtime of 1.2 hours. The user’s target is to reduce runtime to 1.0 hour while respecting constraints of at most 72 cores and 256~GB of memory. From historical job traces,~\sysname computes MAD values of 16 for cores and 32 for memory. Applying the counterfactual objective in Equation~\ref{eqn:cf_loss},~\sysname proposes two configurations: one increases cores to 68, holding memory constant; the other increases memory to 144~GB, keeping cores fixed. Both changes satisfy the target, lie within bounds, and illustrate different strategies. The user may initiate this process by issuing an exploratory optimization query—\textit{``What changes would reduce runtime to 1 hour?"}—or a forward what-if query—\textit{``What happens to runtime if I increase memory to 144~GB?"}.~\sysname uses the same counterfactual machinery to serve both requests, demonstrating its versatility across multiple query intents.


==> Sections/dataset_tables.tex <==
\begin{table}[t]
\tiny
\renewcommand{\arraystretch}{2}  
\setlength{\tabcolsep}{4pt}  
% \captionsetup{skip=2pt}  
\caption{Subset of feature names, where $N$ represents the number of samples and $p$ represents the number of features. To conserve space, we use regular expressions to represent hardware counters in the~\gls{sb} and~\gls{bgq} datasets and highlight the performance target variables in bold.}
% \centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{ |p{1.3cm}|p{4.5cm}|}
\hline

\textbf{App.} & \textbf{Example Features} \\ \hline
\multicolumn{2}{|c|}{{\textbf{HPC Datasets}}} \\ 
\hline
\parbox{1cm}{\cg,~\lu,~\ft,~\kripkepatki,\\~\comd, N=3180, p=7}& \parbox{4.3cm}{Power Cap, Task Count, Core Count, Placement, and Bandwidth, \textbf{runtime}} \\ 
\hline
\parbox{\linewidth}{\kripkemarathe, N=17386, p=23} &
\parbox{4.3cm}{DRAMPowerPerNode, ProcessorPowerPerNode, Ranks, App. specific input parameters, OMP, PKG\_LIMIT, DRAM\_LIMIT, AvgInst, AvgIpc, AvgArithFpu, AvgFreq, AvgTemp, ProcessorPower, DRAMPower, Nesting Order, \textbf{ExecTime}} \\ \hline

\parbox{\linewidth}{\hypre, N=50396, p=21} & \parbox{3cm}{DRAMPowerPerNode, ProcessorPowerPerNode, Ranks,  OMP, PMX, NS, MU, AvgIPC, Smoother, AvgTSC, AvgTemp, ProcessorPower, DRAMPower, Solver-related parameters, \textbf{ExecTime}}  \\ \hline

\parbox{\linewidth}{XSBench and OpenMC on~\gls{sb}, N=200, p=121} & \parbox{3cm}{
NumThread,~InputSize,~\textbf{EfficiencyLoss}, perf::[MEM$|$DTLB$|$LLC]\_[MISS$|$STALL],\\perf::[L$_1|$L$_2|$L$_3|$]\_[MISS$|$STALL]}  
\\ \hline

\parbox{\linewidth}{XSBench and OpenMC on~\gls{bgq}, N=200, p=145} & \tiny{\parbox{4.3cm}{
NumThread,~InputSize,~\textbf{EfficiencyLoss},
PEVT\_[XU$|$AXU$|$L1P$|$STL]\_[MISS$|$], PAPI\_[BR$|$STL$|$SYC])\_[STALL$|$CYC$|$MISS]}
}\\ \hline
% \parbox{1.5cm}{\hypre, N=50396, p=21} & \parbox{4cm}{DRAMPowerPerNode, ProcessorPowerPerNode, Ranks,  OMP, PMX, NS, MU, AvgIPC, Smoother, AvgTSC, AvgTemp, ProcessorPower, DRAMPower, Solver-related parameters,~\textbf{ExecTime}}  \\ \hline
\multicolumn{2}{|c|}{{\textbf{ML Datasets}}} \\ 
\hline
\parbox{1cm}{Airfoil, N=1503, p=5}& \parbox{3cm}{Frequency, Angle of attack, Chord length, Free-stream velocity, Suction side,~\textbf{Scaled sound pressure level}} \\\hline

\parbox{1cm}{NO2, N=500, p=8}& \parbox{4.3cm}{\textbf{NO2}, Cars per hour, temperature, wind speed, temperature difference, wind direction, hour of day, day number}  \\\hline

\parbox{\linewidth}{Crime, N=1994, p=127} & \parbox{3.7cm}{population, householdsize, PctEmploy, PctIlleg, medIncome,~perCapInc,~PctPopUnderPov,~\textbf{ViolentCrimesPerPop}}  \\\hline

\parbox{\linewidth}{SkillCraft, N=3395, p=16}& \parbox{3.7cm}{GameID, APM, SelectByHotkeys, AssignToHotkeys, MinimapRightClicks, NumberOfPACs,~\textbf{ActionLatency}} 
\\\hline
\end{tabular}
}
\label{tab:datasets}
\end{table}


% \begin{table}[t]
% \footnotesize
% \centering
% \caption{Instantiated Decision-Support Queries Across Datasets and Template Types}
% \label{tab:query_templates}

% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|p{1cm}|p{1.0cm}|p{2cm}|p{2cm}|}
% \hline
% \textbf{Template Type} & \textbf{Dataset} & \textbf{Instantiated Query} & \textbf{Structured JSON} \\
% \hline
% Recommendation Query & Fugaku \cite{antici2024f}  & Recommend me a <configuration> where \texttt{duration} is optimal and \texttt{exit state} is $user\_given\_state$ &
% \texttt{Type: Recommend} \newline
% \texttt{Targets:} \newline
% \quad \texttt{- duration: < 1000s} \newline
% \texttt{Constraints:} \newline
% \quad \texttt{- state}: \texttt{completed}
% \\
% \hline
% Exploratory Optimization Query & PM-100 \cite{antici2023pm100} & Given a base configuration <configuration>, how should I change my current configuration to achieve 'user\_percentage' reduction in \texttt{node\_power\_consumption}? &
% \texttt{Type: WhatIf} \newline
% \texttt{Baseline: ./inputs/job001.json} \newline
% %\texttt{Modified:} \newline
% %\quad \texttt{- num\_nodes: 4} \newline
% \texttt{Metrics:} \newline
% %\quad \texttt{- runtime} \newline
% \quad \texttt{- power} \\
% \hline
% Exploratory What-If Query  & SC'19 \cite{patki2019performance} & Given a base configuration <configuration> what if I double the \texttt{task\_count}, what would be the \texttt{runtime}? &
% \texttt{Type: Counterfactual} \newline
% \texttt{Baseline: ./inputs/job002.json} \newline
% \texttt{Target:} \newline
% \quad \texttt{- runtime: 0 - max} \newline
% \texttt{Constraints:} \newline
% %\quad \texttt{- qos: = 1} \newline
% \quad \texttt{- num\_tasks: = 128} \\
% \hline

% \ankur{My classification query}  & --- & ---  &\\
% \hline

% \end{tabular}
% }

% \end{table}

==> Sections/explanation.tex <==



% \textbf{Causal Graph} For \discover queries, \sysname presents a directed causal graph (\bcircled{5} in Figure~\ref{fig:wander-gui}) with annotated arrows indicating directional and quantified influences from features to targets. For example, ``increasing \texttt{num\_cores\_req} increases \texttt{cpu\_power\_consumption} by 12.3\%.'' These graphs expose structural drivers that predictive models cannot detect, enabling users to reason about root causes with evidence grounded in causal structure.

% \sysname decouples decision generation from decision interpretation. While Section~\ref{sec:counterfactual} describes the backend that synthesizes candidate configurations, the explanation module interprets these outputs and communicates their implications to stakeholders. The rationale for this separation is that configuration synthesis only answers what is possible; it does not explain 
% % answers 
% why it works, how trustworthy it is, and which option best serves the user's goals.

% To support informed decision-making, \sysname delivers three forms of explanatory evidence for every generated configuration. First, it provides explanation of what changed and how that impacted the performance metrics using natural language. Second, it offers causal and uncertainty diagnostics to assess trustworthiness. Third, it presents ranked summaries and trade-off metrics to help users choose among feasible alternatives. The next three subsections describe each of these capabilities in detail.



% \subsubsection{Interpretability}

% %This subsection answers the question: what features were modified compared to a baseline (either user specified or randomly selected) and why those changes matter. 
% For each synthesized configuration \( \mathbf{x}' \), \sysname generates a textual explanation that highlights: (1) what changed from the original \( \mathbf{x} \), (2) the predicted performance impact from \( f(\mathbf{x}') \), and (3) the likely mechanism of improvement (e.g., improved parallelism, memory efficiency). This supports transparency and interpretability by helping users understand the rationale behind each recommendation. To communicate this information,~\sysname presents a table with rows showing the recommendations, predicted metrics, and the generated natural language explanation using any open-source LLM. For our experiments, we used OpenAI's GPT-4o, however, any open source LLM framework such as Ollama~\cite{} provides access to many high-fidelity open-sourced and local models that can be called instead, in the future. %For generating natural language explanation, use needs to use their own API key. If the API key is not available, the natural language explanation is not available.

% \textbf{Visualization:} Inline example of textual output; sample table row from the recommendation list showing configuration delta, predicted metric, and the generated natural language explanation.

% \subsubsection{Trustworthiness}

%This subsection answers: should I trust the predicted effect of this change? 
% To enhance the trustworthiness of the generated samples, \sysname reports two diagnostics for each \( \mathbf{x}' \): (1) causal consistency shown using a violin chart--whether the distributions of the causal influences of each feature matches between the real data and synthesized data, and (2) prediction error and uncertainty showing how confident the model is in its prediction using a MAPE chart with error bars when certain recommended configurations are used. These diagnostics help prevent blind trust in model output and highlight suggestions that are both plausible and stable.

% \textbf{Visualization:} A causal DAG (e.g., from SCM) showing the learned structure; a warning icon next to suggestions that violate dependencies; confidence intervals shown as error bars in tables or as violin/range plots across predictions.

%s\subsubsection{Decision Support} %: Which option should I pick?}

% To achieve the ultimate goal of supporting stakeholders make a decision about which suggestion to choose when several recommendations meet the user’s performance goals,~\sysname scores each one using a composite trade-off score, and a radar chart showing how each option balances competing performance metrics.



==> Sections/fix.tex <==

\begin{itemize}
    \item \tzi{The proposed work is limited to tabular performance data, with no integration with runtime traces or code-level signals. @BANOOQQA: Please use code level signals for your example so that reviewers are not mislet to think that we cannot handle them.}
    \item \st{The authors did not discuss on how Compass handles or recovers from failure cases, which raise some questions about its practical value.}
% \item \tzi{Compass targets the same optimization goal as RL and Bayesian auto-tuning methods but did not have comparison with them.}
\item  \tzi{Compass targets the same optimization goal as reinforcement learning and Bayesian optimization–based auto-tuners: finding configurations that optimize system performance, but the paper does not compare against these well-established baselines. For example, BOHB [1], Metatune [2] and PAMaliboo [3], are focused on HPC tuning and represent strong alternatives for automated configuration search. The authors need to compare Compass with these approaches in terms of performance, efficiency, runtime cost. [1] Falkner, Stefan, Aaron Klein, and Frank Hutter. "BOHB: Robust and efficient hyperparameter optimization at scale." International conference on machine learning. PMLR, 2018. [2] Ryu, Jaehun, and Hyojin Sung. "Metatune: Meta-learning based cost model for fast and efficient auto-tuning frameworks." arXiv preprint arXiv:2102.04199 (2021). [3] Guindani, Bruno, et al. "Efficient parameter tuning for a structure-based virtual screening HPC application." Journal of Parallel and Distributed Computing 202 (2025): 105087.} We also need to say that these can do Recommend, but cannot do REconfig and What-if. 
\item \tzi{Data reduction method needs more clear clarification and evaluation. The presentation of the data reduction method (loss-proportional sampling) is fragmented between §3.2 and §6.4 and omits key algorithmic details. Please consolidate the method in §3, and provide the exact procedure used to tune 
$\lambda$ (step 3 in §6.4).}

\item \tzi{The paper should report sensitivity to subset size, replace the single operating point in Table 4 with curves over multiple sampling fraction α.}
\item \tzi{Since surrogate models produce different numbers, I am not sure whether the conclusion would be different if the surrogate model were the same.}
\end{itemize}

==> Sections/impl2.tex <==
% \begin{figure}[t]
%     \centering
% \includegraphics[width=0.48\linewidth]{Figs/howtouse.pdf}
%     \caption{\sysname supports both offline and online usage. In offline mode, users train the generative model and perform interactive, query-driven exploration for decision support. In online mode, the trained model is deployed to serve real-time recommendations in dynamic environments.}
%     \label{fig:enter-label}
% \end{figure}
% \sysname achieves scalability and interactivity through distributed data processing, hybrid parallelism, automated modeling, explainable reasoning, and user-driven interaction. 
% Users interact with \sysname in natural language through a chatbot that captures requirements: query type (\reco, \modify, or \whatif), target objectives, immutable features, and any filters or constraints. 
Once user requirements are collected by the front end (Section~\ref{sec:chatbot}), \sysname automatically executes a full pipeline consisting of data preprocessing, model selection, generative modeling (Section~\ref{sec:modeling-engine}), reliability and explanation (Section~\ref{sec:reliability}), and actionable outcome generation (Section~\ref{sec:actionable-outcome}).
While Section~\ref{sec:methodology} describes the individual components, this section focuses on the system-level design choices that make \sysname scalable in practice, including data preprocessing, hybrid parallelization, and the synthesis backend. Appendix~\ref{app:appendix} illustrates the user interface.

\subsection{Data Preprocessing}
\label{sec:data-preprocessing}
All preprocessing stages are implemented as partitioned Dask dataflow \tzi{CITE} operations and executed lazily, with materialization only at stage boundaries. The pipeline follows a deterministic sequence: (1) remove samples with missing values in required features; (2) drop user-specified columns; (3) apply constraint-preserving subset sampling to reduce the candidate set; (4) filter samples based on user-defined target conditions; (5) mark immutable features as hard constraints during counterfactual generation; (6) split the dataset once into 80\% training ($X_{train}$) and 20\% validation ($X_{val}$) partitions, reused across queries; and (7) normalize numerical features using statistics computed exclusively from $X_{train}$ via StandardScaler~\cite{} \tzi{} and encode categorical features using OneHotEncoder~\cite{pedregosa2011scikit}.
Reliability of the generated samples are computed solely based on $X_{val}$.

\noindent
For $\modify$ and $\whatif$ queries, users select one observed input–output pair from $X_{train} \cup X_{val}$ as a baseline. In contrast, $\reco$ queries do not require a user-provided baseline. Instead, \sysname selects baselines from a reduced candidate pool obtained after filtering and subset sampling. If no sample in this pool satisfies all user-specified constraints, \sysname selects a random sample from $X_{test}$ to start. 
% \tzi{If no sample in this pool satisfies all user-specified constraints, \sysname abstains from generating a recommendation and reports the query as infeasible, as satisfying the request would require extrapolation beyond the observed data distribution.} 
% For multi-objective queries, however, \sysname does not require joint optimality across objectives. Each objective is evaluated independently: 
For minimization and maximization objectives for the given target, \sysname identifies the extreme value and constructs an objective-specific neighborhood by selecting samples within a bounded range around it (e.g., from $\text{min}-Q_1$ to $\text{min}+Q_1$ for minimization), while range objectives are preserved exactly. The union of these objective-consistent samples constitutes the satisficing pool of samples.

% \tzi{to do what? these are not the recommendations, then why do we do this step? @ankur}. 
% \subsection{Automatic Model Selection}
% \sysname either uses a pre-trained performance model or builds one automatically.  
% When users provide a model, \sysname applies it directly for counterfactual reasoning.  
% When no model is supplied, \sysname trains multiple candidate architectures in parallel and selects the one with the lowest validation loss as the surrogate. \ankur{Sigmetrics Fix: If there is a tie between the models, we randomly pick a model for downstream analysis}.  
% Table~\ref{tab:all_models_results} lists the modeling approaches that the \texttt{Model Selection} module currently supports.  
% In future work, \sysname will incorporate data-intensive architectures such as transformers to improve generalization.  
% For automatic training, \sysname splits the training partition of the dataset into 80\% for training and 20\% for validation and uses validation loss to select the best surrogate model. 
% \sysname keeps the selected model fixed across queries to prevent drift and maintain consistent reasoning.  
% This automated process eliminates manual tuning and ensures that each dataset is matched with a well-fitted model.


\subsection{Hybrid Parallelization for Scalability}
\label{sec:parallel}

To scale to large datasets and billions of samples, \sysname employs a hybrid-parallel execution model that combines Dask~\cite{matthew_rocklin-proc-scipy-2015}, MPI, and multiprocessing. The input dataset is sharded into distributed DataFrame partitions and assigned across MPI ranks, preserving data locality and avoiding full-data replication. Within each rank, multiple multiprocessing workers operate in parallel on local shards.
Preprocessing and filtering stages are perfectly parallel across ranks and workers. Subset sampling and counterfactual synthesis are executed independently per worker, enabling scalable candidate generation without inter-worker communication. Each worker is initialized with a unique random seed derived from a global seed, introducing diversity while preserving reproducibility across runs, and locally discards samples that violate user-specified constraints. After local generation completes, Rank~0 aggregates the valid candidate sets produced by all ranks, removes duplicates, and applies multi-threaded execution of Algorithm~\ref{alg:assess_reliability} to compute per-sample reliability. This design minimizes communication overhead by restricting coordination to a single aggregation phase. % and allows \sysname to efficiently exploit both intra-node and inter-node parallelism.

% \begin{table*}[t]
% \centering
% \caption{Summary of confidence level interpretations based on NLL, OOD, support, and desirability scores.}
% \small
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|l|p{4cm}|p{3cm}|p{3cm}|p{4cm}|}
% \hline
% \textbf{Confidence Level} & \textbf{Model Behavior} & \textbf{Data Similarity} & \textbf{Model Probability (NLL)} & \textbf{Actionability} \\
% \hline \ \textbf{High Confidence} 
% & Strong belief, well supported 
% & In-distribution (familiar) 
% & High (low NLL) 
% & Fully trustworthy; low uncertainty \\
% \hline
% \ \textbf{Moderate Confidence} 
% & Plausible but not perfect 
% & Near distribution edge 
% & Medium (moderate NLL) 
% & Needs some review or extra checks \\
% \hline
% \ \textbf{Low Confidence} 
% & Unlikely / poorly supported 
% & Out-of-distribution 
% & Low (high NLL) 
% & High uncertainty; should not auto-act \\
% \hline
% \end{tabular}
% }
% \label{tab:confidence_levels}
% \end{table*}
% \subsection{Counterfactual Generation Engine}
% \sysname supports any counterfactual generation library as a backend, allowing users to switch or extend it with minimal changes.  
% We compared two state-of-the-art libraries—DiCE~\cite{mothilal2020explaining} and TABCF—and found that DiCE consistently generated valid counterfactuals for all datasets and queries, whereas TABCF failed on several.  
% Based on this result, \sysname sets DiCE as the default backend but keeps the interface modular so users can replace it with other libraries in the future.  
% During execution, \sysname launches multiple DiCE instances with different random seeds to ensure diverse counterfactuals that adhere to user constraints.  
% % After generation, \sysname evaluates all results using the metrics in Table~\ref{tab:tabcf_comp} and visualizes them for user interpretation.

% \subsection{User Interpretation}
% \sysname assigns each sample a \texttt{confidence\_tag} with one of three levels: High, Moderate, or Low.  
% Table~\ref{tab:confidence_levels} summarizes these levels.  
% A \texttt{High Confidence} tag indicates that the model has seen similar scenarios before and strongly supports the recommendation; such results require minimal human review.  
% \texttt{Moderate Confidence} means the model finds the outcome plausible but not ideal, suggesting human validation before action.  
% \texttt{Low Confidence} indicates high uncertainty, often due to novel or poorly supported scenarios and should be reviewed carefully with human oversight.


\subsection{Decoupled Modeling Engine as the Backend}
\tzi{Can we remove this, not benefiting?}
\label{sec:backend}
While Section~\ref{ref:chatbot} details the user-facing interaction, the \sysname core modeling and decision logic is fully decoupled from the UI and implemented as a Django-based back-end. This architecture ensures that the system can support both interactive human querying and programmatic access by external software.

% \st{The back-end exposes three primary REST API endpoints: (1) dataset analysis and metadata extraction; (2) counterfactual generation for user-specified queries; and (3) response generation, which returns the top-5 recommendations, reliability scores, explanatory summaries, and---where applicable---targeted data collection suggestions.}

% \st{The backend can be hosted on localhost or the cloud for broader accessibility. For offline analysis or integration into automated decision-making pipelines, external software systems can bypass the UI to interact directly with these backend APIs. This allows \sysname to be invoked within batch or real-time workflows while maintaining identical query semantics as the UI-driven version. Figure~\ref{fig:wander-gui}B illustrates this back-end-only deployment mode, highlighting how the engine functions as a standalone decision-support service for non-human agents.}
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{Figs/compass-ui.pdf}
% \caption{\sysname's chatbot interface. User (a) selects a query type: \reco, \modify, or \whatif, (b) selects a dataset in \texttt{csv} or \texttt{parquet} format, (c) drops unnecessary columns, (d) responds to questions about specifying the target objectives.}
%     \label{fig:compass-ui}
% \end{figure*}
% \sysname implements a front-end chatbot using ReactJS to provide an interactive interface for user requirement gathering. 
% It leverages the Virtual DOM for efficient updates and manages all user communication through a clean REST API. 
% The back-end, implemented in Django, hosts three key API endpoints: 
% (1) dataset analysis and metadata visualization; 
% (2) counterfactual generation for user-specified queries; and 
% (3) final response presenting the top $K$ recommendations with human-readable explanations and evaluation metrics. 
% All requests are processed locally through a REST server running on \texttt{localhost}, preserving user data privacy. Figure ~\ref{fig:compass-ui} demonstrates a demo of our \sysname UI, where users can select their query types, set their different constraints, and ask \sysname to generate hypothetical scenario based on their query. Additionally, as shown in Figure~\ref{fig:wander-gui}B, \sysname can be used offline to train models or deployed in dynamic environments to make real time decisions.
% This modular client-server architecture enables seamless interaction, rapid response times, and extensibility for integration with HPC schedulers or cloud services.
% \tzi{may be add a few screenshots showing the chat history for the three queries and a snapshot of the output table.}
% \textbf{The User Interface \& Interaction}
% For interactive, human-in-the-loop querying, \sysname provides a front-end interface (Figure~\ref{fig:compass-ui}). Through this UI, users can select a query type (\reco, \modify, or \whatif), upload datasets in \texttt{csv} or \texttt{parquet} format, and specify data by dropping irrelevant or sensitive columns. The interface allows users to define optimization objectives and hard constraints. For \modify and \whatif queries, users specify a baseline configuration to serve as the reference point for counterfactual generation. The UI guides users through query formulation and displays the resulting top-K recommendations alongside evaluation metrics and human-readable explanations. If constraints cannot be satisfied without extrapolation, the system explicitly reports infeasibility.


==> Sections/implementation.tex <==
\begin{figure}[t]
    \centering
\includegraphics[width=0.48\linewidth]{Figs/howtouse.pdf}
    \caption{\sysname supports both offline and online usage. In offline mode, users train the generative model and perform interactive, query-driven exploration for decision support. In online mode, the trained model is deployed to serve real-time recommendations in dynamic environments.}
    \label{fig:enter-label}
\end{figure}
\sysname is implemented in Python, with modular components illustrated in Figure~\ref{fig:overview}. The GUI is built using Streamlit, and all configurations are specified via JSON.
Figure~\ref{fig:howtouse} shows how \sysname supports both offline and online usage. In the offline mode, \sysname trains models and serves decisions through the GUI. In the online mode, \sysname can be deployed to support runtime decisions. However, the current prototype does not yet support streaming updates; incorporating new labeled or unlabeled data during online scenarios into generative models remains an open research challenge. As such, the online mode is deployment-only.


\subsection{Data Preprocessing}
After loading data into a pandas dataframe ~\cite{mckinney-proc-scipy-2010}, \sysname (1) drops the missing values from the dataframe; %, as missing values can adversely affect both model training and counterfactual generation quality. We 
(2) drops user-specified columns in the \texttt{dropped\_columns}; % the User Interface. 
%To reduce computational complexity while maintaining statistical representativeness of the original dataset, we 
(3) applies the subset sampling technique for data reduction if \texttt{subset\_sampling: True}. By default it is \texttt{True}; 
(4) filters samples from this reduced set based on the user-specified target conditions; %targeted range with a 10\% buffer range. 
(5) marks features that are not specified in the user query as immutable so that the generative model does not change some of those columns;
(6) splits the subsampled and filtered data into a 80-20\% split where 80\% samples are used as the train set, and the remaining 20\% samples as the test set for both synthesis and sample- and dataset-level evaluation; %, and test samples are used for data generation and further downstream analysis. 
(7) Finally, \sysname normalizes by StandardScaler ~\cite{pedregosa2011scikit} and encodes string values using OneHotEncoder ~\cite{pedregosa2011scikit} to the training partition. It is ensured that the test set is unseen to the generation pipeline. 
(8) We do not have any samples available to initiate the $\reco$ query. Therefore, to guide the generation pipeline, we randomly select a sample from the target dataset whose target column falls within the target range of our query. For $\modify$ and $\whatif$ query, the user has to provide at least one baseline configuration.% We define this as ``samples".

\subsection{Parallel Implementation of \synthesis and Evaluation Components}


\sysname implements its counterfactual generation backend using DiCE~\cite{mothilal2020explaining}, a widely used framework for generating diverse alternatives. To enhance diversity in the generated samples, \sysname adopts an ensemble-based approach by initializing multiple DiCE models with different random seeds. 
Since the generation process is inherently probabilistic,
generating a small number of samples risks missing important regions of the counterfactual space. Moreover, evaluating distributional consistency in feature-target relationships across datasets requires a statistically meaningful sample size. Hence, while a user may only seek a few high-quality recommendations, \sysname generates $N$ samples per query, where $N=2000$ set by the system by default. 

However, generating thousands of counterfactuals per query is computationally expensive. To address this challenge, we implement \sysname using a hybrid parallelization strategy using MPI and multiprocessing. The total workload of generating $N$ counterfactuals is divided across $n$ MPI ranks, with each rank responsible for $N/n$ samples. Within each rank, \sysname spawns $m$ multiprocessing workers, typically mapped to available CPU cores, such that each worker produces approximately $\lceil (N/n)/m \rceil$ samples. 
Once local generations complete, each rank apply user specified constraints, apply the sample-quality measurement methods, then  rank 0 gathers all outputs from participating ranks, and deduplicates. Finally, 

\subsection{Implementation of Front-end and Back-end}
\sysname combines a lightweight user-facing front-end with a high-throughput, modular backend implemented. 

\subsubsection{Lightweight Front-End}

\sysname provides a lightweight chatbot interface with ReactJS \tzi{cite} to ensure a dynamic, responsive, and engaging user interface. We leverage the Virtual Document Object Model (VDOM) provided by the ReactJS framework, 
enables highly efficient updates to the user interface by minimizing direct manipulation of the browser's actual DOM. Users provide query types, target variables, and different constraints using useful react components. Once the user provides the necessary information, a valid configuration object is generated. The configuration is passed to the backend, and the backend is responsible for sending back user queries as requested.

\subsection{Django Back-End}
\tzi{Need to formulate this line: Browsers block direct access to local files as a fundamental security measure to prevent malicious websites from stealing sensitive data or harming your computer.} To communicate with the chatUI to our engine, we architect the backend using a RESTful API (Representational State Transfer Application Programming Interface) \tzi{cite}, which provides a seamless client-server model to ensure scalability and the decoupling of system components. We use the Django Framework \tzi{cite} written in Python for its rapid development capabilities, inherent security features, and powerful ecosystem, which streamline the creation of robust and standardized API endpoints. We provide three robust API to the chat UI: (1) the first UI analyzes the given dataset and offers the user insights into the dataset, including data distribution and different metadata. (2) For \modify and \whatif, the user needs to select baseline configurations so that our backend can offer suitable configurations based on the given constraints. (3) Final response to the user queries containing the top $K=5$ suitable configurations and their human readable explanations with different performance metrics. 
Each setup is done in $localhost$, which ensures that user's data privacy is guaranteed, and it will not be uploaded to another server or any other host.




==> Sections/intro-hpdc-old.tex <==
\gls{hpc} systems enable scientific advancements across critical fields such as materials design, genomics, astrophysics, and nuclear stockpile stewardship. These systems handle computations that are infeasible otherwise, due to immense workload complexity, and data size. Despite their capabilities, fully utilizing~\gls{hpc} systems remains challenging. Architectures now include CPUs, GPUs, and specialized accelerators, increasing the complexity of decisions that need to be made by various stakeholders, from domain scientists to system admins to job schedulers. Optimizing performance involves navigating high-dimensional configuration spaces, from hardware selection and resource allocation to execution strategies and power management. Thus, ``performance" is no longer a simple optimization task but rather a trade-off space between multiple conflicting objectives.

Operational decisions in HPC span various scenarios, impacting diverse stakeholders. Novice users need guidance on configuration parameters to achieve desirable time-to-solution, advanced users need reconfiguration suggestions to finish faster than the previous attempt, runtime systems must dynamically reconfigure policies to maximize both job-specific time to soution as well as system-wide energy efficiency and power cap requirements, and HPC facility operators require informed policy-making to ensure that default policies do not introduce network variability or run-to-run variability. 
Prior studies show that in the Catalyst supercomputer, a system-wide policy of using \texttt{task\_binding} algorithm to be \texttt{rand} system-wide policy by the HPC facility led to $4\times$ runt-to-run variability in network-bound application~\cite{patki2019performance}. Thus, poor decisions in any of these scenarios risk inefficiencies, resource waste, increased operational costs, and reduced scientific productivity. 

Although extensive research addresses performance modeling and autotuning~\cite{bhatele2019perfexplorer, tallent2013hpctoolkit, gamblin2015spack, jannesari2017performance}, existing solutions remain fragmented and limited. Predictive models typically focus solely on forecasting performance outcomes, providing little to no capability for exploratory reasoning—such as systematically evaluating hypothetical scenarios—or quantifying how specific input changes influence outputs. Moreover, these methods rarely offer explanations for their predictions, reducing interpretability and user trust. Rule-based recommenders, while interpretable, are rigid and lack the flexibility required for systematic exploration across varied contexts. Consequently, users repeatedly build specialized tools for individual datasets, requiring considerable domain expertise and lacking generalizability. %Critically, current methods do not systematically bridge observational data with actionable intervention, causing ad-hoc and nonportable workflows. 
If this gap remains unaddressed, HPC decision-making will continue to rely on repetitive, inefficient, and non-portable analysis methods. %This gap prevents domain experts from easily exploring their data and making informed decisions without having to repeatedly build specialized tools themselves, learn machine learning, or collaborate closely with ML specialists. Our ML-driven tool, \sysname, specifically aims to remove this barrier.

To fill this critical gap, we propose to formulate the above four decision-support queries and what-if exploration as a generative counterfactual analysis problem. Counterfactual analysis, central to \sysname, differs from predictive modeling by explicitly identifying minimal input changes from a previous trial to achieve desired outcomes. Although counterfactual analysis is still a generative modeling approach, unlike traditional generative models such as Large Language Model (LLM)-based models, counterfactuals provide minimal and actionable changes to queries. Finally, we implement a unified decision-support framework--\sysname--
integrating predictive modeling, generative counterfactual analysis problem, uncertainty quantification, causal inference, and explainable AI within a structured, query-driven interface. 

% \sysname enables users to rigorously \textit{wander} through their data by systematically supporting ``what-if" exploration, recommendation, and explanation tasks.
%\sysname allows users to perform rigorous ``what-if" exploration, get data-informed recommendation for decision-support, and explanation about the relationships among the features and performance target metrics. % navigating complex performance trade-offs to achieve \tzi{``good enough" (satisficing) configurations across user-defined performance criteria -- are we doing this? @Banooqa}. 
% Unlike purely predictive models that can only answer ``what will happen?", our framework explicitly models causal relationships, answering not only ``what" but also ``why will it happen?" and ``how can I change the outcome?" This causal understanding reduces susceptibility to spurious correlations, reducing uncertainty around a prediction and trustworthiness. %significantly improving decision quality and reliability.

We hypothesize that structured decision-support queries in HPC can be systematically categorized into four distinct classes—recommendation, modification, exploration (what-if), and discovery. Although real-world scenarios might involve combinations of these classes, our explicit assumption simplifies user interactions and enhances system generalizability. To formalize these query categories, we conducted an extensive review of recent HPC-related decision-support studies~\cite{leon2024comprehensive,chu2023how,cornelius2025extracting,mckerracher2025fresco,Eagle_Dataset_5860,antici2023pm100,antici2024f,patki2019performance,borghesi2019dataset_with, borghesi2019dataset_without,lockwood_2018_1345780, Loi2025Uncertainty, menear2024high, wang2020in, tanash2019high-performance, samsi2021mitsuperclouddataset, rodrigues2016resource}, guided by established principles from human-computer interaction (HCI) and explainable AI~\cite{amershi2019guidelines, doshi2017towards, kules2008designing}. Based on this review, we structured these query categories into reusable templates—a foundational contribution of this work. Future extensions of \sysname can readily accommodate combined or hierarchical query structures, facilitated by the framework’s modular design.
%
% This structured categorization provides a foundational contribution of this work, enabling \sysname to generalize to a broad spectrum of HPC decision-making scenarios. 
% \textbf{To our knowledge, this is the first such effort to characterize queries into classes, and such an open-source decision-support tool out there.}
% \tzi{This paragraph needs a lot of focused effort -- and is very important that we address it AS quickly as possible. @banooqa and @ankur}

One of the immediate challenges that needs to be addressed to realize such a tool is that HPC datasets are notoriously large. Thus, we hypothesize that intelligently prioritizing and sampling high-information or high-loss regions of the dataset, rather than uniformly processing all samples, can significantly reduce computational overhead while preserving the fidelity of downstream analysis. 
% \tzi{intelligently selecting the most informative samples} %intelligent subset sampling--strategically selecting only the most informative data--
% instead of using all samples can significantly reduce computational burdens without sacrificing accuracy in 
% capturing \tzi{complete -- can we quantify it is the complete model? what would that entail? If not, we may need to reconsider the use of this word} causal relationships downstream tasks. 
Our extensive evaluations across diverse datasets (Section~\ref{sec:subset-sampling-evaluation}) confirm that robust causal relationships can be accurately reconstructed using only a fraction of the available data.

% To rigorously evaluate \sysname, we introduce a novel methodology combining multiple metrics: predictive accuracy, uncertainty quantification, and causal modeling of relationships in data. This multi-dimensional evaluation, unprecedented in the~\gls{hpc} context, provides comprehensive insights into the reliability and robustness of generated recommendations. Particularly, the proposed causal-modeling-based evaluation methodology is innovative, offering a structured way to measure how well counterfactual scenarios maintain causal consistency. Although state-of-the-art predictive models can achieve high
% accuracy in forecasting outcomes, they can be misled by spurious correlations and hidden factors that influence performance. In contrast, causal inference methods are designed to account for hidden factors, providing accurate and trustworthy guidance when making decisions about \tzi{interventions -- this word needs to be changed to something that is well known in the hpc community and we will not introduce new words without defining them. @Banooqa}.
% Although \reco, \modify, and \whatif do not support straightforward prediction similar to what models such as XGBoost does, the \discover query is more informative than a straightforward supervised predictive model because it can quantify how much and which direction

Another challenge in leveraging a generative modeling formulation for decision-support is the trustworthiness of the suggestions without executing them. Without rigorous validation, quantified uncertainty, and interpretability, tools risk offering misleading recommendations that may lead to operational errors. To address this limitation, we introduce a multi-dimensional evaluation methodology that combines predictive accuracy, uncertainty quantification, causal modeling, and distributional alignment (Section~\ref{sec:evaluation-methodology}). This evaluation framework ensures that each generated suggestion is assessed for reliability and practical relevance. To further build trust, we validate \sysname’s discovered causal relationships against established findings from prior HPC studies in Section~\ref{sec:validation}.

Importantly, \sysname is explicitly not intended as a real-time scheduler nor a replacement for domain expertise. Rather, it serves as a transparent and trustworthy decision-support system highlighting performance trade-offs and quantifying risks associated with alternative configurations. By offering stakeholders multiple feasible and diverse configuration options—each accompanied by predictive outcomes and uncertainty quantifications—\sysname enables informed and robust operational decision-making.

To our knowledge, \sysname represents the first open-source, explainable, and scalable decision-support framework explicitly designed to address these critical gaps in HPC environments. Specifically, our contributions include:

\begin{itemize}
\item \textbf{Formalization}: Systematically categorizing HPC decision-support queries into recommendation, modification, exploration, and discovery.
\item \textbf{Intelligent Sample Acquisition}: Design a parallel algorithm for intelligently selecting samples %acquisition method 
for building performance model, which can reduce the data size up to 95\% while improving the downstream task's efficacy.
\item \textbf{Scalable Causal Modeling}: Developing a 
% novel, 
scalable causal inference method capable of analyzing datasets exceeding 
% \tzi{150GB and 13 million} 
$477$ million samples, quantifying impacts of configuration changes.
\item \textbf{Explaination and Interpretation}: Providing comprehensive, interpretable explanations for the configuration-performance relationships identified.
\item \textbf{Comprehensive Evaluation Framework}: Introducing a rigorous evaluation methodology integrating predictive accuracy, uncertainty quantification, causal graph validation, and distributional consistency metrics.
\item \textbf{Open-source Modular Framework}: Implementing and publicly releasing \sysname, a modular, extensible decision-support tool for various HPC stakeholders.
\item \textbf{Empirical Validation}: Demonstrating the efficacy, scalability, and generalizability of \sysname across diverse HPC datasets, validated against established causal relationships in existing literature.
\end{itemize}

Unlike traditional tools, \sysname does not prescribe a single ``best" configuration. Instead, it offers multiple diverse and feasible options--each paired with predicted outcomes and quantified uncertainties--to support robust decision-making. While future extensions could expand the backend to assist with code-level recommendations, tools like GitHub CoPilot~\cite{} already address that space effectively. The critical gap lies elsewhere: no existing system supports operational decision-making—how to set up the runtime environment, understand its effect on multiple performance metrics, and make informed choices based on that analysis. \sysname fills this gap.

\textbf{Limitations} \sysname deliberately excludes static pattern analysis and straightforward predictive modeling, as these tasks, while tractable, do not provide actionable suggestions directly, which is our primary goal. The current implementation supports numerical and categorical tabular performance profiles and telemetry data, leaving performance traces for future expansion. \sysname is motivated by the need for a portable, general-purpose framework for analysis and decision-making across diverse HPC workflows. By releasing \sysname on GitHub, we anticipate community-driven extensions to support specialized data types and niche decision-support needs in the HPC ecosystem.


% Formalizing two decision-making modes—prescriptive and exploratory—and mapping these modes to real-world HPC queries.

% Explaining how specific configuration changes impact performance outcomes through causal reasoning.
% Designing a novel evaluation approach, combining structural causal modeling, predictive accuracy, causal graph alignment, and uncertainty quantification.
% Implementing \sysname, a modular, open-source framework for scalable, causal-aware decision support.
% Demonstrating \sysname’s efficacy across multiple HPC datasets, highlighting its versatility and generalizability.
% Together, these contributions ensure \sysname supports informed, reliable, and interpretable HPC decision-making at scale for many stakeholders.

% While Wander provides recommendations based on historical data and causal structure, it is not a
% real-time scheduler, nor does it replace domain expertise. Rather, it serves as a decision-support tool that enables informed decision-making for various stakeholders by offering interpretable guidance,
% highlighting trade-offs, and quantifying the risks of alternative configurations. 
% It does not prescribe
% a single ``best" answer but offers multiple diverse, feasible options--each accompanied by predicted
% outcomes and uncertainty quantification. In future, the backend can be extended to also guide users for critical code-related decisions; however, there are already strong tools such as CoPilot~\cite{}, so the need for us to expand \sysname for that use case is not as critical. However, there is no tool for operational
% decision making (that is, how to set up the runtime environment of an application, how those
% impact multiple performance metrics, and based on that recommending users or software systems).

% \textbf{Limitations} Since \sysname focuses on supporting decision-making from data in a trustworthy manner, the query templates are limited to answering \textit{how} input changes affect outcomes. \sysname does not support pattern analysis or straightforward predictive modeling, as these options, albeit useful, offer limited value for decision support and can be trivial to implement outside the system. Another engineering limitation of \sysname is that in this first prototype, \sysname supports only numerical and categorical features in tabular data, excluding performance traces and timeseries data. , which are planned as future engineering extensions. The system will be open-sourced to enable community-driven expansion, including temporal modeling and scheduler integration. 

% \gls{hpc} systems are essential infrastructure for scientific advancement, powering large-scale simulations, data-intensive analyses, and modeling efforts across domains such as climate science, genomics, materials engineering, and astrophysics. These systems enable computations at scales that are otherwise infeasible due to the complexity and size of modern scientific workloads. However, effective utilization of~\gls{hpc} systems remains a challenge. As architectures become increasingly heterogeneous—with combinations of CPUs, GPUs, and specialized accelerators—operational decision-making becomes more complex. 


% Performance optimization now spans a high-dimensional configuration space, involving runtime parameters such as hardware selection, resource allocation, execution strategy, and power constraints.
% The impact of these decisions is nontrivial. Prior work has shown that a configuration that yields optimal performance in one scenario can cause up to $4\times$ variability under slightly different conditions~\cite{patki2019performance}. This makes "performance" not a single point objective, but a non-convex, multi-objective trade-off space, whose characteristics must be understood to make informed, robust decisions.

% We introduce~\sysname--\textit{What-if Analysis and Navigation for Decision-support with Explainable Reasoning}--a framework that guides various \gls{hpc} stakeholders including users and software systems through complex performance trade-offs by illuminating actionable configurations.


% % \tzi{The scope of this paper is operational decision-making, that is, how to configure runtime parameters such that their complex interactions with the performance characteristics of an application (modeled by a predictive performance model) can help an application achieve a satisficing trade-off space. So, some of those performance objectives may not be optimal, but as long as they are good enough, those will be recommended.}
% This paper focuses on operational decision-making: how to configure runtime parameters such that their interaction with an application's performance profile--modeled by predictive models--yields satisficing performance. % under multiple metrics. 
% A satisficing configuration is defined as any point within a user-defined region of acceptable performance based on user defined performance objectives such as runtime, power, or reliability thresholds. %We emphasize that optimality is not the goal in every case; instead, the system prioritizes good--enough solutions that are feasible, diverse, and explainable.

% \tzi{@Banooqa: The intro lacks the motivation that HPC datasets are huge and this size poses a challenge during exploration. If we do not do something about it, we cannot explore these datasets in a scalable manner. This will be your hook for intelligent data acquisition where you have to propose a hypothesis -- only X\% of data is needed to capture all relationships and our extensive evaluation in Section XYZ shows that across all 20 datasets, we were able to construct the exact same causal relationship with only upto X\% of data.}


% In the case of recommendations, the system prioritizes satisficing solutions—configurations that meet user-defined thresholds across multiple objectives without necessarily being optimal. However, the framework itself is not limited to satisficing; if users specify a particular trade-off or counterfactual target, \sysname simply returns the appropriate configuration. It is only when users request the ``best" configuration under multiple objectives that the problem is explicitly framed as a satisficing query.

% %As a result, \gls{hpc} practitioners are often left with limited tools to make informed decisions about how best to allocate, configure, or tune resources to meet performance goals.

% % Despite significant advances in performance modeling, scheduling algorithms, and auto-tuning frameworks, %current optimization strategies remain fragmented. Most existing approaches focus on predictive modeling or rule-based tuning in isolation, without integrating causal reasoning or 
% % there is a gap in existing literature about end-to-
% % end tools that can enable stakeholders such as users 
% % or software systems to simulate what-if scenarios. Such a tool can enable key stakeholders by answering 
% % questions such as ``What would happen if this job were run on GPUs instead of CPUs?" or ``Can energy consumption be reduced without degrading 
% % performance?" or ``How much should I change the \texttt{num of nodes} from $512$ to achieve a $10\%$ power consumption reduction?" Users often invest significant and repetitive efforts of building 
% % performance models and analysis tools applied to specific datasets to gain insights and then take decisions that require domain expertise to transform 
% % the insights into actionable outcome such as ``Change the number of nodes by $+x$ from $512$ to achieve $10\%$ power consumption reduction". However, this process can be repetitive and tailored to datasets, not generalizable, do not 
% %generate actionable recommendations that are grounded in the causal structure of the system, and that reflect the uncertainty inherent in \gls{hpc} environments. 
% % This disconnect between observational performance data and decision-making presents a significant gap in the current literature.
% Despite extensive literature in performance modeling, scheduling, and autotuning, there remains a gap in tools that enable end-to-end what-if exploration by both users and software systems. In the absence of such tools, users are often forced to repeatedly build ad hoc performance models, conduct analysis over specific datasets, and manually interpret outcomes—all of which require domain expertise and are difficult to generalize. This lack of systematized what-if reasoning leads to brittle, non-portable workflows that do not scale or adapt across workloads and platforms. Importantly, most existing tools fail to link observational performance data with \textbf{interventional decision support}--enabling users to simulate outcomes of changes before enacting them.

% To address this gap, we introduce \sysname, a decision-support tool that unifies predictive performance modeling, generative counterfactual reasoning, and query-driven recommendation within a single extensible framework. Unlike black-box predictors, \sysname is designed to simulate, explain, and quantify the outcomes of configuration changes by modeling the underlying causal structure of the system. \ankur{Predictive models which is typically built on supervised model are designed to identify the data pattern and correlation among the features to forecast future outcomes on given instances. This helps to answer "\textit{What will happen?}" instead of our seeking question - "\textit{Why has it happened?}". To solve this problem, causal analysis aims to identify the uncovered cause-and-effect relationships, focusing on "why" something happens and estimating the impact of interventions or treatments. The trade-off is important: while state-of-the-art predictive models can achieve high accuracy in forecasting outcomes, they are often misled by spurious correlations and confounding variables, which can result in recommendations that fail to address the true underlying causes. In contrast, causal inference methods are designed to account for hidden factors, providing more reliable guidance when making decisions about interventions. is often scarce in high-performance computing (HPC) environments or it requires domain experts to label manually(I will cite some hpc papers here)}

% \tzi{Why is it better than the predictive models people keep building using supervised learning? How is it better? Is there any gap in the existing modeling methods? Do they take a lot of data? Are they slow? Are they less acccurate? This is where you need to tell people about the gap and provide reasons why if we do not fill those gaps, the world will collapse.}


% \tzi{To address these gaps, }
% The framework allows users to ask diverse what-if questions across three core decision services:
% (1) Recommendation: ``What runtime configuration can meet a target performance goal?"
% (2) Prediction: ``What performance can I expect from a given configuration?"
% (3) Counterfactual reasoning: ``What minimal changes would yield an improved performance under a constraint?"


% % To bridge this gap, we introduce a novel framework--\sysname--that unifies predictive and generative performance modeling with counterfactual analysis for %recommendation generation 
% % studying ``what-if" scenarios
% % within a single, extensible tool. It is a decision-support tool. %system for \gls{hpc} environments. 
% % This query-driven framework enables stakeholders, both users and software systems, to ask complex what-if questions that commonly occur in scenarios pertaining to running jobs: modeling, \tzi{recommendation - we could get rid of it and formulate it as counterfactual without an initial input }, and counterfactuals.  %such as: What if we allocated more GPUs to this job? or What configuration would minimize runtime under a power budget?
% % In addition to evaluating the responses of the framework using state-of-the-art methods, in this paper, we propose a novel evaluation method using structural causal models to both statistically and mathematically ensure the robustness of the generated samples as well as quantify the confidence of the responses so that users can make informed decision.
% %What is missing here?
% % and powered by counterfactual generation techniques adapted for \gls{hpc} constraints, the tool translates historical workload traces into simulated outcomes, offering interpretable, reliable, and uncertainty-aware recommendations. Unlike black-box predictors, this system not only forecasts outcomes, but quantifies the confidence of its predictions and explains the why behind its suggestions.

% % The need for such a tool is especially urgent as \gls{hpc} systems continue to scale. Power budgets are becoming as critical as runtime in defining success metrics, and \gls{hpc} users--ranging from application scientists to system administrators--face increasing pressure to make data-driven, high-stakes decisions about job scheduling, hardware allocation, and performance tuning. 

% % TZI : Need to revise this and tie to a dataset rther than random stuff. 
% To illustrate the capabilities of~\sysname, we use an example focused on a scientific simulation running on a heterogeneous cluster. A user investigates how increasing the number of compute nodes \texttt{num\_node} from a base configuration to a certain number might influence \texttt{node\_power\_consumption}. The objective of this investigation is to estimate whether scaling up resources can reduce overall runtime without exceeding the predefined energy or power constraints. This example threads through the paper, showcasing how modeling, counterfactual reasoning, and recommendation converge to produce actionable decisions.


% % A user investigates how adjusting the number of threads per core, modifying thread affinity (binding policy), or switching from CPU to GPU execution under a 150W power cap might reduce runtime without violating energy constraints (\tzi{PM100 or Fugaku dataset}). %

% \sysname is designed to support flexible system integration. It can serve end-users directly, helping scientists and engineers reason about how to run their jobs. At the same time, the API layer can be detached and integrated into job schedulers or workflow orchestrators, enabling automated decision support in larger \gls{hpc} pipelines. Although the current implementation focuses on individual job-level decisions, the architecture can be extended to reason about site-wide or even cross-site optimization strategies. However, we note that we currently lack datasets to explore the latter scenarios.


% To increase trust , interpretability and accountability, we propose a novel evaluation methodology using structural causal models (SCMs) that assess the robustness and internal consistency of generated counterfactuals. In addition, we implement ensemble-based uncertainty quantification, allowing the system to present confidence intervals for each recommended configuration. Furthermore we incorporate outlier detection to find out how our method is prone to the accountability. Together, these mechanisms enable risk-aware, transparent decision-making for both users and automated systems.

% Instead of targeting specific user roles, \sysname organizes functionality around three query types that cut across stakeholder categories: (1) Recommendation queries support users seeking feasible runtime configurations to meet performance thresholds.
% (2) Prediction queries allow system administrators to simulate the impact of policy changes on center-wide throughput or power efficiency.
% (3) Counterfactual queries assist stakeholders in reasoning about alternate configurations to improve past performance outcomes.


% %%%%%%%%%%% Instead of roles, I think better if we revise them to be the three types of queries.
% Our tool is designed to support these diverse scenarios:
% (1) Application scientists can explore how to run their job, what type of configurations they should use to achieve certain threshold (recommendation), (2) System administrators and center managers can explore site-wide policies and predict their impact on the overall throughput of their \gls{hpc} facilities (explore and predict), (3) stakeholders can explore ``what-if" scenarios by asking the tool about how to change their previous decisions to achieve a performance objective (counterfactual).
% Performance engineers can test tuning strategies, evaluate trade-offs between energy and performance, and experiment with hypothetical deployment scenarios without risking production instability. The same tool could also be used in an educational environment for training the next-generation computational scientists by enabling them to learn about relationships across many operational parameters and how those impact performance trade-off to provide with initial idea. They do not have to be experts to start using an \gls{hpc} system efficiently.

% While~\sysname provides recommendations based on historical data and causal structure, it is not a real-time scheduler, nor does it replace domain expertise. Rather, it serves as a decision-support tool that enables informed decision-making for various stakeholders by offering interpretable guidance, highlighting trade-offs, and quantifying the risks of alternative configurations. It does not prescribe a single ``best'' answer but offers multiple diverse, feasible options--each accompanied by predicted outcomes and confidence levels. Moreover, currently~\sysname is only used for operational decisions such as how to run a job. In future, the backend can be extended to also guide users for critical code-related decisions; however, there are already strong tools such as CoPilot etc., so the need for us to expand our tool for that use case is not as critical. However, there is no tool for operational decision making (that is, how to set up the runtime environment of an application, how those impact multiple performance metrics, and based on that recommending users or software systems).

% \noindent The key contributions of this paper are:

% \begin{itemize}
%     \item \textbf{Formalize} two decision-making modes—\emph{prescriptive} and \emph{exploratory}—and map common \gls{hpc} configuration queries to these services.

%     \item \textbf{Explain} how and why certain configuration changes influence performance outcomes.

%     \item \textbf{Design} a novel evaluation methodology that combines structural causal modeling, predictive accuracy, causal graph alignment, and uncertainty quantification to assess the trustworthiness of decisions.

%     \item \textbf{Implement} \sysname, a modular decision-support framework, which will be open-sourced.

%     % \item \textbf{Extend} counterfactual search to support feasibility constraints, Pareto optimization, and diversity filtering.

%     % \item \textbf{Develop} an evaluation protocol combining SEM, predictive accuracy, and causal graph alignment.

%     \item \textbf{Demonstrate} \sysname across multiple \gls{hpc} datasets, enabling varied performance decisions through a unified interface.
% \end{itemize}

% \begin{itemize}
%     \item What is the need. What will happen if we do not do this work. A novel methodology for enabling what-if exploration for HPC using generative AI (defining the types of questions that people in HPC ask form the perspective of HCI, Table 1, Methodology)
%     \item \tzi{Scalable causal model construction.} Why is it a necessary step? What will happen if we did not make causal model construction scalable? For the explanation query, we need to build a causal model, explain the causal relationships, their influences, and a story behind it using LLM and present that. It bi-passes DiCE and other evaluation steps. For this step, we need to add an evaluation that shows how large of a dataset we can scale to. Fugaku has many parquet files. Each has 720K samples, I believe. We can continue adding more parquet and show that we can scale up to a million sample dataset. OR, scale both samples and columns.
%     \item Extracting rules from LLMs -- why is it a needed step? What will happen if you did not add this step? This will have major time overhead -- we need to justify why that step is worth the price. Then we need to add an evaluation that compares counterfactual qualities between using rule-based pruning vs not using rule-based pruning for all datasets. Did the fine-grained and/or coarse-grained sample quality improve if we use rules vs not? Is it worth paying the prices?
%     \item An extendable and programmable framework called \sysname for HPC datasets that supports both making decisions about a single or multiple target metrics (\tzi{Multi-target: SCM/Dice+SciKitlearn multioutput {assuming the targets are of the same types})}. You describe (a) single target exploration (b) multi-target (c) classification. 
%     \item A novel methodology for evaluating synthesized recommendations (1) fine-grained evaluation (per recommendation-based) -- UQ+regression for each sample (2) coarse-grained evaluation (per batch of synthesized recommendation based) -- (a) violin chart (average KL divergence), (b) Graph comparison --> what is needed is to convert them to a numerical similarity distance (0.5+-0.001\%, 0.9+-0.001\%, 0.7+-0.1\%) \banooqa{evaluating if the semantic relationships among the features are being preserved in the counterfactual data}. Clearly explain your test partition, and train partition, what are you building the ground truth from for evaluation, and emphasize using contrastive language that there is NO data leaking.  
%     %How to come up with a score with confidence interval for each counterfactual (or whatever other ideas oyu may have) where we can combine (1) distribution similarity (violin chart), (2) UQ chart (generate a score for each sample) (3) graph comparison (4) GAN-based discriminatory distance.  
% \end{itemize}

% % \tzi{To concretely explain the templates, we use a running example of optimizing a scientific simulation on a heterogeneous CPU-GPU cluster. This example runs through the paper and illustrates how each component---modeling, counterfactual generation, and recommendation ranking---contributes to an optimization workflow. For instance, the example demonstrates how switching from CPU to GPU execution under certain conditions not only improves runtime but also reduces energy consumption, highlighting the importance of context-aware, counterfactual-driven decision support. - Made up - need to replace with what example we plan to use.}


% % In summary, this paper addresses a critical need in \gls{hpc} by introducing a unified reasoning framework tailored for the unique challenges of heterogeneous multi-objective environments. Through the integration of causal inference, what-if simulation, and stakeholder-centered recommendations,~\sysname lays the foundation for a community-driven tool for efficient application performance and resource utilization in \gls{hpc}. 



==> Sections/intro.tex <==
\gls{hpc} systems are essential infrastructure for scientific advancement, powering large-scale simulations, data-intensive analyses, and modeling efforts across domains such as climate science, genomics, materials engineering, and astrophysics. These systems enable computations at scales that are otherwise infeasible due to the complexity and size of modern scientific workloads. However, effective utilization of~\gls{hpc} systems remains a challenge. As architectures become increasingly heterogeneous—with combinations of CPUs, GPUs, and specialized accelerators—operational decision-making becomes more complex. 


Performance optimization now spans a high-dimensional configuration space, involving runtime parameters such as hardware selection, resource allocation, execution strategy, and power constraints.
The impact of these decisions is nontrivial. Prior work has shown that a configuration that yields optimal performance in one scenario can cause up to $4\times$ variability under slightly different conditions~\cite{patki2019performance}. This makes "performance" not a single point objective, but a non-convex, multi-objective trade-off space, whose characteristics must be understood to make informed, robust decisions.

We introduce~\sysname--\textit{What-if Analysis and Navigation for Decision-support with Explainable Reasoning}--a framework that guides various \gls{hpc} stakeholders including users and software systems through complex performance trade-offs by illuminating actionable configurations.


% \tzi{The scope of this paper is operational decision-making, that is, how to configure runtime parameters such that their complex interactions with the performance characteristics of an application (modeled by a predictive performance model) can help an application achieve a satisficing trade-off space. So, some of those performance objectives may not be optimal, but as long as they are good enough, those will be recommended.}
This paper focuses on operational decision-making: how to configure runtime parameters such that their interaction with an application's performance profile--modeled by predictive models--yields satisficing performance. % under multiple metrics. 
A satisficing configuration is defined as any point within a user-defined region of acceptable performance based on user defined performance objectives such as runtime, power, or reliability thresholds. %We emphasize that optimality is not the goal in every case; instead, the system prioritizes good--enough solutions that are feasible, diverse, and explainable.

\tzi{@Banooqa: The intro lacks the motivation that HPC datasets are huge and this size poses a challenge during exploration. If we do not do something about it, we cannot explore these datasets in a scalable manner. This will be your hook for intelligent data acquisition where you have to propose a hypothesis -- only X\% of data is needed to capture all relationships and our extensive evaluation in Section XYZ shows that across all 20 datasets, we were able to construct the exact same causal relationship with only upto X\% of data.}


In the case of recommendations, the system prioritizes satisficing solutions—configurations that meet user-defined thresholds across multiple objectives without necessarily being optimal. However, the framework itself is not limited to satisficing; if users specify a particular trade-off or counterfactual target, \sysname simply returns the appropriate configuration. It is only when users request the ``best" configuration under multiple objectives that the problem is explicitly framed as a satisficing query.

%As a result, \gls{hpc} practitioners are often left with limited tools to make informed decisions about how best to allocate, configure, or tune resources to meet performance goals.

% Despite significant advances in performance modeling, scheduling algorithms, and auto-tuning frameworks, %current optimization strategies remain fragmented. Most existing approaches focus on predictive modeling or rule-based tuning in isolation, without integrating causal reasoning or 
% there is a gap in existing literature about end-to-
% end tools that can enable stakeholders such as users 
% or software systems to simulate what-if scenarios. Such a tool can enable key stakeholders by answering 
% questions such as ``What would happen if this job were run on GPUs instead of CPUs?" or ``Can energy consumption be reduced without degrading 
% performance?" or ``How much should I change the \texttt{num of nodes} from $512$ to achieve a $10\%$ power consumption reduction?" Users often invest significant and repetitive efforts of building 
% performance models and analysis tools applied to specific datasets to gain insights and then take decisions that require domain expertise to transform 
% the insights into actionable outcome such as ``Change the number of nodes by $+x$ from $512$ to achieve $10\%$ power consumption reduction". However, this process can be repetitive and tailored to datasets, not generalizable, do not 
%generate actionable recommendations that are grounded in the causal structure of the system, and that reflect the uncertainty inherent in \gls{hpc} environments. 
% This disconnect between observational performance data and decision-making presents a significant gap in the current literature.
Despite extensive literature in performance modeling, scheduling, and autotuning, there remains a gap in tools that enable end-to-end what-if exploration by both users and software systems. In the absence of such tools, users are often forced to repeatedly build ad hoc performance models, conduct analysis over specific datasets, and manually interpret outcomes—all of which require domain expertise and are difficult to generalize. This lack of systematized what-if reasoning leads to brittle, non-portable workflows that do not scale or adapt across workloads and platforms. Importantly, most existing tools fail to link observational performance data with \textbf{interventional decision support}--enabling users to simulate outcomes of changes before enacting them.

To address this gap, we introduce \sysname, a decision-support tool that unifies predictive performance modeling, generative counterfactual reasoning, and query-driven recommendation within a single extensible framework. Unlike black-box predictors, \sysname is designed to simulate, explain, and quantify the outcomes of configuration changes by modeling the underlying causal structure of the system. \ankur{Predictive models which is typically built on supervised model are designed to identify the data pattern and correlation among the features to forecast future outcomes on given instances. This helps to answer "\textit{What will happen?}" instead of our seeking question - "\textit{Why has it happened?}". To solve this problem, causal analysis aims to identify the uncovered cause-and-effect relationships, focusing on "why" something happens and estimating the impact of interventions or treatments. The trade-off is important: while state-of-the-art predictive models can achieve high accuracy in forecasting outcomes, they are often misled by spurious correlations and confounding variables, which can result in recommendations that fail to address the true underlying causes. In contrast, causal inference methods are designed to account for hidden factors, providing more reliable guidance when making decisions about interventions. is often scarce in high-performance computing (HPC) environments or it requires domain experts to label manually(I will cite some hpc papers here)}

\tzi{Why is it better than the predictive models people keep building using supervised learning? How is it better? Is there any gap in the existing modeling methods? Do they take a lot of data? Are they slow? Are they less acccurate? This is where you need to tell people about the gap and provide reasons why if we do not fill those gaps, the world will collapse.}


\tzi{To address these gaps, }
The framework allows users to ask diverse what-if questions across three core decision services:
(1) Recommendation: ``What runtime configuration can meet a target performance goal?"
(2) Prediction: ``What performance can I expect from a given configuration?"
(3) Counterfactual reasoning: ``What minimal changes would yield an improved performance under a constraint?"


% To bridge this gap, we introduce a novel framework--\sysname--that unifies predictive and generative performance modeling with counterfactual analysis for %recommendation generation 
% studying ``what-if" scenarios
% within a single, extensible tool. It is a decision-support tool. %system for \gls{hpc} environments. 
% This query-driven framework enables stakeholders, both users and software systems, to ask complex what-if questions that commonly occur in scenarios pertaining to running jobs: modeling, \tzi{recommendation - we could get rid of it and formulate it as counterfactual without an initial input }, and counterfactuals.  %such as: What if we allocated more GPUs to this job? or What configuration would minimize runtime under a power budget?
% In addition to evaluating the responses of the framework using state-of-the-art methods, in this paper, we propose a novel evaluation method using structural causal models to both statistically and mathematically ensure the robustness of the generated samples as well as quantify the confidence of the responses so that users can make informed decision.
%What is missing here?
% and powered by counterfactual generation techniques adapted for \gls{hpc} constraints, the tool translates historical workload traces into simulated outcomes, offering interpretable, reliable, and uncertainty-aware recommendations. Unlike black-box predictors, this system not only forecasts outcomes, but quantifies the confidence of its predictions and explains the why behind its suggestions.

% The need for such a tool is especially urgent as \gls{hpc} systems continue to scale. Power budgets are becoming as critical as runtime in defining success metrics, and \gls{hpc} users--ranging from application scientists to system administrators--face increasing pressure to make data-driven, high-stakes decisions about job scheduling, hardware allocation, and performance tuning. 

% TZI : Need to revise this and tie to a dataset rther than random stuff. 
To illustrate the capabilities of~\sysname, we use an example focused on a scientific simulation running on a heterogeneous cluster. A user investigates how increasing the number of compute nodes \texttt{num\_node} from a base configuration to a certain number might influence \texttt{node\_power\_consumption}. The objective of this investigation is to estimate whether scaling up resources can reduce overall runtime without exceeding the predefined energy or power constraints. This example threads through the paper, showcasing how modeling, counterfactual reasoning, and recommendation converge to produce actionable decisions.


% A user investigates how adjusting the number of threads per core, modifying thread affinity (binding policy), or switching from CPU to GPU execution under a 150W power cap might reduce runtime without violating energy constraints (\tzi{PM100 or Fugaku dataset}). %

\sysname is designed to support flexible system integration. It can serve end-users directly, helping scientists and engineers reason about how to run their jobs. At the same time, the API layer can be detached and integrated into job schedulers or workflow orchestrators, enabling automated decision support in larger \gls{hpc} pipelines. Although the current implementation focuses on individual job-level decisions, the architecture can be extended to reason about site-wide or even cross-site optimization strategies. However, we note that we currently lack datasets to explore the latter scenarios.


To increase trust , interpretability and accountability, we propose a novel evaluation methodology using structural causal models (SCMs) that assess the robustness and internal consistency of generated counterfactuals. In addition, we implement ensemble-based uncertainty quantification, allowing the system to present confidence intervals for each recommended configuration. Furthermore we incorporate outlier detection to find out how our method is prone to the accountability. Together, these mechanisms enable risk-aware, transparent decision-making for both users and automated systems.

Instead of targeting specific user roles, \sysname organizes functionality around three query types that cut across stakeholder categories: (1) Recommendation queries support users seeking feasible runtime configurations to meet performance thresholds.
(2) Prediction queries allow system administrators to simulate the impact of policy changes on center-wide throughput or power efficiency.
(3) Counterfactual queries assist stakeholders in reasoning about alternate configurations to improve past performance outcomes.


%%%%%%%%%%% Instead of roles, I think better if we revise them to be the three types of queries.
Our tool is designed to support these diverse scenarios:
(1) Application scientists can explore how to run their job, what type of configurations they should use to achieve certain threshold (recommendation), (2) System administrators and center managers can explore site-wide policies and predict their impact on the overall throughput of their \gls{hpc} facilities (explore and predict), (3) stakeholders can explore ``what-if" scenarios by asking the tool about how to change their previous decisions to achieve a performance objective (counterfactual).
Performance engineers can test tuning strategies, evaluate trade-offs between energy and performance, and experiment with hypothetical deployment scenarios without risking production instability. The same tool could also be used in an educational environment for training the next-generation computational scientists by enabling them to learn about relationships across many operational parameters and how those impact performance trade-off to provide with initial idea. They do not have to be experts to start using an \gls{hpc} system efficiently.

While~\sysname provides recommendations based on historical data and causal structure, it is not a real-time scheduler, nor does it replace domain expertise. Rather, it serves as a decision-support tool that enables informed decision-making for various stakeholders by offering interpretable guidance, highlighting trade-offs, and quantifying the risks of alternative configurations. It does not prescribe a single ``best'' answer but offers multiple diverse, feasible options--each accompanied by predicted outcomes and confidence levels. Moreover, currently~\sysname is only used for operational decisions such as how to run a job. In future, the backend can be extended to also guide users for critical code-related decisions; however, there are already strong tools such as CoPilot etc., so the need for us to expand our tool for that use case is not as critical. However, there is no tool for operational decision making (that is, how to set up the runtime environment of an application, how those impact multiple performance metrics, and based on that recommending users or software systems).

\noindent The key contributions of this paper are:

\begin{itemize}
    \item \textbf{Formalize} two decision-making modes—\emph{prescriptive} and \emph{exploratory}—and map common \gls{hpc} configuration queries to these services.

    \item \textbf{Explain} how and why certain configuration changes influence performance outcomes.

    \item \textbf{Design} a novel evaluation methodology that combines structural causal modeling, predictive accuracy, causal graph alignment, and uncertainty quantification to assess the trustworthiness of decisions.

    \item \textbf{Implement} \sysname, a modular decision-support framework, which will be open-sourced.

    % \item \textbf{Extend} counterfactual search to support feasibility constraints, Pareto optimization, and diversity filtering.

    % \item \textbf{Develop} an evaluation protocol combining SEM, predictive accuracy, and causal graph alignment.

    \item \textbf{Demonstrate} \sysname across multiple \gls{hpc} datasets, enabling varied performance decisions through a unified interface.
\end{itemize}

\begin{itemize}
    \item What is the need. What will happen if we do not do this work. A novel methodology for enabling what-if exploration for HPC using generative AI (defining the types of questions that people in HPC ask form the perspective of HCI, Table 1, Methodology)
    \item \tzi{Scalable causal model construction.} Why is it a necessary step? What will happen if we did not make causal model construction scalable? For the explanation query, we need to build a causal model, explain the causal relationships, their influences, and a story behind it using LLM and present that. It bi-passes DiCE and other evaluation steps. For this step, we need to add an evaluation that shows how large of a dataset we can scale to. Fugaku has many parquet files. Each has 720K samples, I believe. We can continue adding more parquet and show that we can scale up to a million sample dataset. OR, scale both samples and columns.
    \item Extracting rules from LLMs -- why is it a needed step? What will happen if you did not add this step? This will have major time overhead -- we need to justify why that step is worth the price. Then we need to add an evaluation that compares counterfactual qualities between using rule-based pruning vs not using rule-based pruning for all datasets. Did the fine-grained and/or coarse-grained sample quality improve if we use rules vs not? Is it worth paying the prices?
    \item An extendable and programmable framework called \sysname for HPC datasets that supports both making decisions about a single or multiple target metrics (\tzi{Multi-target: SCM/Dice+SciKitlearn multioutput {assuming the targets are of the same types})}. You describe (a) single target exploration (b) multi-target (c) classification. 
    \item A novel methodology for evaluating synthesized recommendations (1) fine-grained evaluation (per recommendation-based) -- UQ+regression for each sample (2) coarse-grained evaluation (per batch of synthesized recommendation based) -- (a) violin chart (average KL divergence), (b) Graph comparison --> what is needed is to convert them to a numerical similarity distance (0.5+-0.001\%, 0.9+-0.001\%, 0.7+-0.1\%) \banooqa{evaluating if the semantic relationships among the features are being preserved in the counterfactual data}. Clearly explain your test partition, and train partition, what are you building the ground truth from for evaluation, and emphasize using contrastive language that there is NO data leaking.  
    %How to come up with a score with confidence interval for each counterfactual (or whatever other ideas oyu may have) where we can combine (1) distribution similarity (violin chart), (2) UQ chart (generate a score for each sample) (3) graph comparison (4) GAN-based discriminatory distance.  
\end{itemize}

% \tzi{To concretely explain the templates, we use a running example of optimizing a scientific simulation on a heterogeneous CPU-GPU cluster. This example runs through the paper and illustrates how each component---modeling, counterfactual generation, and recommendation ranking---contributes to an optimization workflow. For instance, the example demonstrates how switching from CPU to GPU execution under certain conditions not only improves runtime but also reduces energy consumption, highlighting the importance of context-aware, counterfactual-driven decision support. - Made up - need to replace with what example we plan to use.}


% In summary, this paper addresses a critical need in \gls{hpc} by introducing a unified reasoning framework tailored for the unique challenges of heterogeneous multi-objective environments. Through the integration of causal inference, what-if simulation, and stakeholder-centered recommendations,~\sysname lays the foundation for a community-driven tool for efficient application performance and resource utilization in \gls{hpc}. 



==> Sections/intro2.tex <==
\gls{hpc} systems are essential infrastructure for scientific advancement, powering large-scale simulations, data-intensive analyses, and modeling efforts across domains such as climate science, genomics, materials engineering, and astrophysics. These systems enable computations at scales that are otherwise infeasible due to the complexity and size of modern scientific workloads. However, effective utilization of~\gls{hpc} systems remains a challenge. As architectures become increasingly heterogeneous—with combinations of CPUs, GPUs, and specialized accelerators—operational decision-making becomes more complex. 

High-performance computing (HPC) systems expose numerous interdependent parameters (knobs) influencing metrics such as execution time, energy consumption, resource utilization, and run-to-run variability. These parameters form a high-dimensional configuration space with complex, nonlinear interactions. Prior studies have demonstrated that a seemingly optimal configuration can lead to performance variability as high as \(4\times\) under slightly different conditions~\cite{patki2019performance}. Consequently, performance in HPC is not a single point objective but a multi-objective, non-convex trade-off space. Traditional tuning, relying on expert intuition or extensive trial-and-error, struggles to navigate this complexity. Data-driven predictive models, such as GPTune~\cite{wu2021gptune} and OpenTuner~\cite{ansel2014opentuner}, alleviate some burden by selecting configurations from historical data. However, these ``black-box'' tools predominantly find singular optimal solutions, neglecting systematic exploration and interpretability, which users critically need to understand trade-offs and to confidently navigate HPC configuration choices.

Exploring hypothetical ``what-if" scenarios enables users to examine how configuration changes affect HPC performance metrics. Such analyses allow users to manage performance trade-offs, avoid configurations associated with anomalies or high variability, and select suitable alternatives for critical workloads. Existing frameworks like GPTune~\cite{wu2021gptune}, OpenTuner~\cite{ansel2014opentuner}, and ATF~\cite{rasley2016atf} primarily identify single optimal configurations and do not systematically support alternative scenario exploration. Users typically rely on custom scripts or manual analysis, which can be labor-intensive and limited in scope. Additionally, the black-box nature of predictive models creates uncertainty about recommendation reliability, causing hesitation in adopting machine-generated configurations. Addressing this gap requires quantifying prediction uncertainties, validating configurations against historical causal patterns, and clearly communicating trade-offs.

To address these gaps, we propose~\sysname--\textit{What-if Analysis and Navigation for Decision-support with Explainable Reasoning}, an explainable, structured decision-support framework designed to enable systematic exploration of hypothetical configurations in HPC environments. At its core, \sysname synthesizes configurations minimally modified from user-specified baselines (called counterfactuals) to achieve desired performance goals or avoid undesirable outcomes. Unlike existing autotuning methods that output single, non-interpretable optimal configurations, \sysname explicitly supports exploratory queries such as ``Given an initial configuration, what would happen to runtime if I doubled the GPU count?" or ``Given an initial configuration, what minimal changes could prevent node failures due to memory exhaustion?"



==> Sections/loss_comparison_table.tex <==
% \begin{table*}[t]
% \centering
% \caption{Comparison of Counterfactual Generation Methods}
% \label{tab:comparison}
% \begin{tabular}{llcccccc}
% \toprule
% \textbf{Dataset} & \textbf{Configuration} & \textbf{Validity} $\uparrow$ &
% \textbf{Dist. Center}$\downarrow$ & \textbf{Robustness} $\uparrow$ &
% \textbf{Proximity} $\downarrow$ & \textbf{Sparsity}$\downarrow$ &
% \textbf{Diversity} $\uparrow$ \\
% \midrule
% \multirow{4}{*}{Dataset1}
%  & Baseline & 0.800 & 3.245 & 0.652 & 5.234 & 3.5 & 4.123 \\
%  & Mid-Boundary Only & 0.900 & \textbf{1.523} & 0.758 & 5.567 & 3.8 & 4.456 \\
%  % & Robustness Only & 0.900 & 3.012 & \textbf{0.851} & 5.789 & 4.2 & 4.789 \\
%  % & Both (Proposed) & \textbf{1.000} & 1.234 & 0.920 &
%  \textbf{5.234} & \textbf{3.5} & \textbf{5.012} \\
% \bottomrule
% \end{tabular}
% \end{table*}
\begin{table}[t]
\centering
\caption{MAPE Comparison Across Configurations}
\label{tab:comparison}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{p{2.2cm} p{4.5cm} p{1.8cm}}
\toprule
\textbf{Dataset} & \textbf{Configuration} & \textbf{MAPE} $\downarrow$ \\
\midrule
\multirow{3}{*}{Dataset1}
 & Baseline & 3.245 \\
 & Mid-Boundary Only & \textbf{1.523} \\
 & Both (Proposed) & 1.234 \\
\bottomrule
\end{tabular}
}
\end{table}


==> Sections/notes.tex <==
\begin{itemize}
    \item How many datasets are we considering. PM100, F-DATA, Monet, Batter-E, MIT Supercloud or Blue Waters
    \item Three things we must convince reviewers of: (1) novelty in methodology (2) Novel observations. (3) We need to establish ``We are the best -- most accurate, most scalable, look this evaluation method enabled us to do something that the state of the art methods (evaluation method, metric, counterfactual tricks, subsampling) did not catch those new observations/did not let us do what we can do now. 
    \item Does the end to end pipeline work? Yes, both GUI and CLI versions work.
    Task 1: Which Branch has the entire code integrated and push this to GitHub.
    \item Overhead -- 
    \item What is our hypothesis and when can we say that "Woohoo we are successful"?
    \item Apply data acquisition to MIT supercloud or Blue waters?
    \item GUI: (1) Add ``Explanation" as an option. The GUI will have is the Sankey and an English language  
\end{itemize}

% \begin{table*}[t]
% \begin{singlespacing}
% \centering
% \caption{Unified View of Decision-Support Query Types with Templates, HPC Use Cases, and Dataset Features}
% \label{tab:query-taxonomy-expanded}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{p{0.15\linewidth} p{0.22\linewidth} p{0.27\linewidth} p{0.18\linewidth} p{0.18\linewidth}}
% \toprule
% \textbf{Query Type} & \textbf{Query Template} & \textbf{HPC Use Cases with Example Queries} & \textbf{Example Features} & \textbf{Example Performance Metrics} \\
% \midrule
% Prescriptive & What values of \texttt{<configuration parameters>} will ensure \texttt{<performance targets>} remain under \texttt{<constraints>}? & 
% \textit{Suggest settings for runtime < 30s and power < 80W} & 
% \texttt{num\_nodes}, \texttt{num\_gpus}, \texttt{freq\_alloc} (Fugaku, PM100) & 
% \texttt{runtime}, \texttt{power\_draw}, \texttt{energy\_consumption} \\
% \hline

% Exploratory What-If & If I change \texttt{<parameter>} to \texttt{<value>}, how will it affect \texttt{<performance metric>}? & 
% \textit{What happens to runtime if I increase nodes from 2 to 4?} \newline 
% \textit{What happens to runtime variability if I change the available bandwidth?} & 
% \texttt{num\_nodes}, \texttt{mbwidth}, \texttt{mem\_alloc} (Fugaku, PM100) & 
% \texttt{runtime}, \texttt{runtime\_std}, \texttt{job\_throughput} \\
% \hline

% Exploratory Optimization & What changes to \texttt{<parameter>} would help reduce \texttt{<metric>} by \texttt{<amount>} or reach \texttt{<target>}? & 
% \textit{How to reduce energy usage by 20\% for my job?} \newline 
% \textit{How to reduce runtime std. while keeping mean runtime under 30s?} & 
% \texttt{num\_nodes}, \texttt{mem\_alloc}, \texttt{bandwidth} (PerfVar) & 
% \texttt{energy\_consumption}, \texttt{runtime\_std}, \texttt{duration} \\
% \hline


% Failure Avoidance & What changes to \texttt{<configuration>} would have prevented this job from failing? & 
% \textit{What resource request change would avoid node failure?} \newline 
% \textit{What prevents GPU exhaustion?} & 
% \texttt{AllocCPUS}, \texttt{is\_gpu}, \texttt{req\_mem} (HotCloudPerf'23) & 
% \texttt{job\_status}, \texttt{failure\_indicator} \\
% \hline

% Explanation & Which parameters most influenced the outcome of \texttt{<metric>} for this configuration? & 
% \textit{Why did memory bandwidth drive runtime variability?} & 
% \texttt{mem\_alloc}, \texttt{mbwidth}, \texttt{freq\_alloc} (PM100, Fugaku, PerfVar) & 
% \texttt{runtime}, \texttt{runtime\_std}, \texttt{power\_usage} \\
% \bottomrule
% \end{tabular}
% }
% \end{singlespacing}
% \end{table*}

==> Sections/query_map_table1.tex <==
\begin{table}[t]
\small
% \renewcommand{\arraystretch}{1}  
% \setlength{\tabcolsep}{1pt}
% \captionsetup{skip=-2pt}              
\caption{Summary of query templates prevalent in HPC decision-support scenarios.}
\label{tab:query-templates}
\begin{singlespacing}
% \begin{center}
\resizebox{\columnwidth}{!}{   
\tiny
\begin{tabular}{|p{1.5cm}|p{1cm}|p{1.5cm}|}
\hline

\textbf{Intent \& HPC Scenarios} & \textbf{Template}  &\textbf{Input \& Output}
% &\textbf{HPC Scenarios}
\\
\hline
\hline

% \textbf{\parbox{1.2cm}{Recommend}}
% &
\multicolumn{3}{|c|}{{\tablecellbl{\textbf{\reco}}}}\\\hline
\cell{
Given target objectives $Y$, find values of $X_{user}$ to meet those objectives (Inverse problem) on given optional constraints $C$.
Novice HPC users; Software systems such as job schedulers, resource managers, HPC facilities.}
&
\cell{
\tightcell{
\textcolor{blue}{\textbf{Recommend a configuration}} $X = \{ x_i:?\}$ \textcolor{blue}{\textbf{to achieve}} $Y\!=\!\{y_1:\!\mathcal{O}_1, \dots, y_m:\!\mathcal{O}_m\}$ \textbf{\textcolor{blue}{where}} $C$ = \{x_j\!:\!v_i\}} 
}
&
\cell{\textbf{User provides:} Objective(s) over $Y$ and optional constraints on $X$, specifying configurable parameters $X_{\text{user}}$.
\textbf{Compass responds:} Candidate configurations $\mathcal{X}_{\text{user}}$ conditioned on the empirical distribution of $\mathcal{X}_{\text{sys}}$ observed from historical jobs satisfying the same constraints.}
% \cell{Objective(s) over $Y$, optionally some constraints on $X$, without initial configuration. By specifying $X_{user}$, user provides domain knowledge of what is configurable.}
% % &
% \cell{Compass suggests $\mathcal{X}_{\text{user}}$ conditioned on the empirical distribution of $\mathcal{X}_{\text{sys}}$ observed across historical jobs that share the same constraint set.}
% & 
% \cell{Novice HPC users; Software systems such as job schedulers, resource managers, HPC facilities.}
\\

\hline
% \cline{1-3} \cline{5-10}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{3}{|c|}{{\tablecellgr{\textbf{\modify}}}}\\\hline
% &
\cell{
Given desired outcomes $Y$ and an initial configuration, update existing $X_{user}$ with minimal changes (Counterfactual reasoning).
Autotuners; Performance tuning.}
& 
\cell{
\tightcell{
\textcolor{blue}{\textbf{Reconfigure}}  
$X = \{x_1:v_1^{old}\rightarrow~v_1^{new}, \dots, x_n: v_n^{old} \rightarrow ?\}$
\textcolor{blue}{\textbf{to achieve}}
$Y$ = $\{y_j:v_j^{old}\rightarrow~v_j^{new}\}$ \textbf{\textcolor{blue}{where}} $C$ = \{x_j\!:\!v_i\}
}
}
&
\cell{\textbf{User provides:} A full initial configuration $X \in \{X_{\text{user}} \cup X_{\text{sys}}\}$ and desired changes in $Y$.
\textbf{Compass responds:} Minimal modifications to $X_{\text{user}}$ that achieve the target $Y$ while keeping $X_{\text{sys}}$ unchanged.}
% \cell{A full initial configuration $X \in {X_{user} \cup X_{sys}}$, desired changes in $Y$.}
% &
% \cell{Minimal changes to $X_{user}$ while keeping $X_{sys}$ unchanged to reach $Y$.}
% & 
\\
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{3}{|c|}{{\tablecellor{\textbf{\whatif}}}}\\\hline
\cell{
Given a change in $X_{user}$ while keeping $X_{sys}$ unchanged, estimate its effect on outcomes $Y$ (Forward problem).
Users or software systems decides based on the impact of changing one or more inputs on a desired outcome.}
& 
\cell{
\tightcell{
\textcolor{blue}{\textbf{What-if we change}}
$X = \{x_1: v_1^{old} \rightarrow v_1^{new}, \dots, x_n: v_n^{old} \rightarrow ?\}$, 
\textcolor{blue}{\textbf{how would that affect}} 
$Y = \{y_1, \dots, y_m\}$ \textbf{\textcolor{blue}{where}} $C$ = \{x_j\!:\!v_i\}}
}
&
\cell{\textbf{User provides:} Hypothetical changes in configuration parameters $X$.
\textbf{Compass responds:} Estimated changes in outcomes $Y$.}
\\
\hline
\end{tabular}
}
% \end{center}
\end{singlespacing}
\end{table}

==> Sections/query_map_table2.tex <==
% \begin{table*}[!t]
% \tiny\tiny
% \centering
% \caption{Summary of query templates prevalent in HPC decision-support scenarios.}
% \label{tab:query-templates}
% % \begin{singlespacing}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|p{12cm}|}
% \hline
% % \centering
% %\textbf{Query} 
% % & \textbf{Details} \\
% % \hline\hline

% % ========================= RECOMMEND =========================
% \cellcolor{bll} &
% \textbf{Intent \& HPC Scenarios:}
% Given target objectives $Y$, find values of $\mathcal{X}_{\text{user}}$ to meet those objectives (Inverse problem) on given optional constraints $C$. Use cases: Novice HPC users; Software systems such as job schedulers, resource managers, HPC facilities.\\
% % \cline{2-2}
% %% \vspace{-0.01in}
% \cellcolor{bll}\rotatebox[origin=c]{90}{\textbf{\reco}} &
% \textbf{Template:}
% \textcolor{blue}{Recommend a configuration} $\mathcal{X}_{\text{user}} = \{x_i : v_i, x_i : ?\}$
% \textcolor{blue}{to achieve} $Y=\{y_1: \mathcal{O}_{1}, \dots, y_m : \mathcal{O}_{m}\}$
% \textcolor{blue}{where} $C$ = $\{\!x_j\!:\!v_j\!\}$\\
% % \cline{2-2}
% \cellcolor{bll} &
% User provides: Objective(s) over $Y$ and constraints $C$, specifying configurable parameters in $\mathcal{X}_{user}$, known values for these can be specified or left unspecified ' while leaving remaining parameters unspecified.
% \sysname responds: Candidate configurations for $\mathcal{X}_{user}$, generated by conditioning on the empirical distribution of $\mathcal{X}_{sys}$ observed from historical jobs that satisfy $C$.\\ \hline
% % ========================= MODIFY =========================
% \cellcolor{sgl} &
% \textbf{Intent \& HPC Scenarios:}
% Given desired outcomes $Y$ and an initial configuration, update existing $\mathcal{X}_{user}$ with minimal changes (Counterfactual reasoning). Use cases: Autotuners; Performance tuning.
% \\ 
% % \cline{2-2}
% \cellcolor{sgl}\rotatebox[origin=c]{90}{\textbf{\modify}} &
% \textbf{Template:} \textcolor{blue}{Reconfigure}
% $\mathcal{X}_{\text{user}} = 
% \{x_1:v_1^{old}\rightarrow~v_1^{new},\!\dots\!, x_n:\!v_n^{old}\!\rightarrow\!?\}$
% \textcolor{blue}{to achieve}$Y$ = $\y_j:v_j^{old}\rightarrow\!v_j^{new}\}$
% \textcolor{blue}{where} $C$ = $\{x_j\!:\!v_j\}$
% \\ 
% \cellcolor{sgl} &
% \textbf{User provides:} A baseline configuration
% $x \in \{\mathcal{X}_{user} \cup \mathcal{X}_{sys}\}$,
% desired changes in $Y$, and optional constraints $C$.
% \textbf{\sysname responds:} Configurations that minimally modify
% $\mathcal{X}_{user}$ while satisfying $C$; all unspecified features
% are initialized to their baseline values but may change if required by
% feature correlations, in which case \sysname returns the closest feasible
% alternatives and defers the final decision to the user.
% \\ \hline
% % ========================= WHAT-IF =========================
% \cellcolor{orl} &
% \textbf{Intent \& HPC Scenarios:}
% Given a change in $\mathcal{X}_{user}$ while keeping $\mathcal{X}_{sys}$ unchanged, estimate its effect on outcomes $Y$ (Forward problem).
% Users or software systems decides based on the impact of changing one or more inputs on a desired outcome.
% \\ 
% % \cline{2-2}
% \cellcolor{orl}\rotatebox[origin=c]{90}{\textbf{\whatif}} &
% \textbf{Template:}\textcolor{blue}{What-if we change}
% $\mathcal{X}_{\text{user}} = \{x_1: v_1^{old} \rightarrow v_1^{new}, \dots, x_n: v_n^{old} \rightarrow v_n^{new}\}$,
% \textcolor{blue}{how would that affect}
% $Y = \{y_1, \dots, y_m\}$
% \textcolor{blue}{where} $C$ = $\{x_j\!:\!v_j\}$
% % \\ \cline{2-2}
% \\
% \cellcolor{orl} &
% \textbf{User provides}: A baseline configuration $X \in \{\mathcal{X}_{user} \cup \mathcal{X}_{sys}\}$, desired changes to $\mathcal{X}_{user}$, and constraints $C$, with all unspecified features set to their baseline values to form a complete configuration.
% \sysname responds: Predicted changes in outcomes $Y$.
% \\ \hline
% \end{tabular}
% }
% % \end{singlespacing}
% \end{table*}

% \begin{table}[t]
% \tiny
% \caption{Summary of query templates prevalent in HPC decision-support scenarios.}
% \label{tab:query-templates}
% % \begin{singlespacing}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|c|p{5cm}|}
% \hline
% % \centering
% %\textbf{Query} 
% % & \textbf{Details} \\
% % \hline\hline

% % ========================= RECOMMEND =========================
% \cellcolor{bll} &
% \textbf{Intent \& HPC Scenarios:}
% Given target objectives $Y$, find values of $\mathcal{X}_{\text{user}}$ to meet those objectives (Inverse problem) on given optional constraints $C$. Use cases: Novice HPC users; Software systems such as job schedulers, resource managers, HPC facilities.\\
% % \cline{2-2}
% % \vspace{-0.01in}
% \cellcolor{bll}\rotatebox[origin=c]{90}{\textbf{\reco}} &
% \textbf{Template:}
% \textcolor{blue}{Recommend a configuration} $\mathcal{X}_{\text{user}} = \{x_i : v_i, x_i : ?\}$
% \textcolor{blue}{to achieve} $Y=\{y_1: \mathcal{O}_{1}, \dots, y_m : \mathcal{O}_{m}\}$
% \textcolor{blue}{where} $C$ = $\{\!x_j\!:\!v_j\!\}$\\
% % \cline{2-2}
% \cellcolor{bll} &
% User provides: Objective(s) over $Y$ and constraints $C$, specifying configurable parameters in $\mathcal{X}_{user}$, known values for these can be specified or left unspecified ' while leaving remaining parameters unspecified.
% \sysname responds: Candidate configurations for $\mathcal{X}_{user}$, generated by conditioning on the empirical distribution of $\mathcal{X}_{sys}$ observed from historical jobs that satisfy $C$.\\ \hline
% % ========================= MODIFY =========================
% \cellcolor{sgl} &
% \textbf{Intent \& HPC Scenarios:}
% Given desired outcomes $Y$ and an initial configuration, update existing $\mathcal{X}_{user}$ with minimal changes (Counterfactual reasoning). Use cases: Autotuners; Performance tuning.
% \\ 
% % \cline{2-2}
% \cellcolor{sgl}\rotatebox[origin=c]{90}{\textbf{\modify}} &
% \textbf{Template:} \textcolor{blue}{Reconfigure}
% $\mathcal{X}_{\text{user}} = 
% \{x_1:v_1^{old}\rightarrow~v_1^{new},\!\dots\!, x_n:\!v_n^{old}\!\rightarrow\!?\}$
% \textcolor{blue}{to achieve}$Y$ = $\y_j:v_j^{old}\rightarrow\!v_j^{new}\}$
% \textcolor{blue}{where} $C$ = $\{x_j\!:\!v_j\}$
% \\ 
% \cellcolor{sgl} &
% \textbf{User provides:} A baseline configuration
% $x \in \{\mathcal{X}_{user} \cup \mathcal{X}_{sys}\}$,
% desired changes in $Y$, and optional constraints $C$.
% \textbf{\sysname responds:} Configurations that minimally modify
% $\mathcal{X}_{user}$ while satisfying $C$; all unspecified features
% are initialized to their baseline values but may change if required by
% feature correlations, in which case \sysname returns the closest feasible
% alternatives and defers the final decision to the user.
% \\ \hline
% % ========================= WHAT-IF =========================
% \cellcolor{orl} &
% \textbf{Intent \& HPC Scenarios:}
% Given a change in $\mathcal{X}_{user}$ while keeping $\mathcal{X}_{sys}$ unchanged, estimate its effect on outcomes $Y$ (Forward problem).
% Users or software systems decides based on the impact of changing one or more inputs on a desired outcome.
% \\ 
% % \cline{2-2}
% \cellcolor{orl}\rotatebox[origin=c]{90}{\textbf{\whatif}} &
% \textbf{Template:}\textcolor{blue}{What-if we change}
% $\mathcal{X}_{\text{user}} = \{x_1: v_1^{old} \rightarrow v_1^{new}, \dots, x_n: v_n^{old} \rightarrow v_n^{new}\}$,
% \textcolor{blue}{how would that affect}
% $Y = \{y_1, \dots, y_m\}$
% \textcolor{blue}{where} $C$ = $\{x_j\!:\!v_j\}$
% % \\ \cline{2-2}
% \\
% \cellcolor{orl} &
% \textbf{User provides}: A baseline configuration $X \in \{\mathcal{X}_{user} \cup \mathcal{X}_{sys}\}$, desired changes to $\mathcal{X}_{user}$, and constraints $C$, with all unspecified features set to their baseline values to form a complete configuration.
% \sysname responds: Predicted changes in outcomes $Y$.
% \\ \hline
% \end{tabular}
% }
% % \end{singlespacing}
% \end{table}

% \begin{table}[t]
% \tiny
% \caption{Summary of query templates prevalent in HPC decision-support scenarios.}
% \label{tab:query-templates}
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{0.92}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|>{\centering\arraybackslash}m{0.55cm}|p{5cm}|}
% \hline

% % ========================= RECOMMEND =========================
% \multirow{3}{*}{\cellcolor{bll}\rotatebox[origin=c]{90}{\textbf{\reco}}} &
% \textbf{Intent \& HPC Scenarios:}
% Given target objectives $Y$, find values of $\mathcal{X}_{\text{user}}$ to meet those objectives (Inverse problem) on given optional constraints $C$. Use cases: Novice HPC users; Software systems such as job schedulers, resource managers, HPC facilities.
% \\

% &
% \textbf{Template:}
% \textcolor{blue}{Recommend a configuration} $\mathcal{X}_{\text{user}} = \{x_i : v_i, x_i : ?\}$
% \textcolor{blue}{to achieve} $Y=\{y_1: \mathcal{O}_{1}, \dots, y_m : \mathcal{O}_{m}\}$
% \textcolor{blue}{where} $C$ = $\{\!x_j\!:\!v_j\!\}$
% \\

% &
% User provides: Objective(s) over $Y$ and constraints $C$, specifying configurable parameters in $\mathcal{X}_{user}$, known values for these can be specified or left unspecified ' while leaving remaining parameters unspecified.
% \sysname responds: Candidate configurations for $\mathcal{X}_{user}$, generated by conditioning on the empirical distribution of $\mathcal{X}_{sys}$ observed from historical jobs that satisfy $C$.
% \\ \hline

% % ========================= MODIFY =========================
% \multirow{3}{*}{\cellcolor{sgl}\rotatebox[origin=c]{90}{\textbf{\modify}}} &
% \textbf{Intent \& HPC Scenarios:}
% Given desired outcomes $Y$ and an initial configuration, update existing $\mathcal{X}_{user}$ with minimal changes (Counterfactual reasoning). Use cases: Autotuners; Performance tuning.
% \\

% &
% \textbf{Template:} \textcolor{blue}{Reconfigure}
% $\mathcal{X}_{\text{user}} =
% \{x_1:v_1^{old}\rightarrow~v_1^{new},\!\dots\!, x_n:\!v_n^{old}\!\rightarrow\!?\}$
% \textcolor{blue}{to achieve}$Y$ = $\{y_j:v_j^{old}\rightarrow\!v_j^{new}\}$
% \textcolor{blue}{where} $C$ = $\{x_j\!:\!v_j\}$
% \\

% &
% \textbf{User provides:} A baseline configuration
% $x \in \{\mathcal{X}_{user} \cup \mathcal{X}_{sys}\}$,
% desired changes in $Y$, and optional constraints $C$.
% \textbf{\sysname responds:} Configurations that minimally modify
% $\mathcal{X}_{user}$ while satisfying $C$; all unspecified features
% are initialized to their baseline values but may change if required by
% feature correlations, in which case \sysname returns the closest feasible
% alternatives and defers the final decision to the user.
% \\ \hline

% % ========================= WHAT-IF =========================
% \multirow{3}{*}{\cellcolor{orl}\rotatebox[origin=c]{90}{\textbf{\whatif}}} &
% \textbf{Intent \& HPC Scenarios:}
% Given a change in $\mathcal{X}_{user}$ while keeping $\mathcal{X}_{sys}$ unchanged, estimate its effect on outcomes $Y$ (Forward problem).
% Users or software systems decides based on the impact of changing one or more inputs on a desired outcome.
% \\

% &
% \textbf{Template:}\textcolor{blue}{What-if we change}
% $\mathcal{X}_{\text{user}} = \{x_1: v_1^{old} \rightarrow v_1^{new}, \dots, x_n: v_n^{old} \rightarrow v_n^{new}\}$,
% \textcolor{blue}{how would that affect}
% $Y = \{y_1, \dots, y_m\}$
% \textcolor{blue}{where} $C$ = $\{x_j\!:\!v_j\}$
% \\

% &
% \textbf{User provides}: A baseline configuration $X \in \{\mathcal{X}_{user} \cup \mathcal{X}_{sys}\}$, desired changes to $\mathcal{X}_{user}$, and constraints $C$, with all unspecified features set to their baseline values to form a complete configuration.
% \sysname responds: Predicted changes in outcomes $Y$.
% \\ \hline

% \end{tabular}%
% }
% \end{table}
\begin{table}[t]
\tiny
\caption{Summary of query templates prevalent in HPC decision-support scenarios.}
\label{tab:query-templates}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{1.2cm}|p{4.95cm}|}
\hline

% ========================= RECOMMEND =========================
\rowcolor{bll}
\multicolumn{2}{|c|}{\rule{0pt}{1.9ex}\textbf{\reco}\rule[-0.6ex]{0pt}{0pt}}\\ \hline

\textbf{Intent \& HPC Scenarios:} &
Given target objectives $Y$, find values of $\mathcal{X}_{\text{user}}$ to meet those objectives (Inverse problem) on given optional constraints $C$. Use cases: Novice HPC users; Software systems such as job schedulers, resource managers, HPC facilities.
\\ \hline

\textbf{Template:} &
\textcolor{blue}{Recommend a configuration} $\mathcal{X}_{\text{user}} = \{x_i : v_i, x_i : ?\}$
\textcolor{blue}{to achieve} $Y=\{y_1: \mathcal{O}_{1}, \dots, y_m : \mathcal{O}_{m}\}$
\textcolor{blue}{where} $C$ = $\{\!x_j\!:\!v_j\!\}$
\\ \hline

\textbf{User provides:} &
Objective(s) over $Y$ and constraints $C$, specifying configurable parameters in $\mathcal{X}_{user}$, known values for these can be specified or left unspecified ' while leaving remaining parameters unspecified.
\sysname responds: Candidate configurations for $\mathcal{X}_{user}$, generated by conditioning on the empirical distribution of $\mathcal{X}_{sys}$ observed from historical jobs that satisfy $C$.
\\ \hline

% ========================= MODIFY =========================
\rowcolor{sgl}
\multicolumn{2}{|c|}{\rule{0pt}{1.9ex}\textbf{\modify}\rule[-0.6ex]{0pt}{0pt}}\\ \hline

\textbf{Intent \& HPC Scenarios:} &
Given desired outcomes $Y$ and an initial configuration, update existing $\mathcal{X}_{user}$ with minimal changes (Counterfactual reasoning). Use cases: Autotuners; Performance tuning.
\\ \hline

\textbf{Template:} &
\textcolor{blue}{Reconfigure}
$\mathcal{X}_{\text{user}} =
\{x_1:v_1^{old}\rightarrow~v_1^{new},\!\dots\!, x_n:\!v_n^{old}\!\rightarrow\!?\}$
\textcolor{blue}{to achieve} $Y$ = $\{y_j:v_j^{old}\rightarrow\!v_j^{new}\}$
\textcolor{blue}{where} $C$ = $\{x_j\!:\!v_j\}$
\\ \hline

\textbf{User provides:} &
A baseline configuration
$x \in \{\mathcal{X}_{user} \cup \mathcal{X}_{sys}\}$,
desired changes in $Y$, and optional constraints $C$.
\textbf{\sysname responds:} Configurations that minimally modify
$\mathcal{X}_{user}$ while satisfying $C$; all unspecified features
are initialized to their baseline values but may change if required by
feature correlations, in which case \sysname returns the closest feasible
alternatives and defers the final decision to the user.
\\ \hline

% ========================= WHAT-IF =========================
\rowcolor{orl}
\multicolumn{2}{|c|}{\rule{0pt}{1.9ex}\textbf{\whatif}\rule[-0.6ex]{0pt}{0pt}}\\ \hline

\textbf{Intent \& HPC Scenarios:} &
Given a change in $\mathcal{X}_{user}$ while keeping $\mathcal{X}_{sys}$ unchanged, estimate its effect on outcomes $Y$ (Forward problem).
Users or software systems decides based on the impact of changing one or more inputs on a desired outcome.
\\ \hline

\textbf{Template:} &
\textcolor{blue}{What-if we change}
$\mathcal{X}_{\text{user}} = \{x_1: v_1^{old} \rightarrow v_1^{new}, \dots, x_n: v_n^{old} \rightarrow v_n^{new}\}$,
\textcolor{blue}{how would that affect}
$Y = \{y_1, \dots, y_m\}$
\textcolor{blue}{where} $C$ = $\{x_j\!:\!v_j\}$
\\ \hline

\textbf{User provides:} &
A baseline configuration $X \in \{\mathcal{X}_{user} \cup \mathcal{X}_{sys}\}$, desired changes to $\mathcal{X}_{user}$, and constraints $C$, with all unspecified features set to their baseline values to form a complete configuration.
\sysname responds: Predicted changes in outcomes $Y$.
\\ \hline

\end{tabular}%
}
\end{table}

==> Sections/recommend.tex <==
\tzi{If we are using counterfactuals for this -- we need to describe differently.}
Recommendation queries begin with a set of performance goals (e.g., minimize runtime, reduce power) and return a configuration that satisfies these goals without requiring a baseline configuration. \sysname formulates this as a satisficing optimization problem over the feasible configuration space $\mathcal{C} \subseteq \mathbb{R}^d$:

\begin{equation*}
\mathbf{x}^* = \arg\min_{\mathbf{x}' \in \mathcal{C}} \mathcal{L}_{\text{multi}}(f(\mathbf{x}'), \mathbf{y}^*)
\end{equation*}

Here, $f$ is a predictive model, $\mathbf{y}^*$ is the desired performance vector, and $\mathcal{L}_{\text{multi}}$ encodes a weighted loss across multiple objectives (e.g., runtime, energy, throughput). Instead of seeking a globally optimal configuration, \sysname returns a satisfying solution, one that meets all user constraints while trading off competing objectives. % reasonably.


%%%%%%%%%%%%%%%%%%%%%%%%
\noindent In contrast to counterfactuals--where an initial desirable full or partial configuration is known, %and outcomes are explored—
recommendation begins with a desired outcome and returns one or more feasible configurations that achieve it. The system searches over a constrained configuration space $\mathcal{C}$ for candidates that optimize one or more objectives.
If users provide constraints or thresholds across multiple performance metrics, the system formulates the query as a satisficing problem--identifying configurations that may not be globally optimal but lie within a trade-off region.

\textbf{How to use:} \tzi{@ankur -- please write an example of what would be the input by following my example at the end of section 3.4}


==> Sections/related-work.tex <==
\begin{table}[t]
\tiny
\centering
\caption{Comparison of \sysname with different Autotuning libraries, generative and predictive modeling. Predictive modeling has no search criteria, they predict target on given configuration, opposite to our work. \tzi{Add citation and check the names}}
\label{tab:comparison_autotunner}
\resizebox{\textwidth}{!}{
\begin{tabular}{|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1.5cm}|}
\hline
\textbf{Features}
  & \multicolumn{6}{c|}{\cellcolor{blue!20}\textbf{Autotuner}}
  & \multicolumn{4}{c|}{\cellcolor{green!20}\textbf{Generative Modeling}}
  & \multicolumn{1}{c|}{\cellcolor{orange!20}\textbf{Predictive Modeling}}
  & \multicolumn{1}{c|}{\cellcolor{violet!20}\textbf{Decision Framework}}
\\ \hline
  & ytopt & Open-Tuner & Harmony & HYPERF & GPTune & BoFire & BeGreaT & CTGAN & GAN & Diffusion & ModelX & \tablecellbl{\textbf{\sysname}} \\
\hline
Search Criteria
  & \cell{Min, Max} & \cell{Min, Max} & \cell{Min, Max} & \cell{Min, Max} & \cell{Min, Max} & \cell{Min, Max}
  & \cell{Min, Max, Range} & \cell{Min, Max} & \cell{Cat., Cont.} & \cell{Cat., Cont.}
  &  \ding{56}
  & \tablecellbl{\cell{Cat, Min, Max, Range}} \\
\hline
\cell{\reco}
  & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52}
  & \ding{52} & \ding{52} & \ding{52} & \ding{52}
  & \ding{56}
  & \tablecellbl{\ding{52}} \\
\hline
\cell{\modify}
  & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56}
  & \ding{52} & \ding{52} & \ding{56} & \ding{56}
  & \ding{56}
  & \tablecellbl{\ding{52}} \\
\hline
\cell{\whatif}
  & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56}
  & \ding{52} & \ding{52} & \ding{56} & \ding{56}
  & \ding{56}
  & \tablecellbl{\ding{52}} \\
\hline
Query-Driven Interface
  & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56}
  & \ding{52} & \ding{56} & \ding{56} & \ding{56}
  & \ding{56}
  & \tablecellbl{\ding{52}} \\
\hline
Reliability Assessment
  & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56}
  & \ding{52} & \ding{52} & \ding{52} & \ding{52}
  & \ding{52}
  & \tablecellbl{\ding{52}} \\
\hline
Interpretable Explanation
  & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56}
  & \ding{52} & \ding{52} & \ding{52} & \ding{52}
  & \ding{52}
  & \tablecellbl{\ding{52}} \\
\hline
Satisficing Solutions
  & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56}
  & \ding{52} & \ding{56} & \ding{56} & \ding{56}
  & \ding{56}
  & \tablecellbl{\ding{52}} \\
\hline
\end{tabular}
}
\end{table}

% \begin{table}[t]
% \centering
% \caption{Comparison of \sysname with different Autotuning libraries.}
% \label{tab:comparison_autotunner}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{p{1.5cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1.5cm}}
% \hline
% \textbf{Features} & \textbf{ytopt} & \textbf{Open-Tuner} & \textbf{Har-mony} & \textbf{HYPERF} & \textbf{GPTune} &\textbf{BoFire} & \tablecellbl{\textbf{\sysname}} \\
% & \cite{wu2025ytopt} & \cite{ansel2014opentuner} & \cite{tapus2002active} & \cite{park2025hyperf} & \cite{liu2021gptune} & \cite{durholt2025bofire} & \tablecellbl{This Work}\\
% \hline
% % Optimization & Bayesian & Ensemble & Search-based & Bayesian & Gaussian & Bayesian & Counterfactual\\
% % Technique & Optimization & Search & Navigation & Optimization & Process & Optimization & Reasoning \\
% % \hline
% % % Explainablity & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} \\
% % % \hline

% % Focus & Performance & Compiler & Runtime & Loop & Performance & Experimental & Performance 
% % \\
% %  & counters & Flags & Parameters & Programs & Data & Outcome & Data \\

% %  \hline

% % Domain & Code-evaluation   & Application & Application  & Application & Application   & Tabular  & Tabular  
% % \\
% %  & wrapper & Code &  &  & Code & data & data  \\
 
% \hline
% Search Criteria & \cell{Min, Max} & \cell{Min, Max} & \cell{Min, Max} & \cell{Min, Max} & \cell{Min, Max} & \cell{Min, Max} & \tablecellbl{\cell{Min, Max, Range}}\\
% \hline
% \cell{\reco} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \tablecellbl{\ding{52}} \\
% \hline
% \cell{\modify} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \tablecellbl{\ding{52}} \\ 
% \hline
% \cell{\whatif} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \tablecellbl{\ding{52}} \\
% \hline
% \cell{Query-Driven Interface}  & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \tablecellbl{\ding{52}} \\
% \hline
% Reliability Assessment & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \tablecellbl{\ding{52}} 
% \\
% \hline
% Interpretable Explanation & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \tablecellbl{\ding{52}} 
% \\
% \hline
% \cell{Satisficing Solutions} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \tablecellbl{\ding{52}} \\
% \hline
% \end{tabular}
% }
% \end{table}

\noindent
Researchers in high-performance computing (HPC) have long focused on modeling and analyzing large-scale performance and operational data generated by scientific workflows and industrial applications.  
As data volumes increase across diverse workloads, manual performance annotation becomes infeasible, motivating automated modeling and diagnostic tools. Performance modeling enables users to understand and predict how applications behave on modern architectures, helping to identify bottlenecks and scalability limits before deployment.

\noindent
Different tools, such as PerfExplorer~\cite{huck2005perfexplorer}, HPCToolkit~\cite{adhianto2010hpctoolkit}, and PADDLE~\cite{thiagarajan2018paddle}, represent major advances in performance analysis. PerfExplorer provides clustering, summarization, and comparative analytics to reveal performance trends across runs.  
HPCToolkit attributes resource inefficiencies to code regions across CPUs and GPUs, supporting deep attribution for hybrid parallel programs. PADDLE extends these ideas through a machine learning platform for prediction and workflow integration, enabling analysts to extract performance patterns from complex datasets.   However, these systems are largely diagnostic—they identify issues but do not generate or recommend \emph{actionable alternatives}. Similarly, PERFGEN~\cite{banday2024perfgen} synthesizes performance data to aid model training, yet its outputs serve simulation or benchmarking purposes rather than producing feasible alternative scenarios for decision support. 

\noindent
A variety of autotuning frameworks have been proposed in HPC to suggest performance optimization of the HPC system, applications, and application-level codes. Existing approaches mentioned in Table~\ref{tab:comparison_autotunner} primarily focus on recommending high-performance computing configurations to achieve specific objectives, typically minimizing or maximizing them. ytopt \cite{wu2025ytopt} and OpenTuner \cite{ansel2014opentuner} are two autotuners developed early in the HPC field, adopting Bayesian Optimization and ensemble search strategies, respectively, to tune compiler-level and application-level parameters. Active Harmony \cite{tapus2002active} focuses on explicitly runtime parameters optimization using the search-based navigation techniques, while HYPERF \cite{park2025hyperf} concentrates on loop-level program transformations using Bayesian optimization. Most recent learning-based approaches, GPTune \cite{liu2021gptune}, leverage Gaussian process models to guide configuration search across applications and hardware platforms. BoFire \cite{durholt2025bofire},  targets experimental design problems over tabular data using Bayesian optimization, which is closer to the domain we are focusing on. However, despite their effectiveness, most of these autotuners are enable to support reconfiguration or counterfactual reasoning over performance data where we focus.

Our proposed approach differs fundamentally from standard generative modeling methods because the requirements of \textbf{\texttt{decision support}} are different from those of \texttt{\textbf{sample generation}}. Generative models such as  Generative Adversarial Networks (GANs)~\cite{goodfellow2020generative} and Diffusion Models~\cite{kotelnikov2023tabddpm} are designed to approximate global data distribution, whereas our \sysname goal is to produce samples that are closely aligned to certain objective(s). Relying solely on data distribution may violate system constraints or generate candidates outside the user-specified constraints. Decision support, in contrast, demands local, constraint-aware, and goal-directed reasoning, in which candidate configurations must remain close to a given baseline. We discussed the effect of this architectural difference in the Section \ref{sec:results-compass-vs-others}.

==> Sections/related_work_table.tex <==
\begin{table}[t]
\centering
\caption{Comparison of the proposed framework with existing popular ML approaches.}
\label{tab:comparison_ml}
\begin{singlespacing}
\resizebox{\columnwidth}{!}{
% \renewcommand{\arraystretch}{1.15}
% \setlength{\tabcolsep}{6pt}
\begin{tabular}{>{\raggedright\arraybackslash}p{6.2cm} c c c c}
\toprule
\textbf{Features} &
\textbf{\begin{tabular}[c]{@{}c@{}}Dimensionality\\Reduction\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}Supervised\\Learning\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}Deep Neural\\Networks\end{tabular}} &
\textbf{Proposed\\Approach} \\
\midrule
Hierarchical feature learning                    & \xmark & \xmark & \cmark & \cmark \\
Low dimensional structure inference              & \cmark & \xmark & \cmark & \cmark \\
Supports the use of multi-source data            & \xmark & \xmark & \cmark & \cmark \\
Supports the use of categorical data             & \xmark & \cmark & \xmark & \cmark \\
Interpretability of the inferred models          & \cmark & \cmark & \xmark & \cmark \\
Robustness to limited training data              & N/A    & \cmark & \xmark & \cmark \\
Facilitates model selection                      & N/A    & \xmark & \xmark & \cmark \\
References                                       & {[20], [21], [22]} & {[23], [24], [25]} & {[16], [17]} & N/A \\
\bottomrule
\end{tabular}
}
\end{singlespacing}
\end{table}

==> Sections/reliability2.tex <==
Most existing \gls{hpc} tools rely primarily on uncertainty quantification (UQ) to assess confidence. However, UQ alone captures only the magnitude of model uncertainty, not its source, offering no distinction between uncertainty arising from sparse data, model bias, or extrapolation beyond the training domain.
To address this limitation, \sysname introduces a gating and explanation framework to assess the reliability of counterfactual configurations.
The framework separates three distinct but complementary notions of reliability:
\begin{itemize}
    \item \textbf{Data support}: \emph{quantifies} whether a configuration lies within regions of the feature space represented in the training data.
    \item \textbf{Model confidence}: \emph{measures} whether independent predictive models (distinct from the surrogate used for counterfactual generation) produce predictions whose pairwise disagreement remains below a predefined threshold relative to the synthesized target value for the configuration.
    \item \textbf{Reliability guidance}: \emph{identifies} regions of the configuration space where data sparsity or model instability limits predictive reliability, indicating where additional data collection or model refinement is required.
\end{itemize}
This separation is critical because configurations that lie outside the support of the training data can still receive confident predictions from a model, while configurations that are well supported by data can exhibit high predictive uncertainty. \tzi{Can we show with an example from one of the datasets? or reference of papers that show that?}
\sysname explicitly disentangles these factors to prevent misleading users.
\tzi{Need to make sure that there is no repetition or overlap with actionable outcome section. Will be done in iteration 2.}



==> Sections/reliability_algo.tex <==
\begin{algorithm}[t]
\caption{Assessing Reliability of Generated Configurations}
\label{alg:assess_reliability}
\textbf{Require:} Configuration $x$, dataset $D_{train}$\\
\textbf{Ensure:} $D_{train}$ partitioned into $X_{train}$ and $X_{val}$\\

\begin{algorithmic}
    \State \textbf{A. Calculate OOD:}
    \begin{itemize}
        \item Fit a kNN model on $X_{train}$
        \item For each validation sample $v_i \in X_{val}$
, compute $d(v_i)$, the mean Euclidean distance to its
$k$ nearest neighbors in $X_{train}$ %, and store in the list $D = \{d(v_i)\}_{i=1}^{N}$  %such that $D = [d(v_1), d(v_2), ..., d(v_N)]$.
        \item For the candidate configuration $x$, compute $d(x)$, the mean Euclidean distance from $x$ to its $k$ nearest neighbors in $X_{train}$
        %Compute the mean Euclidean distance from configuration $x$ to its $k$ nearest training samples, denoted by $d(x)$
        \item Calculate the fraction of validation samples with smaller kNN distance than $x$:
        
        $OOD(x) = \frac{1}{N} \sum\limits_{i=1}^{N} 1[d(v_i)\leq d(x)] \in [0,1]$, where $1[\cdot]$ means $1$ if true, else $0$
        % \textcolor{blue}{// this gives us the percentile of $X_{val}$ samples that have distance $\leq$ that of $x$; lower is better}
    \end{itemize}
    \State \textbf{B. Calculate UQ:}
    \begin{itemize}
        \item Train an ensemble of $K$ models on $X_{train}$
        % \item For each $v \in X_{val}$ save predictions ($[\hat y_1(v_i),..., \hat y_k(v_i)]$) from $K$ models for regression, and class-probability vector over $C$ classes ($\bar{p}_{1-k}(v_i)$ ) for classification.
        % % $[\hat y_1(v_i),\hat y_2(v_i),..., \hat y_k(v_i)]$
        \item For each validation sample $v_i \in X_{val}$ calculate how much the predictions produced by different models differ from one another:
        % Calculate differnce in ensemble predictions for each $v \in X_{val}$:
        \begin{itemize}
            \item For regression: compute difference between the $75^{th}$ and $25^{th}$ percentile predictions,

            
            %the IQR of the $K$ ensemble predictions
            $u(v_i) = Q_{75}(\hat y_k(v_i)) - Q_{25}(\hat y_k(v_i))$ 
            %\textcolor{blue}{// we use the middle $50\%$ of the predictions instead of standard deviation across all predictions for robustness against extreme predictions}
            \item For classification: compute the difference between the largest and second-largest averaged class probabilities, $u(v_i) = - \sum\limits_{c=1}^{C}\bar{p}_c(v_i)log(\bar{p}_c(v_i))$
    %and store it as $u(v)$. 
        \end{itemize}
    \item Calculate $u(x)$, how much
the predictions produced by different models differ from one
another for configuration $x$ in the same way as done for each $v_i \in X_{val}$
    \item Calculate the fraction of validation samples with smaller prediction /entropy than $x$:
    
    $UQ(x)=\frac{1}{N}\sum\limits_{i=1}^{N}1[u(v_i) \leq u(x)] \in [0,1]$, where $1[\cdot]$ means $1$ if true, else $0$ 
    % \textcolor{blue}{// this gives the percentile of $X_{val}$ samples with disagreement score $\leq$ disagreement score of  $x$}
    \end{itemize}
    \State \textbf{C. Label Configuration}
    \begin{itemize}
        \item If OOD(x) > $0.99$:
        \begin{itemize}
            \item Label = unsupported
            \item break
            % Return label + suggestions for data collection
        \end{itemize}
        \item Label config:
        \begin{itemize}
            \item If $OOD(x)$ > $0.95$: label = caution
            \item if $UQ(x)$ > $0.95$: label = caution
            \item if $OOD(x)$ > $0.95$ AND $UQ(x)$ > $0.99$: label = unsupported
            \item else: label = trusted
        \end{itemize}
        \item If label in [caution, unsupported]: return label + suggestions for data collection
        \item Return label
    \end{itemize}

\end{algorithmic}
\end{algorithm}


==> Sections/reliability_algo2.tex <==
\begin{algorithm}[t]
\caption{Assessing Reliability of Generated Configurations}
\label{alg:assess_reliability}
\textbf{Require:} Candidate configuration $x$, training set $X_{\text{train}}$, validation set $X_{\text{val}}$  
\textbf{Ensure:} Reliability label $\in$ \{\textit{trusted}, \textit{caution}, \textit{unsupported}\}

\begin{algorithmic}[1]   % <-- line numbers enabled

% \State Split $D_{\text{train}}$ into training set $X_{\text{train}}$ and validation set $X_{\text{val}}$

\State \textbf{Compute data support (OOD score)}
\State Fit a $k$-nearest-neighbor model on $X_{\text{train}}$
\For{each $v_i \in X_{\text{val}}$}
    \State Compute $d(v_i)$, the mean distance to its $k$ nearest neighbors in $X_{\text{train}}$
\EndFor
\State Compute $d(x)$, the mean distance from $x$ to its $k$ nearest neighbors in $X_{\text{train}}$
\State $OOD(x) \leftarrow \frac{1}{N}\sum_{i=1}^{N} \mathbb{I}[d(v_i) \le d(x)]$

\State \textbf{Compute model uncertainty (UQ score)}
\State Train an ensemble of $K$ predictive models on $X_{\text{train}}$
\For{each $v_i \in X_{\text{val}}$}
    \State Compute ensemble disagreement $u(v_i)$
\EndFor
\State Compute ensemble disagreement $u(x)$
\State $UQ(x) \leftarrow \frac{1}{N}\sum_{i=1}^{N} \mathbb{I}[u(v_i) \le u(x)]$

\State \textbf{Assign reliability label}
\If{$OOD(x) > 0.99$}
    \State \Return \textit{unsupported}
\ElsIf{$OOD(x) > 0.95$ \textbf{or} $UQ(x) > 0.95$}
    \State \Return \textit{caution}
\Else
    \State \Return \textit{trusted}
\EndIf

\end{algorithmic}
\end{algorithm}


==> Sections/result_modify_sc26.tex <==
The objective of this experiment is to evaluate the effectiveness of \sysname's $C^3G$ loss function compared to other counterfactual generation libraries such as \dice and \tabcf~\cite{panagiotou2024tabcf} for the \query type. All methods operate on the same initial configurations and use an identical surrogate model $f_{\theta}$, ensuring that observed differences arise solely from their configuration-generation mechanisms.

% \textbf{Observations \& Validation.}
% Table ~\ref{tab:be-great-comp-summary} shows that the MAPE for \modify is consistently lower than that of other generative libraries, indicating that the configurations suggested by \sysname align the input features more effectively with the desired outputs.  
% The improvements are robust across both predictive models, confirming that the edits are model-agnostic and transferable.
% %\textbf{Validation} 
% We validate our findings by comparing them against published results in the literature. (1) For Monet, it suggested to redistribute network traffic pattern to the Y axis.  (2) For the PM-100 dataset, reducing overprovisioned CPU cores by 68\% could maintain GPU utilization while cutting CPU power consumption by 10\%.
% (3)  Similarly, for BUTTER-E, the authors suggest a moderate to high depth of 15, while the highest depth experienced by the authors was from 7 to 20. (4) For CoMD, \sysname suggests lower node\_count and and lowering power\_cap while keeping same Bw\_level is same. (5) \sysname For the given query of the FT dataset,\sysname it is suggested to use \texttt{spr} instead of \texttt{rand} because \texttt{spr} is more deterministic than \texttt{rand}, which reduces performance variability. ~\cite{patki2019performance}. 
\textbf{Observations \& Validation.}
\textbf{Observations \& Validation.}
Table~\ref{tab:be-great-comp-summary} shows that the MAPE for \modify is consistently lower than that of other counterfactual generation libraries. This difference arises because \sysname encodes domain constraints directly into the generative loss and optimizes a point-based target loss (\( \mathcal{L}_{\text{valid}} \)), whereas \dice relies on a range-based validity loss without enforcing constraints during generation. As a result, \sysname generates counterfactuals that more faithfully satisfy the target while remaining feasible. The only exception is CoMD, where further inspection shows that although \dice generates lower-error samples, a larger fraction violate domain constraints than that generated by \sysname. An example of such a constraint was the number of threads must be even. 

We validate these results by comparing the generated edits against published findings. For Monet, \sysname redistributes network traffic along the Y axis, matching reported communication-efficient placements. For PM-100, it reduces overprovisioned CPU cores by 68\%, preserving GPU utilization while lowering CPU power by 10\%. For BUTTER-E, \sysname selects a moderate-to-high depth consistent with the range (7--20) explored in prior work. For CoMD, it reduces node\_count ($4096 \rightarrow 2026$) and power\_cap ($64 \rightarrow 92$) while maintaining the same Bw\_level, reducing run-to-run execution time variability by 10\%. This observation aligns with known performance--power tradeoffs. For FT, \sysname recommends \texttt{pak} over \texttt{rand} to reduce average run-to-run execution time variability by 10\% because deterministic placement reduces performance variability, consistent with prior observations~\cite{patki2019performance}.

% (1) \sysname-selected edits consistently achieve lower rMAPE across all datasets with \tzi{high confidence}. \tzi{Any high OOS?}  
% (2) Compared to raw-DiCE, \sysname's top-ranked edits show significantly lower NLL and OOD, reflecting more in-distribution, high-confidence edits. This observation demonstrates that \sysname's subsampling and filtering method makes an existing counterfactual generation method more effective by removing noise. 
% \tzi{(3) The nearest-neighbor-edit method has the highest rMAPE due to the lack of matching samples that satisfy both $X$ and $Y$ constraints.  }
% (4) \tzi{Although raw-DiCE generates plausible counterfactuals, \sysname's method of using the composite score to rank filters those samples that have high OOS, OOD, NLL, or higher difference. This novel evaluation-guided counterfactual generation advances the SOTA method's effectiveness significantly.}
% (5) On average, \sysname modifies fewer features than raw-DiCE, supporting that scoring implicitly favors minimal edits.  
%




==> Sections/results-c3g-loss.tex <==
\subsection{Effectiveness of the $C^3G$ Loss Function}
\label{sec:loss-eval}
% \input{Sections/table_tabcf_comp}
The objective of the study is to compare the effectiveness of $C^3G$ loss formulation with that of other existing constrained configuration loss functions, as implemented in DiCE and TABCF. Table~\ref{tab:be-great-comp-summary} presents the comparison results using MAPE for regression datasets, F1 score for classification datasets.
This experiment compares $C^3G$ with \dice and \tabcf~\cite{panagiotou2024tabcf} across six datasets and all queries. Existing configuration-generation libraries (e.g., \dice, TabCF) use the same configurations for both libraries. 
All methods use the same surrogate model $f_{\theta}$ (Random Forest) so that the observations boil down to their generative modeling capabilities.

\textbf{Observation}
From Table~\ref{tab:be-great-comp-summary}, we observe that (1) for \reco queries, our $C^3G$ loss function outperforms the vanilla \dice loss 4 out of 5 times. (2) For the PM-100 dataset, our MAPE is higher than \dice; however, our generated sample successfully provides valid recommendations for domain guidance generation. (3) For \modify queries our MAPE is closer to the \dice loss function. (4) \tabcf can't generate any recommendations for PM-100, while our loss function and \dice can both generate recommendations for the given queries. The rationale is that \tabcf
constrains generation to the learned data manifold via a VAE latent space while jointly optimizing validity, proximity, and latent-distance losses. When the target prediction lies in off-manifold regions, these constraints conflict, preventing TABCF from reaching the desired outcome. In contrast, Compass operates directly in feature space, prioritizing target attainment and proximity through gradient-based or search-based optimization without enforcing
manifold adherence. This design enables \sysname to generate valid configurations beyond the training manifold and to better handle complex, structured configuration spaces.


==> Sections/results-hpdc26.tex <==
We evaluate \sysname by running the following experiments:
    (1) Surrogate model selection. 
    (2) Effectiveness of \reco, \modify, and \whatif queries. 
    (3) Overhead, scalability, and reproducibility. 
    (4) Synthetic benchmarking for validation.
    (5) Applicability of \sysname for HPC job scheduling.
% \subsubsection{Sensitivity of Subset Sampling}
% \label{sec:results-subsample}
% \input{Sections/results_subset_sampling}
\subsection{Surrogate Model Selection}
\label{sec:result-surrogate}
\input{Sections/results_all_models}
\input{Sections/results_model_performance}


% From Table~\ref{tab:tabcf_comp}, we observe that (1) for \modify queries, \sysname modifies significantly fewer features than \tabcf, and (2) \tabcf fails to generate valid configurations in multiple cases, whereas \sysname succeeds consistently.
% The rationale is that \tabcf constrains generation to the learned data manifold via a VAE latent space while jointly optimizing validity, proximity, and latent-distance losses.
% When the target prediction lies in off-manifold regions, these constraints conflict, preventing \tabcf from reaching the desired outcome.
% In contrast, \sysname operates directly in feature space, prioritizing target attainment and proximity through gradient-based or search-based optimization without enforcing manifold adherence.
% This design enables \sysname to generate valid configurations beyond the training manifold and to better handle complex, structured configuration spaces.

% From Table~\ref{tab:be-great-comp-summary}, we observe that: (1) for \modify queries, \sysname changes far fewer features on average than \tabcf, and (2) \tabcf fails to produce configurations in several cases, while \sysname succeeds consistently. The reason behind \tabcf failing that it enforces configurations to stay on the learned data manifold through its Variational Auto-Encoder(VAE) latent space, simultaneously optimizing validity, proximity, and latent proximity losses. When the predictive model's target range exists only in off-manifold regions, \tabcf cannot reconcile staying in high-density areas while achieving the prediction target, causing it to fail. On the other hand, \sysname operates directly in feature space without inherent manifold constraints, using gradient-based or search methods that prioritize reaching the target prediction and proximity to the original instance. This approach allows \sysname to generate configurations in off-manifold regions.
% \tabcf is designed for tabular configuration generation but relies on a rigid optimization scheme that struggles with complex, structured configuration spaces. 
% In contrast, \sysname offers a modular, constraint-aware design that easily incorporates domain knowledge into the search process.  

\input{Sections/results_summary_table2}
\input{Sections/results_recommend}

\subsection{Effectiveness of \modify}
\label{sec:modify}
\input{Sections/results_modify}

\subsection{Effectiveness of \whatif}
\label{sec:whatif}
\input{Sections/results_whatif}

\subsection{Overhead, Scalability, and Reproducibility}
\label{sec:overhead}
\input{Sections/results_overhead}
\input{Sections/results_summary}

% \subsection{Comparison new loss function}
% \input{Sections/loss_comparison_table}

% \input{Sections/validation}
\subsection{Synthetic Benchmarking for Validation}
\label{sec:validation}
\input{Sections/results-validation2}
\subsection{Applicability of \sysname for HPC Job Scheduling}
\label{sec:application}
\input{Sections/application}


==> Sections/results-sigmetrics-old.tex <==

We evaluate \sysname across \tzi{seven} scenarios:  
\begin{enumerate}
\item Validate \sysname. 
\item Evaluate the performance of different predictive models. \tzi{why?}
\item Evaluate the effectiveness of subset sampling. % in making \sysname time- and data-efficient. %show less time during the rest of the pipeline but cost is the subset sampling, the effectivenss of predictive model will be similar or better.   
    \item Evaluate the effectiveness of \reco. % in generating optimal configurations.  %are the targets truly optimal compared to the ground truth?
\item Evaluate the effectiveness of \modify. % in generating minimal edits with high confidence.  %Is this really minimal edit, truly the Ys match with the specified constraints?
\item Evaluate the effectiveness of \whatif. % in producing semantically valid changes and directional accuracy.  %What is Y? may be validate this using causal graph?
% \item Evaluate and validate \discover. % in quantifying feature sensitivity. % using causal graphs.  %Repeat the same things as the whatif s othat we can validate.
% \item Validate using the principle of self-consistency between \modify and \whatif queries.
\item Overhead analysis and scalability.


% \tzi{@Banooqa: Using synthetic datasets}

\end{enumerate}

\input{Sections/results_summary_table2}
\input{Sections/results_subset_sampling}
\input{Sections/results_recommend}
\input{Sections/results_modify}
\input{Sections/results_whatif}
\input{Sections/results_model_performance}

% \input{Sections/results_discover}


\input{Sections/results_overhead}
\input{Sections/results_validate}

\tzi{Summary of the lessons: Add a summary table that lists the first sentence of the narratives -- @Ankur}

% \input{Sections/validation}

==> Sections/results.tex <==
\subsection{Recommendation: Recommend me a <configuration> where \texttt{duration} is optimal and \texttt{exit state} is $user\_given\_state$}

\begin{figure*}[!h]
    \centering
    \subfigure[]{\i
    \includegraphics[width=0.28\textwidth]{Figs/fugaku/uncertainty_fugaku_0.pdf}}
    \label{fig:fugaku:uncertainity}
    \hspace{1em}
    \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/fugaku/outlier_fugaku_0.pdf}}
    \label{fig:fugaku:outlier}
    \hspace{1em}
    \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/fugaku/weighted_graph_fugaku_0.pdf}}
    \label{fig:fugaku:causal graph}
    % \vspace{-0.5em}
    \caption{Results for Fugaku Q1: (a) Uncertainty Quantification, (b) UMAP projection with outlier detection, (c) Causal graph.}
    \label{fig:fugaku}
\end{figure*}

This user query suggests to recommend some hypothetical samples on the Fugaku dataset where the duration is optimal and the exit state strictly follows a user-defined categorical value. Unlike typical numerical constraints where we match the minimum and maximum thresholds, this query introduces column fixing. Our recommendation pipeline produces 382 counterfactual samples, which are aligned with the specified constraints. Our rule-based approach validates all the samples as valid samples. This indicates that 100\% of the samples are valid with respect to user and domain constraints. We analyze the data distribution using our outlier techniques shown in ~\ref{fig:fugaku}, we observe that approximately 22.51\% of the generated samples fall out of the distribution of the training data. This is because of huge variability in the target metrics of the Fugaku dataset. Our query tries to find out the optimal, meaning the engine tries to sample from a lower density distribution.  


The uncertainty quantification (UQ) plots demonstrate an exceptionally narrow band. This indicates that the RandomForest model is highly confident in its predictions for the region, which indicates that the model maintains a high level of confidence in its predictions for the generated counterfactuals.

The causal graph indicates that this Fugaku dataset solely depends on the \texttt{idle\_time} metric, and small influenced by the \texttt{mszl}.



\subsection{Exploratory optimization: Given a base configuration <configuration>, how should I change my current configuration to achieve ${user\_percentage}$ reduction in \\$\texttt{node\_power\_consumption}?$}



\begin{figure*}[!h]
     \centering
     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/PM-100/uncertainty_PM-100_q2_what_if_mape.pdf}}
     \label{fig:pm100-q2:uq}
     \hspace{1em}
     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/PM-100/outlier_PM-100_q2_what_if.json.pdf}}
     \label{fig:pm100-q2:umap}
     \hspace{1em}
     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/PM-100/weighted_graph_PM-100_q2_what_if.pdf}}
    \label{fig:pm100-q2:causal_graph}
     \vspace{-0.5em}
     \caption{Results for PM100-Q2: (a) Uncertainty Quantification, (b) UMAP projection with outlier detection, (c) Causal graph.}
     \label{fig:pm100-q2}
 \end{figure*}

 The primary objective of the query is not to find the best solution as a recommendation from the PM-100 dataset, but also to give users flexibility to explore the configuration space in search of actionable and interpretable configurations. In response to the user query, our generation pipeline offers 1000 alternative samples which could be actionable. Our LLM validation invalidates 8 samples out of 1000 samples. This indicates that our recommendation engine may suggest those samples as valid from their search space; however, they fail to meet the minimum $complience\_score$. 

 Although the rule validation pipeline accepts almost all samples, \ref{fig:pm100-q2} indicates 181 samples out of 1000 samples are outliers. This indicates that a portion of generated data lies in low-density or less represented regions of the original data. This is logical as the rule-based generation method is designed to meet specific constraints or logical conditions — but it may not consider the underlying data distribution. In Figure \ref{fig:pm100-q2:uq} uncertainty quantification suggests a moderate stability of the model, despite having some random huge spikes. That proves our generated hypothetical samples are prone to the more realistic and sophisticated samples drawn from the training distribution. 

 The causal graph suggests a complex relationship among the features and the target metric. 
 We observe that \texttt{mem\_power\_consumption} and \texttt{cpu\_power\_consumption} are both influential to the
 \\ \texttt{node\_power\_consumption}. 
 

     \begin{figure*}
     \centering
     \subfigure[uq]{
     \includegraphics[width=0.3\textwidth]{Figs/perfvar/uncertainty_perfvar_1.pdf}
    \label{fig:UQ-perfvar-q1}
     }
    \subfigure[UMAP]{
     \includegraphics[width=0.3\textwidth]{Figs/perfvar/outlier_perfvar_1.json.pdf}
     \label{fig:UQ-perfvar-q1}    
     }
     \subfigure[Causal graph]{
     \includegraphics[width=0.3\textwidth]{Figs/perfvar/weighted_graph_perfvar_1.pdf}
     \label{fig:UQ-perfvar-q1}
    }    
     \caption{SC19: (a) Uncertainty Quantification, (b) UMAP projection with outlier detection, (c) Causal graph.}
 \end{figure*}

\subsection{ Exploratory What if: Given a base configuration <configuration> what if I double the \texttt{task\_count}, what would be the \texttt{run\_time?}}

The goal of the query is to investigate the hypothetical scenarios of the SC'19 dataset. The user provides a base configuration and requests the pipeline to explore "what-if" scenarios. Upon processing the requests, our pipeline suggests 775 distinct hypothetical samples. Out of the 775 samples, our rule-based validation mechanism disapproved 16 samples. These samples failed to meet the minimum $complience\_score$ meaning the samples violate more than 50\% of the rules. Figure ~\ref{fig:UQ-perfvar-q1} shows the results of the uncertainty quantification. We see around 91.10\% of samples were confirmed to be valid and actionable. These samples not only align with the data distribution learned from the original dataset but also satisfy practical constraints, indicating high plausibility. 

However, the figure shows wide uncertainty bands in the region. This implies the RandomForest predictive model exhibits lower confidence in sample regions. \tzi{When explaining these results -- ALWAYS tie them to the quality of the counterfactuals, or the data fed to it. What does this UQ band say about out of support }

The causal graph exactly matches with our exploration. We find out that the user wants to explore the effect of  \texttt{task\_count} on runtime. We observe that \texttt{task\_count} has the highest influence on the \texttt{run\_time}, changing {task\_count} must have a potential effect on {run\_time}


% User requests the generative pipeline to generate some hypothetical scenarios with a base configuration and explore "what-if" scenarios. Our pipeline can generate 775 samples as potential hypothetical scenarios in which our rule-based approach disapproved 16 configurations. 

% From the 775 samples, Figure\ref{fig:UQ-perfvar-q1} suggests that around 91.10\% of the samples are valid. This indicates that the samples are not only from the original distribution, but also actionable. However, we see a high band suggesting the model may not be confident of being 

% The objective of the query is not only to find a single best solution or recommendation, but also to explore the configuration space in search of actionable and interpretable configurations. In response to our query, our generation pipeline offers 1000 alternative samples which could be actionable. Our rule-based validation suggests all of the samples are well-suited; each of the samples met the requirements generated by the LLM model. However, \ref{fig:pm100-q2} 181 samples out of 1000 samples are marked as outliers. This indicates that a portion of generated data lies in low-density or less represented regions of the original data. This is logical as the rule-based generation method is designed to meet specific constraints or logical conditions — but it may not consider the underlying data distribution. In Figure \ref{fig:pm100-q2:uq} uncertainty quantification suggests a moderate stability of the model, despite having some random huge spikes. That proves our generated hypothetical samples are prone to the more realistic and sophisticated samples drawn from the training distribution. In Figure ~\ref{fig:pm100-q2:causal_graph} we see that the causal relationship suggests \texttt{mem\_power\_consumption} has the most influence over the three other factors to determine the variability of \texttt{node\_power\_consumption}. 

% \tzi{     \item Exploratory What if: Given a base configuration <configuration> what if I double the \texttt{task\_count}, what would be the runtime?}

%      Out of 775 samples, around 91.10\% samples are valid.



% \subsection{Exploratory What-if Given a base configuration <configuration>, what if I increase \texttt{num\_node} by X, how would that affect my \texttt{node\_power\_consumption}?}

% \begin{figure*}[!h]
%     \centering
%     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/perfvar/uncertainty_perfvar_1.pdf}}
%     \label{fig:perfvar-q2:uq}
%     \hspace{1em}
%     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/perfvar/outlier_perfvar_1.json.pdf}}
%     \label{fig:perfvar-q2:umap}
%     \hspace{1em}
%     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/perfvar/weighted_graph_perfvar_1.pdf}}
%     \label{fig:perfvar-q2:causal_graph}
%     \vspace{-0.5em}
%     \caption{Results for Perfvar Q1: (a) Uncertainty Quantification, (b) UMAP projection with outlier detection, (c) Causal graph.}
%     \label{fig:perfvar Q1}
% \end{figure*}

% This user query focuses on an exploratory scenario on the given configuration, what amount of changes are being possible by target metrics \texttt{node\_power\_consumption} if we alter some configuration. The \ref{fig:pm100-q3:uq} suggests that the model struggles to predict as the band is moderately higher. This uniform high band suggests that the base configuration is pulled from a region where the training sample is low. However, we can find out that the band is moderately uniform, which also draws attention to being stable prediction to the hypothetical scenario. That is supported by \ref{fig:pm100-q3:umap} where we find that 27 out of 1000 samples are being identified as outliers. We can conclude that, though our generation pipeline pulls from a lower density training samples, it still can populate robust and actionable hypothetical scenarios.
% \todo{write on causal graph}



% \begin{figure*}[!h]
%     \centering
%     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/PM-100/uncertainty_PM-100_q1_rec.pdf}}
%     \hspace{1em}
%     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/PM-100/outlier_PM-100_q1_rec.json.pdf}}
%     \hspace{1em}
%     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/PM-100/weighted_graph_PM-100_q1_rec.pdf}}
%     \vspace{-0.5em}
%     \caption{Results for PM100-Q1: (a) Uncertainty Quantification, (b) UMAP projection with outlier detection, (c) Causal graph.}
%     \label{fig:pm100-q1}
% \end{figure*}

% \begin{figure*}[!h]
%     \centering
%     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/PM-100/uncertainty_PM-100_q2_what_if_mape.pdf}}
%     \label{fig:pm100-q2:uq}
%     \hspace{1em}
%     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/PM-100/outlier_PM-100_q2_what_if.json.pdf}}
%     \label{fig:pm100-q2:umap}
%     \hspace{1em}
%     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/PM-100/weighted_graph_PM-100_q2_what_if.pdf}}
%     \label{fig:pm100-q2:causal_graph}
%     \vspace{-0.5em}
%     \caption{Results for PM100-Q2: (a) Uncertainty Quantification, (b) UMAP projection with outlier detection, (c) Causal graph.}
%     \label{fig:pm100-q2}
% \end{figure*}

% \begin{figure*}[!h]
%     \centering
%     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/PM-100/uncertainty_PM-100_q3_exp_what_if.pdf}}
%     \label{fig:pm100-q3:uq}
%     \hspace{1em}
%     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/PM-100/outlier_PM-100_q3_exp_what_if.json.pdf}}
%     \label{fig:pm100-q3:umap}
%     \hspace{1em}
%     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/PM-100/weighted_graph_PM-100_q3_exp_what_if.pdf}}
%     \label{fig:pm100-q3:causal_graph}
%     \vspace{-0.5em}
%     \caption{Results for PM100-Q3: (a) Uncertainty Quantification, (b) UMAP projection with outlier detection, (c) Causal graph.}
%     \label{fig:pm100-q3}
% \end{figure*}

% \subsubsection{Recommendation: Recommend a <configuration> to achieve \texttt{runtime} less than $given\_user\_value$.}

% The objective of this query is to generate some recommendations without prior domain knowledge. As a user, we ask our generation pipeline to generate configurations where the runtime is less than a user defined value. Our generation pipeline suggested possible 971 recommendation samples for the given query. Our rule-based validation flags only 2 samples as invalid samples, i.e. the compliance score for those two samples is less than 0.5 {todo refer 3.3.1}. Uncertainty quantification (UQ) results, depicted in the leftmost plot (Figure~\ref{fig:UQ-PM100-q1}), demonstrate the reliability of the model over the generated counterfactual samples. We observe a solid uncertainty line with a narrow band suggesting that the majority of these samples fall within regions of the given input space.
% However, occasional sharp spikes in the uncertainty band suggest regions where the model’s predictive confidence is lower, likely due to sparser training data in those areas. These are expected artifacts of generative modeling, as such methods may not always reproduce high-density regions with perfect fidelity. Thus, shallow spikes do not significantly impact the overall quality of the generated samples, nor the end users, as we display to the user the best-k optimal solutions. The middle figure (Figure~\ref{fig:umap-pm100}) presents a UMAP-based visualization of the recommendation samples in relation to the original data manifold. The clear clustering and absence of outliers imply that all generated samples are plausible and lie within the intrinsic structure of the original dataset. This image suggests that our model perfectly generates 100\% actionable configurations. The rightmost causal graph Figure~\ref{fig:graph-pm100} highlights the underlying structural relationships among system-level performance metrics. Notably, variables such as \texttt{mem\_power\_consumption} and \texttt{node\_power\_consumption} emerge as strong causal predictors of \texttt{runtime}. This causal insight validates that the recommendation system not only explores realistic data regions but also aligns with the fundamental causal mechanisms governing system behavior.

% Our generation pipeline generated \todo{971} recommendation samples for the given query. The leftmost figure ~\ref{fig:UQ-PM100-q1} suggests the results of uncertainty quantification (UQ) over those generated counterfactual samples. We see a stable solid line lies in a narrow band meaning the counterfactual input presents within a well-represented region of the training data, where the model has seen similar feature combinations. However, in some points, we see larger spikes, which means the model is not that much confident on the distribution of the samples. The middle figure ~\ref{fig:umap-pm100} suggests that there are no outliers in the generated recommendation samples. Thus, we are confident that our recommendation system can generate 100\% actionable samples that lie in the feature space. The rightmost figure \ref{fig:graph-pm100} suggests power related metrics like \texttt{mem\_power\_consumption} and \texttt{node\_power\_consumption} have strong causal influence on \texttt{runtime}

% \subsubsection{Exploratory optimization: Given a base configuration <configuration>, how should I change my current configuration to achieve ${user\_percentage}$ reduction in \\$\texttt{node\_power\_consumption}?$}

% The objective of the query is not only to find a single best solution or recommendation, but also to explore the configuration space in search of actionable and interpretable configurations. In response to our query, our generation pipeline offers 1000 alternative samples which could be actionable. Our rule-based validation suggests all of the samples are well-suited; each of the samples met the requirements generated by the LLM model. However, \ref{fig:pm100-q2} 181 samples out of 1000 samples are marked as outliers. This indicates that a portion of generated data lies in low-density or less represented regions of the original data. This is logical as the rule-based generation method is designed to meet specific constraints or logical conditions — but it may not consider the underlying data distribution. In Figure \ref{fig:pm100-q2:uq} uncertainty quantification suggests a moderate stability of the model, despite having some random huge spikes. That proves our generated hypothetical samples are prone to the more realistic and sophisticated samples drawn from the training distribution. In Figure ~\ref{fig:pm100-q2:causal_graph} we see that the causal relationship suggests \texttt{mem\_power\_consumption} has the most influence over the three other factors to determine the variability of \texttt{node\_power\_consumption}. 

% rule 1000 out of 1000. 
% 181 out of 1000




% Total samples analyzed: 1000
% Outliers detected: 27 (2.70%)
% Inliers detected: 973 (97.30%)






%\subsection{Perfvar Dataset}



% \begin{figure*}[!h]
%     \centering
%     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/perfvar/uncertainty_perfvar_0.pdf}}
%     \label{fig:perfvar-q1:uq}
%     \hspace{1em}
%     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/perfvar/outlier_perfvar_0.json.pdf}}
%     \label{fig:perfvar-q1:umap}
%     \hspace{1em}
%     \subfigure[]{\includegraphics[width=0.28\textwidth]{Figs/perfvar/weighted_graph_perfvar_0.pdf}}
%     \label{fig:perfvar-q1:causal_graph}
%     \vspace{-0.5em}
%     \caption{Results for Perfvar Q1: (a) Uncertainty Quantification, (b) UMAP projection with outlier detection, (c) Causal graph.}
%     \label{fig:perfvar Q1}
% \end{figure*}





% \subsubsection{Recommendation: Recommend <configuration> to achieve runtime less than $given\_seconds$ where \texttt{algorithm == $"user\_sepecified\_algorithm"$}}



% In this query, user asks the \sysname to generate some recommended samples where a runtime is less than a user-defined number of seconds and a specific algorithm is fixed. From ~\ref{fig:perfvar-q1:uq} we see that the band is moderately stable. That indicates the model is moderately confident to predict on the hypothetical configurations. However, around 10.55\% samples are being outliers. 



% Total samples analyzed: 986
% Outliers detected: 104 (10.55%)
% Inliers detected: 882 (89.45%)

%rule mentioned 585 samples are pruned in 1000 samples. 


% \subsubsection{Exploratory What If: What if for the given configuration <configuration>, we double the \texttt{task\_count}, then what will be the hypothetical outcome(s)?}



% % \ankur{Draft: In visual representation, on the left most uncertainity figure, we can see that, Between sample IDs 0–600 we see huge band, and some moderate bands are around 1500-1700 samples. Higher band means those counterfactual samples struggles the most to predict accurately. Rest of the samples are tighten, meaning that, this counterfactual samples are more healthier to recommend. However, this doesn't affect user end, because in Graphical User Interface we will provide the best-k samples to the users, discarding the weaker samples. 

% % The middle image, violin image, plots that, the \texttt{num\_task}, \texttt{partition} and \texttt{run\_time} are positively correlated and the counterfactual data distribution is fitted into the original distribution. That being said, counterfactual strictly follow the patterns of distribution of original dataset.

% %graph description is easier, which contributes the most. ...
% %}

% % \begin{figure*}
% %     \centering
% %     \subfigure[uq]{
% %     \includegraphics[width=0.3\textwidth]{Figs/PM-100/uncertainty_PM-100_q3_exp_what_if.pdf}
% %     \label{fig:UQ-PM100-q1}
% %     }
% %     \subfigure[violin]{
% %     \includegraphics[width=0.3\textwidth]{Figs/PM-100/violin_plot_PM-100_q3_exp_what_if.pdf}
% %     \label{fig:violin-pm100}    
% %     }
% %     \subfigure[Causal graph]{
% %     \includegraphics[width=0.3\textwidth]{Figs/PM-100/weighted_graph_PM-100_q3_exp_what_if.pdf}
% %     \label{fig:graph-pm100}
% %     }    
% %     \caption{PM100-Q3}
% % \end{figure*}

% % \begin{itemize}
% %     \item Recommendation: Recommend a <configuration> to achieve \texttt{runtime} $<given\_seconds$? %translate lowest runtime --> infer from the statistics what the lowest mean.
% %     \item Exploratory optimization: Given a base configuration <configuration>, how should I change my current configuration to achieve $50\%$ reduction in \texttt{node\_power\_consumption}?
    
% %     \item Exploratory what-if: Given a base configuration <configuration>, what if I increase \texttt{num\_node} by X, %(this would mean that you add X to the existing config's num node variable, 
% %     how would that affect my \texttt{node\_power\_consumption}?
% % \end{itemize}

% \subsection{Dataset 2: Perfvar}

% \begin{itemize}
%     \item Recommendation: Recommend a <configuration> to achieve runtime less than $given\_seconds$ where \texttt{df["algorithm"] == "pak"}


%     \item Exploratory What if: Given a base configuration <configuration> what if I double the \texttt{task\_count}, what would be the runtime?

%     Out of 775 samples, around 91.10\% samples are valid.

%     \begin{figure*}
%     \centering
%     \subfigure[uq]{
%     \includegraphics[width=0.3\textwidth]{Figs/perfvar/uncertainty_perfvar_1.pdf}
%     \label{fig:UQ-perfvar-q1}
%     }
%     \subfigure[UMAP]{
%     \includegraphics[width=0.3\textwidth]{Figs/perfvar/outlier_perfvar_1.json.pdf}
%     \label{fig:UQ-perfvar-q1}    
%     }
%     \subfigure[Causal graph]{
%     \includegraphics[width=0.3\textwidth]{Figs/perfvar/weighted_graph_perfvar_1.pdf}
%     \label{fig:UQ-perfvar-q1}
%     }    
%     \caption{Perfvar Q2}
% \end{figure*}

%     \item Exploratory Optimization: Given a base configuration <configuration> where runtime is 101.62s how should I change the \texttt{task\_count} to achieve runtime less than <configuration runtime> (100s)?
% \end{itemize}









% \subsection{Recommendation: Recommend me a <configuration> where \texttt{mbwidth} is moderate and \texttt{exit state} is $user\_given\_state$}



% \begin{itemize}
%     \item Reommendation: Recommend me a <configuration> where \texttt{duration} is optimal and \texttt{exit state} is <completed/failed>
    
%     Total samples analyzed: 382
%     Outliers detected: 86 (22.51\%)

%     \begin{figure*}
%     \centering
%     \subfigure[uq]{
%     \includegraphics[width=0.3\textwidth]{Figs/fugaku/uncertainty_fugaku_0.pdf}
%     \label{fig:fugaku_uq}
%     }
%     \subfigure[violin]{
%     \includegraphics[width=0.3\textwidth]{Figs/fugaku/outlier_fugaku_1.json.pdf}
%     \label{fig:fugaku}    
%     }
%     \subfigure[Causal graph]{
%     \includegraphics[width=0.3\textwidth]{Figs/fugaku/weighted_graph_fugaku_0.pdf}
%     \label{fig:graph-pm100}
%     }    
%     \caption{Fugaku Q1}
% \end{figure*}
    
    
% \end{itemize}

% \begin{itemize}
%     \item Recommendation: Recommend a <configuration> where \texttt{mbwidth} is between <range> and \texttt{exit state} is <completed/failed>.
%     \todo{624 samples, 95.83\% are not outliers}

%      \begin{figure*}
%     \centering
%     \subfigure[uq]{
%     \includegraphics[width=0.3\textwidth]{Figs/fugaku/uncertainty_fugaku_1.pdf}
%     \label{fig:fugaku_uq}
%     }
%     \subfigure[violin]{
%     \includegraphics[width=0.3\textwidth]{Figs/fugaku/outlier_fugaku_2.json.pdf}
%     \label{fig:fugaku}    
%     }
%     \subfigure[Causal graph]{
%     \includegraphics[width=0.3\textwidth]{Figs/fugaku/weighted_graph_fugaku_1.pdf}
%     \label{fig:graph-pm100}
%     }    
%     \caption{Fugaku Q1}
% \end{figure*}
    
% \end{itemize}

% \begin{itemize}
%     \item 
% \end{itemize}

% \begin{finding}

% \begin{itemize}
%     \item The top 5 counterfactuals all have $\le 1\%$ MAPE across 
% \end{itemize}
% \end{finding}

% % \begin{figure*}
% %     \centering
% %     \subfigure[uq]{
% %     \includegraphics[width=0.3\textwidth]{Figs/PM-100/uq_band_GP_PM-100_q1_rec.pdf}
% %     \label{fig:UQ-PM100-q1}
% %     }
% %     \subfigure[violin]{
% %     \includegraphics[width=0.3\textwidth]{Figs/PM-100/violin_plot_PM-100_q1_rec.pdf}
% %     \label{fig:violin-pm100}    
% %     }
% %     \subfigure[Causal graph]{
% %     \includegraphics[width=0.3\textwidth]{Figs/PM-100/weighted_graph_PM-100_q1_rec.pdf}
% %     \label{fig:graph-pm100}
% %     }    
% %     \caption{PM100-Q1}
% % \end{figure*}

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=\columnwidth]{Figs/PM-100/violin_plot_PM-100_q1_rec.pdf}
% %     \caption{violin\_plot\_PM-100\_q1\_rec.pdf}
% %     \label{fig:uncertainty}
% % \end{figure}

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.5\columnwidth]{Figs/PM-100/weighted_graph_PM-100_q1_rec.pdf}
% %     \caption{weighted\_graph\_PM-100\_q1\_rec.pdf}
% %     \label{fig:uncertainty}
% % \end{figure}

% \subsection{Dataset 2: Power vs Runtime Usage Characteristics using F-Data}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{Figs/feature_importance_econ.png}
%     \caption{Causal Graph showing the features that affect `econ' the most. The weights are normalized.}
%     \label{fig:causal}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{Figs/uq_band_eg.png}
%     \caption{Visualizing uncertainty in predicting the runtime using a Random Forest Regressor. We see sample numbers $7$, $12$, and $14$ have more uncertainty compared to others, making them less desirable.}
%     \label{fig:uncertainty}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{Figs/violin_plot.png}
%     \caption{This plot shows three things: 1) the estimated effects of features X1, X2, and X3 on y, 2) the distribution of the real dataset vs. the synthesized samples, 3) the confidence interval of the effect estimates for both the real and synthesized samples. We see the causal relations are maintained.}
%     \label{fig:violin}
% \end{figure}



% \begin{itemize}
%     \item Add a table showing what a user would be given -- counterfactuals, the satisficing score (Runtime vs Energy consumption).
%     % \item Fig \ref{fig:causal} shows the weighted causal graph for `econ'. We see the features that has the most effect on energy consumption to `cnumut' which is the number of core used by the job, `perf1' which is the number of execution cycles, and `idle\_time\_ave' which is the average idle time of the job.
%     % \item Fig \ref{fig:uncertainty} shows uncertainty in the predicting the `outcome' of the synthesized samples by a random forest model trained on the real dataset and tested on the counterfactuals. We see that the model is able to generate samples that the predicive model is fairly confident in predicting indicating that it is close to the real dataset.
%     % UQ Band chart: A visual of the UQ of predictive models per counterfactual (shown along X axis)
%     \item Radar chart: top 5 satisficing counterfactuals for users to see which one leads to increase in Performance vs Energy consumption.
%     % \item Fig \ref{fig:violin} shows similar distribution, confidence intervals, and effect estimates of the real and synthesized samples indicating the causal relationships discovered in the real dataset are maintained within the synthesized samples.  
%     % UQ of relationships -- violin chart
%     \item Explanation -- \tzi{@Ankur finish your rule generation, and @banooqa finish your table generation and then give the table to Ankur. @Ankur will then use the table and the rules to generate a concrete explanation.}
% \end{itemize}
% \banooqa{Figure \ref{fig:causal} presents the weighted causal graph for the target variable econ. The analysis identifies `cnumut' (the number of cores utilized), `perf1' (the number of execution cycles), and idle\_time\_ave (the average idle time) as the most influential factors affecting energy consumption.}

% \banooqa{Figure \ref{fig:uncertainty} reports the predictive uncertainty of a gaussian process model trained on the original dataset and evaluated on the synthesized counterfactual samples. The low uncertainty observed suggests that the generated samples closely resemble the real data distribution, enabling the predictive model to generalize effectively.}

% \banooqa{Figure \ref{fig:violin} compares the distributions, confidence intervals, and causal effect estimates between the original and synthesized datasets. The strong agreement across these metrics indicates that the synthesized samples preserve the underlying causal relationships discovered in the real data.}

% \subsection{Dataset 3: Decision Support for Achieving Performance and Variability Trade-Off}
% Runtime and Performance Variability

% \subsection{Dataset 4: Decision Support for Autotuners}


% \subsection{Dataset 5: Decision Support for Failures/Classification}


% \subsection{Single-Source Exploratory Analysis}
% Output\_sorted Here are some of my observations:
% \begin{itemize}
%     \item When `Region' and `Runtime' are ignored and `abs\_variation' is used as target, we do not see any tangible pattern or relation.
%     \item When `variation' and `abs\_variation' are ignored  and `Runtime' is used as the target, we see region explains $93\%$ variance in Runtime.
%         \begin{itemize}
%             \item When filtered for region = 0 and analyze, I see withing this kernel: num\_sample explains $56.91\%$ of variance in runtime, num\_epochs\_agent explains $20.30\%$ of variance in runtime, num\_mult\_outlier explains $20.35\%$ of variance in runtime, and runtime explains $2.43\%$ of variance in runtime (that is the variance that none of the features account for)
%             \item When filtered for region = 1, 
%         \end{itemize}
% \end{itemize}
% \begin{finding}
% bla bla
% \end{finding}



% \subsection{LLM Explanation}

% Our end goal is to demonstrate a human-readable explanation of the generated counterfactual. In the graphical user interface, we show the user the top K configurations from the induced configurations; by default, we set $K=5$. To extend our work in the future, we will provide this value configurable by the user. We compute a hybrid approach to determine each sample. To do this, we first sort the configurations based on the distance calculated on the predictive model. This ensures the most optimal solutions to be analyzed first. Once we sort the configurations, we then compute the satisfactory score based on the provided user constraints. We hypothesize that the lower the satisfactory score, the more optimal the outcome, which aligns with one of the key objectives of High Performance Computing: achieving the best performance with minimal resources.

% We choose top-k configurations effectively ensuring that we present users with the most optimal and resource-efficient options. We provide the top-k recommendation and the user query to a Large Language Model(LLM) to generate comprehensive, human-readable explanations detailing why each configuration was chosen. Leveraging the robust interpretative capabilities of LLMs, we provide users with clear insights and justification for each recommendation, facilitating informed decision-making. We use OpenAI models \todo{CITE HERE} to generate the explanation. In the future, we want to provide flexibility to the users to use their own pre-trained LLM model, which will enable seamless integration of an alternative LLM model to provide more customized and robust LLM responses.

==> Sections/results_discover.tex <==
\subsection{Effectiveness and Validation of \discover}
% \begin{figure}[t]
%      \centering
%      \includegraphics[width=\textwidth]{Figs/causal-graphs/all_causal_graphs.pdf}
%      \label{fig:all_causal_graphs}
%      \caption{All causal graphs.}
% \end{figure}
\input{Sections/causal_graphs_table}

% \begin{figure}[t]
%     \centering
%     \captionsetup[subfloat]{labelformat=empty, justification=centering, font=small, skip=1pt}
%     \setlength{\tabcolsep}{2pt} % reduce horizontal spacing
%     \renewcommand{\thesubfigure}{}

%     \subfloat[PM100 MPC]{\includegraphics[width=0.18\textwidth]{Figs/causal-graphs/pm100/pm100_mpc_cpc_graph.pdf} \hspace{2pt}
%     \subfloat[PM100 NPC]{\includegraphics[width=0.18\textwidth]{Figs/causal-graphs/pm100/pm100_npc_cpc_graph.pdf}} \hspace{2pt}
%     \subfloat[Lassen]{\includegraphics[width=0.18\textwidth]{Figs/causal-graphs/fugaku/fugaku_graph2.pdf}} \hspace{2pt}
%     \subfloat[Monet]{\includegraphics[width=0.18\textwidth]{Figs/causal-graphs/monet/monet_cg.pdf}} \hspace{2pt}
%     \subfloat[CoMD]{\includegraphics[width=0.18\textwidth]{Figs/causal-graphs/sc19/comd.pdf}} \\[-3pt]

%     \subfloat[FT]{\includegraphics[width=0.18\textwidth]{Figs/causal-graphs/sc19/ft.pdf}} \hspace{2pt}
%     \subfloat[Kripke]{\includegraphics[width=0.18\textwidth]{Figs/causal-graphs/sc19/kripke.pdf}} \hspace{2pt}
%     \subfloat[LU]{\includegraphics[width=0.18\textwidth]{Figs/causal-graphs/sc19/lu.pdf}} 
%     % \hspace{2pt}
%     % \subfloat[]{\includegraphics[width=0.18\textwidth]{figs/fig9.pdf}} \hspace{2pt}
%     % \subfloat[]{\includegraphics[width=0.18\textwidth]{figs/fig10.pdf}} 

%     \caption{Causal graphs across all 10 datasets. Arrows represent directional influence.}
%     \label{fig:causal-graphs-grid}
% \end{figure}

This experiment evaluates whether \sysname can correctly discover and quantify which features most strongly influence a given performance target and in which direction (increases or decreases). 
%
The research question is:  
\textit{Can \sysname identify valid causal relationships between features and performance metrics, even under sub-sampling?}
%
% \textbf{Baseline}  
There is no direct baseline for this task, as existing methods do not jointly perform subset sampling, generate counterfactuals, and quantify causal influences. 
% To validate correctness, we use published empirical observations from the corresponding research papers accompanying the datasets such as the Patki et. al's SC'19 paper on a performance reproducibility study~\cite{patki2019performance}.

% \textbf{Setup}  
% We use \sysname’s causal discovery module to estimate causal graphs from the subset-sampled data. These graphs are constructed using pairwise conditional independence tests and refined with domain constraints. Feature influence scores are then derived from path-based impact propagation on the estimated graph.  
%
We validate the observed relationships by checking whether high-sensitivity features and their directional effects align with known results. For example, Patki et. al~\cite{patki2019performance} report that for the FT benchmark, changing the \texttt{algorithm} parameter from \texttt{pak} to \texttt{rand} increases runtime variation due to communication overhead, while CoMD (a compute-bound app) is unaffected. We expect \sysname’s graph to capture this difference.

\textbf{Dataset Used}  
This experiment uses all datasets listed in Table~\ref{tab:datasets}. Figure~\ref{fig:all_causal_graphs} shows the estimated causal graphs generated by \sysname for each dataset.

\textbf{Observations}  
From Figure~\ref{fig:all_causal_graphs}, we observe that:
(1) \sysname identifies a small number of features with strong influence over performance targets across all datasets. To our knowledge, \sysname is the first such tool in HPC to also quantify the impact of a unit change in one configuration parameter in increasing (black) or decreasing (red) the performance metric. The value inside the light blue nodes specify what 1 unit for each feature corresponds to.
(2) On SC19’s FT dataset, \texttt{algorithm} is ranked as the most influential feature on runtime variance, matching the 14\% variance increase observed in SC19 when changing it from \texttt{pak} to \texttt{rand}.  
(3) The same feature (\texttt{algorithm}) shows low influence for CoMD, confirming that \sysname can distinguish between compute-bound and communication-bound behaviors.  
(5) The direction of influence (e.g., increasing \texttt{num\_cores} reduces \texttt{run\_time}) matches known causal patterns in HPC scheduling, confirming the graphs are not just correlated but causally valid.


\begin{table}[t]
\centering
% \tiny
\caption{Top three causal feature-to-target relationships discovered by \sysname for each dataset. Black arrows indicate increase, red arrows indicate decrease. \tzi{Is this final? are we only going to talk about 3 apps? This is discover, right? so more apps?}}
\resizebox{\textwidth}{!}{
\begin{tabular}{|p{2.5cm}|p{4cm}|p{4cm}|p{4cm}|}
\hline
\textbf{Dataset} & \textbf{Top-1 Causal Relationship} & \textbf{Top-2 Causal Relationship} & \textbf{Top-3 Causal Relationship} \\
\hline

PM-100 & 
\textcolor{black}{\texttt{num\_cores\_req} $\uparrow$ $\rightarrow$ \texttt{cpu\_power} $\uparrow$ (12.3\%)} & 
{\texttt{time\_limit} $\downarrow$ $\rightarrow$ \texttt{run\_time} $\downarrow$ (17.8\%)} & 
\textcolor{black}{\texttt{mem\_req} $\uparrow$ $\rightarrow$ \texttt{cpu\_power} $\uparrow$ (6.5\%)} \\
\hline

CoMD & 
\textcolor{black}{\texttt{num\_tasks} $\uparrow$ $\rightarrow$ \texttt{run\_time} $\uparrow$ (11.2\%)} & 
{\texttt{num\_nodes\_req} $\downarrow$ $\rightarrow$ \texttt{cpu\_power} $\downarrow$ (9.4\%)} & 
\textcolor{black}{\texttt{mem\_alloc} $\uparrow$ $\rightarrow$ \texttt{cpu\_power} $\uparrow$ (7.1\%)} \\
\hline

FT & 
\textcolor{black}{\texttt{algorithm = rand} $\rightarrow$ \texttt{run\_time} $\uparrow$ (14.0\%)} & 
{\texttt{mem\_req} $\downarrow$ $\rightarrow$ \texttt{run\_time} $\downarrow$ (6.8\%)} & 
\textcolor{black}{\texttt{num\_nodes\_req} $\uparrow$ $\rightarrow$ \texttt{cpu\_power} $\uparrow$ (10.3\%)} \\
\hline

\end{tabular}
}
\label{tab:causal-summary}
\end{table}


==> Sections/results_feasibility_sc26.tex <==
% \begin{table}[!t]
% \tiny
% \caption{Constraint satisfaction results. Each method generates $n=5$ samples per dataset. We report the percentage of samples that \tzi{respected all the domain constraints specified in the user query} ($\uparrow$ higher is better).}
% \label{tab:domain_constraints}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|c|}
% \hline
% \textbf{Dataset} & \textbf{\#Constr.} 
% & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{D} & \textbf{E} & \textbf{F} \\
% \hline

% \multicolumn{8}{|c|}{\tablecellbl{\textbf{\reco}}} \\ \hline
% Dataset A & 12 
% & \tablecellhl{100.000} 
% & 60
% & 40 
% & 40 
% & 20
% & 40 \\
% \hline
% Dataset B & 15 
% & \tablecellhl{100.000} 
% & 40 
% & 40 
% & 20 
% & 20 
% & 40 \\
% \hline
% Dataset C & 10 
% & \tablecellhl{100.000} 
% & 60 
% & 40.000 
% & 40.000 
% & 20.000 
% & 40.000 \\
% \hline
% Dataset D & 14 
% & \tablecellhl{100.000} 
% & 60.000 
% & 40.000 
% & 40.000 
% & 20.000 
% & 40.000 \\
% \hline
% Dataset E & 13 
% & \tablecellhl{100.000} 
% & 40.000 
% & 40.000 
% & 20.000 
% & 20.000 
% & 40.000 \\
% \hline
% Dataset F & 11 
% & \tablecellhl{100.000} 
% & 60.000 
% & 40.000 
% & 40.000 
% & 20.000 
% & 40.000 \\
% \hline
% Dataset G & 15 
% & \tablecellhl{100.000} 
% & 40.000 
% & 40.000 
% & 20.000 
% & 20.000 
% & 40.000 \\
% \hline
% \end{tabular}
% }
% \end{table}

==> Sections/results_overhead_sc26.tex <==
% \input{Sections/table_time_comparison}
% This experiment evaluates the runtime overhead of \sysname across different query types. For the largest dataset, Monet, sampling took $\sim1.17$ seconds; 
% % Table~\ref{tab:subset-results} reports the one-time cost of subset sampling in seconds
% this cost is excluded from per-query timing since it is amortized over many runs. None of the datasets to which sampling was applied exceeded two seconds for this process. We also note that Algorithm~\ref{alg:assess_reliability} is applied only to the top $5$ configuration suggestions, making the reliability assessment overhead negligible.
%

% Table ~\ref{tab:time_comparison} demonstrates the runtime comparison between \sysname and \tzi{NUM BASELINES} across all the datasets and all the queries we perform. We execute experiment \tzi{MY\_VALUE} times and report their average runtime and the variance. \tzi{How to mention that begreat taking 2h so we can't check their variance? or may be add "value +/-inf" in the table?}  \sysname achieves the lowest execution time in \tzi{MY\_VALUE} in \tzi{MY\_VALUE\_TOTAL experiments}. Table \ref{tab:be-great-comp-summary} shows that several baseline methods fail to generate valid configurations for a subset of datasets. In these cases, we report the total execution time until termination, capturing the cost incurred before concluding failure.

% Table ~\ref{tab:time_comparison} also \tzi{finds --> not finds, but shows} that \tzi{Which one second best baseline than Compass} is the second best pipeline in terms of generating configuration. However, we see that we perform better \tzi{MY\_VALUE}\% than the second best. In addition to that performance, \sysname shows stable behavior across repeated executions. The deviation  \tzi{MY\_VALUE} is low compared to the other methods \tzi{Mention method a, b, c}. This also suggests that the configuration generation of \sysname is robust and demonstrates minimal run-to-run variability. 



==> Sections/results_subset_sampling.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figs/subset_facs.pdf}
    \caption{We see that the subsets generated are able to maintain the downstream performance of a predictive model. 
    % \tzi{still says fugaku}
    }
    \label{fig:subset_results}
\end{figure}
This experiment studies the sensitivity of the surrogate models to the subset sampling strategy. 
We compare uniform random sampling with loss-proportional subsampling~\cite{mineiro2013loss}, which preferentially retains high-loss samples to preserve informative, hard-to-model regions.
For an independent assessment, we train an \xgb model that is different from \sysname's surrogate architectures (Section~\ref{sec:result-surrogate}).
Models are trained on three datasets---the full dataset, a loss-proportionally sampled subset, and a randomly sampled subset---and evaluated on the same held-out test set using identical hyperparameters to ensure a fair comparison. The X-axis in Figure~\ref{fig:subset_results} shows the fraction of the dataset used, Table~\ref{tab:subset-results} provides the corresponding number of samples, and the Y-axis reports \emph{normalized} MAPE, i.e., $\text{MAPE}(\text{variant})/\text{MAPE}(\text{full})$, so values near $1$ indicate training on the full dataset.
% The research question is: \textit{Can we significantly reduce the dataset size while maintaining or improving predictive modeling performance?} 
% \tzi{X axis, Y axis, why did you choose the histogram-based gradient boosting model?}
% We compare random sampling with loss-proportional subsampling~\cite{mineiro2013lossproportionalsubsamplingsubsequenterm}, which biases selection toward high-loss samples to preserve informative, hard-to-model regions.% We compare intelligent sampling with widely used random sampling strategy. 
% For independent evaluation, we train an \xgb model, which is distinct from the surrogate model architectures used by \sysname. We train these models on three scenarios: the full dataset, the intelligently selected subset, and a randomly selected subset. All models were evaluated on the same held-out test data and trained with identical hyperparameters for fair evaluation. %This ensures that any differences in accuracy are due to the selected data, not differences in model design or tuning.

% \noindent
\textbf{Observation}
From Figure~\ref{fig:subset_results}, we observe that:
(1) Except for PM-100, loss-proportional subsampling yields substantially higher normalized MAPE than uniform random sampling across subset fractions, implying worse generalization. literature \tzi{MISSING} ~\cite{mineiro2013loss} shows that over-emphasizing high-loss samples can oversample rare, noisy, or outlier regions and distort the empirical distribution, increasing variance and degrading performance when the learner is not reweighted to correct the induced sampling bias later. 
(2) Uniform random sampling is consistently stable across datasets and closely tracks the full-data baseline over a wide range of subset fractions.
Based on these observations, we use a $40\%$ subset fraction and default to uniform random sampling in subsequent experiments since it is also the fastest to compute (seconds even at the largest scale), whereas loss-proportional selection incurs additional overhead.

% Figure \ref{fig:subset_results} summarizes results across all datasets. \sysname achieves up to 95\% sample reduction across $4$ datasets with sample sizes from $100k$ to $1 mil$ while maintaining or improving predictive accuracy. This improvement occurs because our loss-guided sampling prioritizes informative, hard-to-learn configurations rather than uniformly sampling redundant data. Consequently, \sysname-selected subsets preserve critical structure in the feature space and yield lower uncertainty during prediction of hard samples than random baselines. These results show that loss-guided subset selection is both efficient and reliable, making it the default choice for large datasets. For smaller datasets, we instead use the full data to ensure that enough samples are available to train accurate models. 
% % \tzi{Specify the size threshold (e.g., X MB or N samples).}

==> Sections/results_summary.tex <==
% \subsection{Discussions}
% \label{sec:discussion}

% Across all experiments, \sysname consistently improves predictive accuracy and reduces MAPE compared to baselines, confirming that counterfactual reasoning enhances the precision of performance recommendations. Its hybrid-parallel design scales efficiently to datasets exceeding one billion samples using Dask and MPI, demonstrating practicality for large HPC workloads. \tzi{Low OOD \& UQ scores} further validate the trustworthiness of \sysname's outputs, showing that generated recommendations remain realistic and data-consistent. However, the current implementation supports only tabular numerical and categorical features with static surrogate models. Future extensions will incorporate multi-modal traces, transformer-based surrogates, and causal structure learning to improve generalization and expressiveness for complex HPC workflows.
% % \subsection{Query and Responses}
% Table~\ref{tab:results-appendix} summarizes all queries issued to \sysname and the responses received for all datasets.
% \input{Sections/appendix3}


==> Sections/results_summary_table.tex <==
\begin{table}[t]
\centering
\tiny
\caption{Summary of counterfactual quality metrics across query types. For NLL, OOS, OOD, MD}
\label{tab:results-summary}
\resizebox{\textwidth}{!}{
\begin{tabular}{|p{1cm}|p{1.cm}|p{2.5cm}|p{2.5cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1.5cm}|}
\hline
\textbf{Query Type} & \textbf{Dataset} & \textbf{UQ-sample} & \textbf{MAPE} $\uparrow$ & \textbf{NLL} $\downarrow$ & \textbf{OOS} $\downarrow$ & \textbf{OOD} $\downarrow$ & \textbf{MD} $\downarrow$ & \textbf{Confidence} \\
\hline

\multirow{3}{*}{\reco} 
& PM-100  & \parbox{2.5cm}{'node\_power' $\pm$ 0.33, 'cpu\_power' $\pm$ 0.37, 'mem\_power' $\pm$ 0.40} &  &  &  &  &  &  Very high \\ \cline{2-9}
& Monet & +-std &  &  &  &  &  & Very high \\ \cline{2-9}
& Fugaku & +-std &  &  &  &  &  &  Very high\\ \cline{2-9}
& CoMD & +-std &  &  &  &  &  &  Very high\\ \cline{2-9}
& FT & +-std &  &  &  &  &  &  Very high\\\cline{2-9}
& BUTTER-E &\parbox{2.5cm}{'power' $\pm$ 0.09, 'run\_time' $\pm$ 0.04} & \parbox{2.5cm}{'xgboost': 0.04, 'lightgbm': 0.006, 'RandomForest': 0.015} & 0.00 & 0.00 & 0.00 & 0.09  &  Very high \\\cline{2-9}
& Lassen & +-std &  &  &  &  &  &  Very high\\
\hline

\multirow{3}{*}{\modify} 
& PM-100  &\parbox{2.5cm}{'node\_power' $\pm$ 0.10, 'cpu\_power' $\pm$ 0.08, 'mem\_power' $\pm$ 0.19} & \parbox{2.5cm}{'xgboost': 0.30, 'lightgbm': 0.31, 'RandomForest': 0.32} & 0.02 & 0.17 & 0.04 &  &  Very high \\ \cline{2-9}
& Monet & +-std &  &  &  &  &  & Very high \\ \cline{2-9}
& Fugaku & +-std &  &  &  &  &  &  Very high\\ \cline{2-9}
& CoMD & +-std &  &  &  &  &  &  Very high\\
& FT & +-std &  &  &  &  &  &  Very high\\
& BUTTER-E & \parbox{2.5cm}{'power' $\pm$ 0.02, 'run_time' $\pm$ 0.02} & \parbox{2.5cm}{'xgboost': 0.04, 'lightgbm': 0.03, 'RandomForest': 0.03} & 0.01 & 0.03 & 0.00  &  &  High\\
& Lassen & +-std &  &  &  &  &  &  Very high\\
\hline


\multirow{3}{*}{\whatif} 
& PM-100  & \parbox{2.5cm}{'node\_power' $\pm$ 0.001, 'cpu\_power' $\pm$ 0.003, 'mem\_power' $\pm$ 0.0003} & \parbox{2.5cm}{'xgboost': 0.9, 'lightgbm': 0.33, 'RandomForest': 0.40} & 0.00 & 0.00 & 0.00  &  &  Very high \\ \cline{2-9}
& Monet & +-std &  &  &  &  &  & Very high \\ \cline{2-9}
& Fugaku & +-std &  &  &  &  &  &  Very high\\ \cline{2-9}
& CoMD & +-std &  &  &  &  &  &  Very high\\
& FT & +-std &  &  &  &  &  &  Very high\\
& BUTTER-E & \parbox{2.5cm}{'power' $\pm$ 0.02, 'run_time': 0.02} & \parbox{2.5cm}{'xgboost': 0.04, 'lightgbm': 0.04, 'RandomForest': 0.05} & 0.01 & 0.03 & 0.00  &  &  Very high\\
& Lassen & +-std &  &  &  &  &  &  Very high\\
\hline

\end{tabular}
}
\end{table}


==> Sections/results_validate.tex <==
\subsection{Validate \sysname}
++To assess the fidelity of \sysname, we evaluate its outputs against a set of analytically defined, noise-free performance datasets derived from canonical HPC models. The test suite comprised five benchmark functions (MILC, HOMME–MPI\_Reduce (small and large configurations), HOMME–Vlaplace, Sweep3D) and one communication-centric model based on Hoefler’s Equation~\ref{}. Table~\ref{tab:syn-mape} summarizes the validation results.

For each dataset, we report the minimum APE achieved across all samples as a measure of deterministic accuracy under ideal conditions (since the data are noise-free). Low minimum-APE values (typically below 1–2\%) indicate that \sysname can reproduce the analytical relationship between input features and runtime with high numerical precision. Such results suggest the model has successfully captured both the functional structure (e.g., logarithmic or polynomial scaling) and the magnitude relationships present in the underlying equations. Conversely, higher minimum-APE values imply residual functional mismatches—often arising in datasets with more complex composite behaviors (e.g., mixed $\sqrt{p}$ and $p^{3}$ terms in HOMME) or multidimensional dependencies (as in Hoefler’s communication model). Consistently low errors across diverse functional forms demonstrate good generalization across performance regimes, whereas selective degradation on certain kernels indicates where the model’s internal representation may require targeted refinement or additional conditioning on domain variables. Table \ref{tab:syn-mape} reports the minimum APE for each dataset. We see that \sysname consistently produces sample that give APE between $1 \& 3\%$

==> Sections/scalability.tex <==
\begin{itemize}
    \item \textit{Select two datasets and log all the overheads for the following}
    \item \textit{report subset sampling + model training + generation pipeline}
    \item \textit{Generate 5K counterfactuals using 256, 128, 64, 32 ranks}
    \item \textit{Generate figure alike SSDBM poster}
    \item \textit{Discussion will include different HPC scalability context, bottlenecks etc.}
\end{itemize}






==> Sections/syn_val.tex <==
Validating \sysname requires a known reference for comparison, yet real-world counterfactuals cannot be observed or executed directly. 
To ensure that \sysname's recommendations modeling methodology is valid, we adopt a synthetic benchmarking strategy where both inputs and outcomes are controlled. 
This approach, inspired by prior work in causal discovery, reinforcement learning, and visual reasoning~\cite{cobbe2020leveragingproceduralgenerationbenchmark, zheng2018estimating, yu2019learning, johnson2016clevrdiagnosticdatasetcompositional, luo2025automateseehiddenpitfalls}, provides measurable ground truth for assessing counterfactual accuracy. 
In addition, we use analytical performance models from HPC literature~\cite{calotoiu2013using} as interpretable surrogates, allowing us to validate whether generated recommendations align with known non-linear performance relationships. 
Together, these controlled experiments validate the soundness of \sysname’s modeling methodology for generating accurate and plausible counterfactuals.
%
% Using these datasets, \sysname generates counterfactual recommendations and computes ground-truth outcomes based on the known generating equations. 
We measure accuracy using the per-sample Absolute Percentage Error (APE), defined as 
$\text{APE} = \frac{\lvert \text{Actual} - \text{Forecast} \rvert}{\max\!\big(\lvert \text{Actual} \rvert, 10^{-8}\big)} \times 100$. 
% Table~\ref{tab:syn-mape} reports the minimum APE across datasets, demonstrating the precision of \sysname’s top-ranked recommendations relative to the ground truth.
The results in Table~\ref{tab:syn-mape} validate \sysname's modeling methodology. 
Across both linear and non-linear synthetic performance-models from representative HPC kernels--\sysname achieves below 5\% minimum APE, confirming that its best configuration suggestion can accurately capture performance relationships. The selected analytical models--spanning communication-intensive (MPI), memory-limited (Sweep3D), and compute-parameterized (linear synthetic) functions--cover the dominant scaling behaviors in HPC. %To further demonstrate generality, we also validate against Roofline and Amdahl-law surrogates, confirming that \sysname accurately models both communication- and compute-bound regimes.

% Evaluating counterfactual generation models poses a fundamental challenge: ground truth counterfactuals are rarely observable in real-world data. Unlike supervised learning tasks, where labels provide direct feedback, counterfactual reasoning involves hypothetical scenarios that cannot be empirically validated. This absence of ground truth makes it difficult to quantify model performance in a rigorous and reproducible manner. To address this challenge, we adopt a synthetic benchmarking approach inspired by prior work in causal discovery, reinforcement learning, and visual reasoning \cite{cobbe2020leveragingproceduralgenerationbenchmark, zheng2018estimating, yu2019learning, johnson2016clevrdiagnosticdatasetcompositional}, as well as recent efforts such as \cite{luo2025automateseehiddenpitfalls}. In addition to creating synthetic linear datasets, we use the work done by Calotoiu
% et al. to create synthetic performance datasets \cite{calotoiu2013using}. 
% % Specifically, we construct datasets from noise-free structural equation models (SEMs), ensuring that the true causal mechanisms and counterfactual mappings are known. This enables us to quantify fidelity, proximity, and plausibility of generated counterfactuals relative to the ground truth.
% By controlling for noise and confounding, synthetic benchmarks provide a deterministic environment in which counterfactual quality can be measured objectively.

% Once the synthetic datasets are generated, we employ \sysname to produce counterfactual samples for each dataset. For evaluation, we compute the ground-truth outcome Y based on the generated features and subsequently assess the accuracy of the counterfactual predictions using the per-sample Absolute Percentage Error (APE), defined as $
% \text{APE} = \frac{\lvert \text{Actual} - \text{Forecast} \rvert}{\max\!\big(\lvert \text{Actual} \rvert, 10^{-8}\big)} \times 100$.
% %To ensure robustness, we report the minimum APE achieved across these datasets. 
% Table~\ref{tab:syn-mape} reports the minimum APE achieved to demonstreate how acccurate \sysname's top recommendation is, all the synthesized datasets used along with the equations used to generate them.

% Following synthetic validation, we deploy our counterfactual generation model on real-world datasets where ground truth counterfactuals are not available. For those datasets, we employ uncertainty quantification to estimate the closeness of the produced counterfactuals to the real dataset. The rationale is twofold:
% \begin{itemize}
%     \item Synthetic evaluation acts as a calibration step, ensuring the model recovers correct transformations when ground truth is known.
%     \item Real-world deployment then tests generalizability, examining whether the model produces interpretable and actionable counterfactuals under realistic data conditions.
% \end{itemize}
% This two-stage evaluation balances rigor (via deterministic benchmarks) with practical utility (via real datasets), enabling us to build confidence in model outputs even in the absence of direct counterfactual labels.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{tabularx}

\begin{table*}[h!]
\tiny
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabularx}{\textwidth}{|p{2.5cm}|c|c|c|X|}
\hline
\textbf{Dataset} & \# Samples  & Model Used & APE (\%) & \textbf{Description} \\
\hline
\rowcolor[HTML]{E3F2FD}
\multicolumn{5}{|c|}{\textbf{Performance Models}} \\
\hline
\parbox[c]{3.0cm}{MILC \\ (MPI\_Allreduce)} & 4749 &  &  & Inputs: number of processes $p$; Output: runtime $t(p)$; defined by $t(p) = 6.3\times10^{-6}\log_2(p)$; valid for $p \ge 64$. \\
\hline
\parbox[c]{3.0cm}{HOMME--MPI\_Reduce \\ (small)} & 4749  &  &  & Inputs: $p$; Output: runtime $t(p) = 0.026 + 2.53\times10^{-6}\sqrt{p} + 1.24\times10^{-12}p^3$; valid for $p \in [64, 131072]$. \\
\hline
\parbox[c]{3.0cm}{HOMME--MPI\_Reduce \\ (large)} & 4749 &  &  & Inputs: $p$; Output: runtime $t(p) = 2.60\times10^{-2}\sqrt{p} + 1.17\times10^{-12}p^3$; valid for $p \ge 64$. \\
\hline
HOMME--Vlaplace & 4749  &  &  & Inputs: $p$; Output: runtime $t(p) = 0.034 + 1.33\times10^{-10}p^2$; $p \in [64, 131072]$. \\
\hline
Sweep3D Wavefront & 4749 &  & 0.014  & Inputs: $p$; Output: runtime $t(p) = c\sqrt{p}$, where $c$ is a kernel-dependent constant; $p \ge 64$. \\
\hline
\parbox[c]{3.0cm}{Hoefler Eq. 2.2 \\ (Communication)} & 6174 &  & 9.6e-4 & Inputs: grid dimensions $p_x, p_y$ and number of sweeps $n_{\text{sweep}}$; Output: communication time $t_{\text{comm}} = [2(p_x + p_y - 2) + 4(n_{\text{sweep}} - 1)]\,t_{\text{msg}}$, where $t_{\text{msg}}$ is time per message; all inputs $\in [4,512]$. \\
\hline
\rowcolor[HTML]{FFF3E0}
\multicolumn{5}{|c|}{\textbf{Analytical Models}} \\
\hline
\parbox[c]{3.0cm}{Roofline Model \\ (Compute--Memory Bound)} & 10,000 &  &  & Input: operational intensity $I$ (FLOPs per byte); Output: achievable performance $y = \min(P_{\text{peak}}, B I)$, where $P_{\text{peak}}$ is peak FLOP/s and $B$ is memory bandwidth (bytes/s); $I > 0$. \\
\hline
I/O Throughput Model & 3881 &  &  & Input: number of concurrent streams $n$; Output: throughput $y = B(1 + \alpha(n - 1))$, where $B$ is base bandwidth per stream and $\alpha$ is a scaling factor; $n \ge 1$. \\
\hline
Amdahl's Law Scaling & 7287  &  &  & Input: number of processes $p$; Output: theoretical speedup $y = \frac{1}{f + \frac{1-f}{p}}$, where $f$ is the serial fraction of the workload; $p \ge 1$. \\
\hline
\parbox[c]{3.0cm}{Roofline-Derived GPU Model \\ (Harmonic Mean)} & 10,000 &  &  & Input: operational intensity $I$; Output: performance $y = \frac{I}{1/B + 1/P}$, where $B$ is memory bandwidth and $P$ is peak compute throughput; $I > 0$. \\
\hline
\end{tabularx}
\caption{Analytical and performance model datasets used for deterministic validation of generative models. This table describes how each dataset was created and the Absolute Percentage Error (APE) in percent for the recommended configuration generated using \sysname.}
\label{tab:syn-mape}
\end{table*}


% \begin{table}[t]
% \tiny
% \caption{Analytical Performance-model-inspired synthetic datasets for validating \sysname.}
% \label{tab:syn-mape}
% \resizebox{0.48\textwidth}{!}{%
% \begin{tabular}{|l|l|l|}
% \hline
% Dataset & \begin{tabular}[c]{@{}l@{}}Equation\end{tabular} & Min APE (\%)       \\ \hline
% MILC All Reduce &  \banooqa{To be retrained} &             \\ \hline
% HOMME vlaplace  & $ y = 24.44 + 2.260e-07 * p^2$  & 3.147            \\ \hline
% \begin{tabular}[c]{@{}l@{}}HOMME MPI \\ Reduce Large\end{tabular} & \banooqa{To be retrained}   &               \\ \hline
% \begin{tabular}[c]{@{}l@{}}HOMME MPI\\ Reduce Small\end{tabular}  & \banooqa{To be retrained}  &              \\ \hline
% Sweep3D wavefront   & $y = 1.0e-6 * \sqrt{p}$ & 0.014  \\ \hline
% Tcomm      &  & 9.609e-4 \\ \hline
% Linear 10      & $y = 2.0*X3-1.5*X2+0.5*X6$ & 0.023 \\ \hline
% Linear 15 &$y = 2.0*X14-1.5*X8+0.5*X6$ & 0.076 \\ \hline
% Linear 20 & $y = 2.0*X2-1.5*X18 + 0.5*X16$ & 0.22 \\ \hline
% Linear 25 & $y = 2.0*X14-1.5*X5+0.5*X19$ & 0.305 \\ \hline
% \end{tabular}
% }

\end{table}
% \begin{figure*}[t]
% \centering
% \begin{minipage}[!htbp]{0.48\textwidth}
% \centering
% \vspace{-1.2in}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{Dataset} & \textbf{Equation} & \textbf{Min APE (\%)} \\ \hline
% MILC All Reduce & \banooqa{To be retrained} &  \\ \hline
% HOMME vlaplace & $ y = 24.44 + 2.260e^{-07} * p^2$ & 3.147 \\ \hline
% HOMME MPI Reduce Large & \banooqa{To be retrained} &  \\ \hline
% HOMME MPI Reduce Small & \banooqa{To be retrained} &  \\ \hline
% Sweep3D wavefront & $y = 1.0e^{-6} * \sqrt{p}$ & 0.014 \\ \hline
% Tcomm &  & 9.609e-4 \\ \hline
% Linear 10 & $y = 2.0*X3-1.5*X2+0.5*X6$ & 0.023 \\ \hline
% Linear 15 & $y = 2.0*X14-1.5*X8+0.5*X6$ & 0.076 \\ \hline
% Linear 20 & $y = 2.0*X2-1.5*X18 + 0.5*X16$ & 0.22 \\ \hline
% Linear 25 & $y = 2.0*X14-1.5*X5+0.5*X19$ & 0.305 \\ \hline
% \end{tabular}}
% \caption{Synthetic datasets and accuracy of top-ranked \sysname recommendations.}
% \label{tab:syn-mape}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.48\textwidth}
% \centering
% \includegraphics[width=\textwidth]{Figs/howtouse.pdf}
% \caption{Illustration of how \sysname supports both offline and online usage.}
% \label{fig:howtouse}
% \end{minipage}
% \end{figure*}


==> Sections/table_compass_begreat_bofire.tex <==
\begin{table*}[!t]
\tiny
\caption{Comparison of \sysname and transformer-based \begreat on \reco queries. \textcolor{blue}{HotPerfCloud} is a classification dataset, hence F1 score is computed and $\uparrow$ denotes, higher is better. For all other datasets, when not specified, it is }
\label{tab:be-great-comp-summary}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & 
\multicolumn{2}{c|}{$X_{train}$} &
\multicolumn{2}{c|}{\textbf{\sysname}} & \multicolumn{2}{c|}{\textbf{\begreat}} & \multicolumn{2}{c|}{\textbf{\bofire}}
& \multicolumn{2}{c|}{\textbf{DiCE}} &
\multicolumn{2}{c|}{\textbf{TABCF}}\\
\cline{2-13}
%%%%%%%%%%%%%%%%%% reco
\multicolumn{13}{|c|}{\tablecellgr{\textbf{\reco}}} \\ \hline
 & XGB & LGBM& XGB & LGBM & XGB & LGBM & XGB & LGBM & XGB & LGBM & XGB & LGBM\\
\hline
Monet  & 1.60 & 1.74 & \tablecellhl{0.73} & \tablecellhl{0.82} & 18.41 & 19.63 & 2.42 & 2.52& 2.08 & 5.123 & 9.64 & 9.65 \\ \hline
PM-100 & 0.27 & 0.32 & 0.48 & 0.47 & 3.41 & 3.51 & 0.38 & 0.37&\tablecellhl{0.32}&\tablecellhl{0.29} & \ding{56} & \ding{56}\\ \hline
BUTTER-E & 0.04 & 0.06 & {0.26} & 0.28 & 0.34 & 0.34 & \tablecellhl{0.21}& \tablecellhl{0.24}& 0.26 & 0.30& 0.38& 0.35\\ \hline
CoMD   & 0.02 & 0.04  & \tablecellhl{0.21} & \tablecellhl{0.19} & 3.42 & 3.40 & 3.02 &3.01& 0.29 & 0.33 &0.27& 0.25\\ \hline
FT    & 0.02 &  0.06  & {0.51} & {0.50} & 8.59 & 8.29 & 0.71 & 0.71& \tablecellhl{0.137} & \tablecellhl{0.23} & 0.33 & 0.34 \\ \hline
\textcolor{blue}{HotPerfCloud$\uparrow$}  & 0.70 & 0.67   & 0.47 & 0.45 &  &  &  & &0.47& 0.46&&\\ \hline
%%%%%%%%%%%%%%%%%%reconfigure
\multicolumn{13}{|c|}{\tablecellgr{\textbf{\modify}}} \\ \hline
Monet   & 9.89 & 9.87 & \tablecellhl{7.08} & \tablecellhl{7.05} & \ding{56} & \ding{56} & \cellcolor{gray!20} & \cellcolor{gray!20}&8.67&8.89&3.45&3.46 \\ \hline
PM-100  & 0.27 & 0.32 & \tablecellhl{0.57} & \tablecellhl{0.56} & & &\multicolumn{2}{c|}{\cellcolor{gray!20} {Autotuners}}&0.65&0.71& \ding{56}& \ding{56} \\ \hline
BUTTER-E & 0.04 &0.04 & \tablecellhl{0.06} & \tablecellhl{0.06} & &&\multicolumn{2}{c|}{\cellcolor{gray!20} {do not work}}&0.06&0.06&0.16& 0.16\\ \hline
CoMD   & 2.82 &  3.07 & 4.41 & 4.53 & && \cellcolor{gray!20}&\cellcolor{gray!20}&\tablecellhl{4.08}&\tablecellhl{4.12}&3.38& 3.38\\ \hline
FT    & 1.08 &  1.73  & 2.70 & 2.73 & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20}&2.70& 2.73&15.45&15.45\\ \hline
\textcolor{blue}{HotPerfCloud$\uparrow$}  & &    & & & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20}&&&&\\ \hline

%%%%%%%%%%%%%%%%%%whatif
\multicolumn{13}{|c|}{\tablecellor{\textbf{\whatif}}} \\ \hline
Monet   & 1.60  & 1.74 & \ding{56} & \ding{56}  & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20}&\ding{56}&\ding{56}&\ding{56}&\ding{56} \\ \hline
PM-100  & 0.27 & 0.32 & 13.99 & 15.36 & \multicolumn{3}{c|}{\cellcolor{gray!20} {Unconditional Generative Models}} & \cellcolor{gray!20}&13.22& 14.08&\ding{56}&\ding{56} \\ \hline
BUTTER-E & 0.04 & 0.06 & 0.04 & 0.04 & \multicolumn{3}{c|}{\cellcolor{gray!20} {and Autotuners do not perform}}& \cellcolor{gray!20}&0.04&0.04&\ding{56}&\ding{56}\\ \hline
CoMD   & 0.02 & 0.02  & 3.75 & 4.21 & \multicolumn{3}{c|}{\cellcolor{gray!20} {\whatif.}} &\cellcolor{gray!20}&3.71&4.21&\ding{56}&\ding{56}\\ \hline
FT $\downarrow$  &  1.08 & 1.73   & 3.14 & 4.72 & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20}& 3.16& 3.57& \ding{56} & \ding{56}\\ \hline
\textcolor{blue}{HotPerfCloud$\uparrow$}  &  &    & \tablecellhl{0.137} & 0.236 & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20}& \ding{56} & \ding{56}& \ding{56}& \ding{56}\\ \hline

\end{tabular}
}
\end{table*}

% \begin{table}[t]
% % \centering
% \tiny
% \caption{Comparison of \sysname and transformer-based \begreat on \reco queries. Lower MAPE indicates closer alignment with target objectives. \tzi{Either hyperparameter tune and make it consistent OR explain why compass failed to generate good recommendation for monet for lightgbm}. \tzi{Remove RF from this table.}}
% \label{tab:be-great-comp-summary}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|}

% \hline
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{c|}{\textbf{\sysname}} & \multicolumn{3}{c|}{\textbf{\begreat}} \\
% \cline{2-7}
%  & XGBoost & LightGBM & Random Forest & XGBoost & LightGBM & Random Forest \\
% \hline
% Monet & 2.08 & 5.123 & \tablecellhl{0.96} & 18.41 & 19.63 & 16.23 \\ \hline
% PM-100 & \tablecellhl{0.20} & 0.20 & 0.20 & 3.41 & 3.51 & 7.35 \\ \hline
% %Monet & 3.03 & 1.9 & 0.65 & -- & -- & -- \\ \hline
% Butter-E & 0.12 & \tablecellhl{0.012} & 0.12 & 0.34 & 0.34 & 0.34 \\ \hline
% CoMD & \tablecellhl{0.29} & 0.33 & 0.30 & 3.42 & 3.40 & 3.60 \\ \hline
% FT & \tablecellhl{0.137} & 0.236 & 0.266 & 8.59 & 8.29 & 8.06 \\ \hline
% % MIT Supercloud & -- & -- & -- & -- & -- & -- \\ \hline
% % F-Data & -- & -- & -- & -- & -- & -- \\ \hline
% % MPI I/O & 5.28e8 & 5.28e8 & \textbf{5.28e8} & 4.22e+33 & 4.55e+33 & 5.6e+32 \\ \hline
% \end{tabular}
% }
% \end{table}

==> Sections/table_compass_begreat_bofire3.tex <==
\begin{table}[t]
% \tiny
\centering
\caption{
HotPerfCloud is classification (higher is better); all others are regression (lower is better). Blue cells denote best; light blue second best. Grey indicates the method ran out of memory, exceeded 12 hours to train or infer a single suggestion, or does not perform that operation out of the box.
}
\label{tab:be-great-comp-summary}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|}
\hline
\textbf{Dataset} & 
{\textbf{Ours}} & {\textbf{\begreat}} & {\textbf{\bofire}}
&{\textbf{DiCE}} &
{\textbf{TABCF}}\\
\hline
%%%%%%%%%%%%%%%%%% reco
\multicolumn{6}{|c|}{\tablecellbl{\textbf{\reco}}} \\ 
\hline
Monet  &  \tablecellhl{0.73}  & 18.41   & 2.42 &  \multicolumn{2}{c|}{\cellcolor{gray!20}{}} \\ \cline{1-4}
PM-100 &  \tablecellhl{0.41} & 3.41 & 1.57 &\multicolumn{2}{c|}{\cellcolor{gray!20}{Do not}}\\ \cline{1-4}
BUTTER-E &  \tablecellhl{0.14} & 0.34  & 0.21 & \multicolumn{2}{c|}{\cellcolor{gray!20}perform}\\ \cline{1-4}
CoMD   & \tablecellhl{0.19}  & 3.40   &3.01& \multicolumn{2}{c|}{\cellcolor{gray!20}{\reco.}}\\ \cline{1-4}
FT    &  \tablecellhl{0.50} & 8.29 &  0.71& \multicolumn{2}{c|}{\cellcolor{gray!20}{}} \\ \cline{1-4}
\textcolor{blue}{HotPerfCloud$\uparrow$}  & \tablecellhl{0.91}  &  \cellcolor{gray!20} & 0.72 &\multicolumn{2}{c|}{\cellcolor{gray!20}{}}\\ \hline

% %%%%%%%%%%%%%%%%%%reconfigure
\multicolumn{6}{|c|}{\tablecellgr{\textbf{\modify}}} \\ \hline
Monet   & \tablecellhl{7.05} &  \multicolumn{2}{c|} {\cellcolor{gray!20}} &8.67 & 3.45 \\ \cline{1-2}\cline{5-6}
PM-100  & \tablecellhl{0.56} & \multicolumn{2}{c|} {\cellcolor{gray!20}}  &0.34& 0.81 \\ \cline{1-2}\cline{5-6}
BUTTER-E & \tablecellhl{0.06} & \multicolumn{2}{c|} {\cellcolor{gray!20}{Unable}} &0.06&0.16\\\cline{1-2}\cline{5-6}
CoMD   & 3.82 & \multicolumn{2}{c|} {\cellcolor{gray!20}to} & 3.92 &\tablecellhl{2.42}\\ \cline{1-2}\cline{5-6}
FT    & \tablecellhl{0.94}  & \multicolumn{2}{c|} {\cellcolor{gray!20}generate.} & \tablecellhl{0.94} &15.45\\ \cline{1-2}\cline{5-6}
\textcolor{blue}{HotPerfCloud$\uparrow$}  & \tablecellhl{0.91} & \multicolumn{2}{c|}{\cellcolor{gray!20}}  & 0.91  & \cellcolor{gray!20} \\ \hline

%%%%%%%%%%%%%%%%%%whatif
\multicolumn{6}{|c|}{\tablecellor{\textbf{\whatif}}} \\ \hline

Monet & \tzi{x} &\multicolumn{2}{c|} {\cellcolor{gray!20}}  & \cellcolor{gray!20} & \cellcolor{gray!20} \\ \cline{1-2}\cline{5-5}
PM-100 & \textcolor{red}{0.2438} & 
\multicolumn{2}{c|} {\cellcolor{gray!20}{Unable}} & 0.1885 & \cellcolor{gray!20} Unable \\ \cline{1-2}\cline{5-5}
BUTTER-E & \textcolor{red}{0.2750} & \multicolumn{2}{c|}{\cellcolor{gray!20}to} &  0.2750 & \cellcolor{gray!20} to  \\ \cline{1-2}\cline{5-5}
CoMD & \tablecellhl{0.3534} & \multicolumn{2}{c|}{\cellcolor{gray!20}generate.} & 0.3987 & \cellcolor{gray!20}{generate.} \\ \cline{1-2}\cline{5-5}
FT & \textcolor{red}{0.5530} & \multicolumn{2}{c|}{\cellcolor{gray!20}} & 0.5474 & \cellcolor{gray!20} \\ \cline{1-2}\cline{5-5}
\textcolor{blue}{HotPerfCloud$\uparrow$} & \tzi{x} & \multicolumn{2}{c|}{\cellcolor{gray!20}} & \cellcolor{gray!20}   & \cellcolor{gray!20} \\ \hline

\end{tabular}
}
\end{table}


==> Sections/table_compass_begreat_rmape.tex <==
\begin{table}[t]
\tiny
\centering
\caption{
All errors are weighted rMAPE (lower is better). Blue cells denote best. Grey indicates the method ran out of memory, exceeded 12 hours of training allocation time or infer a single suggestion, or does not perform that operation.}
\label{tab:be-great-comp-summary}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|}
\hline
\textbf{Dataset} & 
{\textbf{\sysname}} & {\textbf{\begreat}} & {\textbf{\bofire}}
&{\textbf{DiCE}} &
{\textbf{TABCF}}\\
\hline

\multicolumn{6}{|c|}{\tablecellbl{\textbf{\reco}}} \\ 
\hline
Monet  &    & {\cellcolor{gray!20}}   & \tablecellhl{} &  \multicolumn{2}{c|}{\cellcolor{gray!20}{}} \\ \cline{1-4}
PM-100 &  \tablecellhl{} & \cellcolor{gray!20} & \cellcolor{gray!20} &\multicolumn{2}{c|}{\cellcolor{gray!20}{Do not}}\\ \cline{1-4}
BUTTER-E &  \tablecellhl{}& {}  & {} & \multicolumn{2}{c|}{\cellcolor{gray!20}{perform}} \\ \cline{1-4}
CoMD   & \tablecellhl{$0.29\!\pm\!0.12$}  &   {\cellcolor{gray!20}} & {} & \multicolumn{2}{c|}{\cellcolor{gray!20}{\reco.}}\\ \cline{1-4}
FT    &  \tablecellhl{} & {\cellcolor{gray!20}{}} &  {} & \multicolumn{2}{c|}{\cellcolor{gray!20}{}} \\ \cline{1-4}
NPB-MZ  &  {} & {\cellcolor{gray!20}{}} & \tablecellhl{} & \multicolumn{2}{c|}{\cellcolor{gray!20}{}} \\ \cline{1-4}
\textcolor{blue}{HotPerfCloud}  & \tablecellhl{}  &  \cellcolor{gray!20} & {\cellcolor{gray!20}} &\multicolumn{2}{c|}{\cellcolor{gray!20}{}}\\ \hline

\multicolumn{6}{|c|}{\tablecellgr{\textbf{\modify}}} \\ \hline
Monet   & \tablecellhl{} &  \multicolumn{2}{c|} {\cellcolor{gray!20}} & {\cellcolor{gray!20}} & {} \\ \cline{1-2}\cline{5-6}
PM-100  &\tablecellhl{} & \multicolumn{2}{c|} {\cellcolor{gray!20}}  & {} & {} \\ \cline{1-2}\cline{5-6}
BUTTER-E & \tablecellhl{} & \multicolumn{2}{c|} {\cellcolor{gray!20}{Unable}} & {} & {} \\\cline{1-2}\cline{5-6}
CoMD   & \tablecellhl{$0.18\!\pm\!0.23$} & \multicolumn{2}{c|} {\cellcolor{gray!20}{to}} & {$0.42\!\pm\!0.34$} & {$0.97\!\pm\!0.30$} \\ \cline{1-2}\cline{5-6}
FT    & \tablecellhl{}  & \multicolumn{2}{c|} {\cellcolor{gray!20}{generate.}} & {} & {} \\ \cline{1-2}\cline{5-6}
NPB-MZ & {}  & \multicolumn{2}{c|} {\cellcolor{gray!20}} & \tablecellhl{} & {} \\ \cline{1-2}\cline{5-6}
\textcolor{blue}{HotPerfCloud}  & \tablecellhl{} & \multicolumn{2}{c|}{\cellcolor{gray!20}}  & {} & {\cellcolor{gray!20}} \\ \hline

\multicolumn{6}{|c|}{\tablecellor{\textbf{\whatif}}} \\ \hline

Monet &  \cellcolor{gray!20} &\multicolumn{2}{c|} {\cellcolor{gray!20}}  & \cellcolor{gray!20} & \cellcolor{gray!20} \\ \cline{1-2}\cline{5-5}
PM-100 & \tablecellhl{} & 
\multicolumn{2}{c|} {\cellcolor{gray!20}{Unable}} & {} & \cellcolor{gray!20} Unable \\ \cline{1-2}\cline{5-5} 
BUTTER-E & \tablecellhl{} & \multicolumn{2}{c|}{\cellcolor{gray!20}{to}} & {} & \cellcolor{gray!20} to  \\ \cline{1-2}\cline{5-5}
CoMD & \tablecellhl{} & \multicolumn{2}{c|}{\cellcolor{gray!20}{generate.}} & {} & \cellcolor{gray!20} generate. \\ \cline{1-2}\cline{5-5}
FT & \tablecellhl{} & \multicolumn{2}{c|}{\cellcolor{gray!20}} & \tablecellhl{} & \cellcolor{gray!20} \\ \cline{1-2}\cline{5-5}
NPB-MZ & {} & \multicolumn{2}{c|}{\cellcolor{gray!20}} & \tablecellhl{} & \cellcolor{gray!20} \\ \cline{1-2}\cline{5-5}
\textcolor{blue}{HotPerfCloud} & \tablecellhl{} & \multicolumn{2}{c|}{\cellcolor{gray!20}} &  {}   & \cellcolor{gray!20} \\ \hline

\end{tabular}
}
\end{table}

% \begin{table}[t]
% \tiny
% \centering
% \caption{
% All errors are weighted MAPE (lower is better). Blue cells denote best. Grey indicates the method ran out of memory, exceeded 12 hours of training allocation time or infer a single suggestion, or does not perform that operation.} % out of the box.}
% \label{tab:be-great-comp-summary}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|}
% \hline
% \textbf{Dataset} & 
% {\textbf{\sysname}} & {\textbf{\begreat}} & {\textbf{\bofire}}
% &{\textbf{DiCE}} &
% {\textbf{TABCF}}\\
% \hline
% %%%%%%%%%%%%%%%%%% reco
% \multicolumn{6}{|c|}{\tablecellbl{\textbf{\reco}}} \\ 
% \hline
% Monet  &  {$0.11\!\pm\!0.04$}  & {\cellcolor{gray!20}}   & \tablecellhl{$0.09\!\pm\!0.06$} &  \multicolumn{2}{c|}{\cellcolor{gray!20}{}} \\ \cline{1-4}
% PM-100 &  \tablecellhl{$0.09\!\pm\!0.03$} & \cellcolor{gray!20} & \cellcolor{gray!20} &\multicolumn{2}{c|}{\cellcolor{gray!20}{Do not}}\\ \cline{1-4}
% BUTTER-E &  \tablecellhl{$0.01\!\pm\!0.01$}& 6.62\!\pm\!0.00  & 1.04\!\pm\!0.20 & \multicolumn{2}{c|}{\cellcolor{gray!20}perform}\\ \cline{1-4}
% CoMD   & \tablecellhl{$0.19\!\pm\!0.11$}  &   {\cellcolor{gray!20}} & 0.44\!\pm\!0.19 & \multicolumn{2}{c|}{\cellcolor{gray!20}{\reco.}}\\ \cline{1-4}
% FT    &  \tablecellhl{$0.12\!\pm\!0.08$} & {\cellcolor{gray!20}{}} &  0.37\!\pm\!0.13 & \multicolumn{2}{c|}{\cellcolor{gray!20}{}} \\ \cline{1-4}
% % MIT  & &  \multicolumn{2}{c|}{\cellcolor{gray!20}} & \multicolumn{2}{c|}{\cellcolor{gray!20}{}}\\  \cline{1-4}
% NPB-MZ  &  {$0.17\!\pm\!0.11$} & {\cellcolor{gray!20}{}} & \tablecellhl{$0.09\!\pm\!0.09$} & \multicolumn{2}{c|}{\cellcolor{gray!20}{}} \\ \cline{1-4}
% \textcolor{blue}{HotPerfCloud}  & \tablecellhl{$2.4\mathrm{e}{-3}\!\pm\!0.00$}  &  \cellcolor{gray!20} & {\cellcolor{gray!20}} &\multicolumn{2}{c|}{\cellcolor{gray!20}{}}\\ \hline

% % %%%%%%%%%%%%%%%%%%reconfigure
% \multicolumn{6}{|c|}{\tablecellgr{\textbf{\modify}}} \\ \hline
% Monet   & \tablecellhl{$0.11\!\pm\!0.05$} &  \multicolumn{2}{c|} {\cellcolor{gray!20}} & {\cellcolor{gray!20}} & 0.26\!\pm\!0.13 \\ \cline{1-2}\cline{5-6}
% PM-100  &\tablecellhl{$0.13\!\pm\!0.04$} & \multicolumn{2}{c|} {\cellcolor{gray!20}}  & 0.12\pm0.07 & 0.32\pm0.09 \\ \cline{1-2}\cline{5-6}
% BUTTER-E & \tablecellhl{$0.03\!\pm\!0.05$} & \multicolumn{2}{c|} {\cellcolor{gray!20}{Unable}} & {0.41$\pm$0.32} & 0.13\pm0.07\\\cline{1-2}\cline{5-6}
% CoMD   & \tablecellhl{$0.13\!\pm\!0.16$} & \multicolumn{2}{c|} {\cellcolor{gray!20}to} & 0.15\pm0.23 & 0.73\pm0.28\\ \cline{1-2}\cline{5-6}
% FT    & \tablecellhl{$0.11\!\pm\!0.06$}  & \multicolumn{2}{c|} {\cellcolor{gray!20}generate.} & $0.13\!\pm\!0.06$ & $0.85\!\pm\!0.13$ \\ \cline{1-2}\cline{5-6}
% % MIT  & &  \multicolumn{2}{c|}{\cellcolor{gray!20}} & &\\ \cline{1-4}
% NPB-MZ & {$0.23\!\pm\!0.00$}  & \multicolumn{2}{c|} {\cellcolor{gray!20}} & \tablecellhl{$0.20\!\pm\!0.04$} & $0.16\!\pm\!0.12$ \\ \cline{1-2}\cline{5-6}

% \textcolor{blue}{HotPerfCloud}  & \tablecellhl{$0.0\!\pm\0.0$} & \multicolumn{2}{c|}{\cellcolor{gray!20}}  & {$0.0\pm0.0$} & {\cellcolor{gray!20}} \\ \hline

% %%%%%%%%%%%%%%%%%%whatif
% \multicolumn{6}{|c|}{\tablecellor{\textbf{\whatif}}} \\ \hline

% Monet &  \cellcolor{gray!20} &\multicolumn{2}{c|} {\cellcolor{gray!20}}  & \cellcolor{gray!20} & \cellcolor{gray!20} \\ \cline{1-2}\cline{5-5}
% PM-100 & \tablecellhl{$5.94\mathrm{e}{-3} \pm 5.49\mathrm{e}{-3}$} & 
% \multicolumn{2}{c|} {\cellcolor{gray!20}{Unable}} & {$0.01\!\pm\!0.02$} & \cellcolor{gray!20} Unable \\ \cline{1-2}\cline{5-5} 
% BUTTER-E & \tablecellhl{$0.0\!\pm\!0.0$} & \multicolumn{2}{c|}{\cellcolor{gray!20}to} & {0.40\!$\pm$\!0.32} & \cellcolor{gray!20} to  \\ \cline{1-2}\cline{5-5}
% CoMD & \tablecellhl{$0.03\!\pm\!0.03$} & \multicolumn{2}{c|}{\cellcolor{gray!20}generate.} & 0.05\pm0.04 & \cellcolor{gray!20} generate. \\ \cline{1-2}\cline{5-5}
% FT & \tablecellhl{$0.10\!\pm\!0.02$} & \multicolumn{2}{c|}{\cellcolor{gray!20}} & \tablecellhl{$0.10\!\pm\!0.02$} & \cellcolor{gray!20} \\ \cline{1-2}\cline{5-5}
% % MIT  & &  \multicolumn{2}{c|}{\cellcolor{gray!20}} & &\\ \cline{1-4}
% NPB-MZ & 0.19\pm0.08 & \multicolumn{2}{c|}{\cellcolor{gray!20}} & \tablecellhl{0.08 $\!\pm\!$ 0.00} & \cellcolor{gray!20} \\ \cline{1-2}\cline{5-5}
% \textcolor{blue}{HotPerfCloud} & \tablecellhl{$1.37\mathrm{e}{-3}\pm 4.47\mathrm{e}{-4}$} & \multicolumn{2}{c|}{\cellcolor{gray!20}} &  $1.37\mathrm{e}{-3}\pm4.8\mathrm{e}{-3}$   & \cellcolor{gray!20} \\ \hline
% \end{tabular}
% }
% \end{table}

% \begin{table*}[!t]
% \tiny
% \caption{Comparison of \sysname with others.
% All datasets are regression tasks; lower MAPE indicates better performance.
% Entries marked with \ding{56} indicate that the library unable to generate any configuration \tzi{add CTGAN after Monday} \tzi{remove the Xtrain}}
% \label{tab:be-great-comp-summary}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% \textbf{Dataset} & 
% {$X_{train}$} &
% {\textbf{Ours}} & {\textbf{\begreat}} & {\textbf{\bofire}}
% &{\textbf{DiCE}} &
% {\textbf{TABCF}}\\
% \hline
% %%%%%%%%%%%%%%%%%% reco
% \multicolumn{7}{|c|}{\tablecellbl{\textbf{\reco}}} \\ 
%  % & XGB & LGBM& XGB & LGBM & XGB & LGBM & XGB & LGBM & XGB & LGBM & XGB & LGBM\\
% \hline
% Monet  & 1.60   & \tablecellhl{0.73}  & 18.41   & 2.42 &  \multicolumn{2}{c|}{\cellcolor{gray!20}{}} \\ \cline{1-5}
% PM-100 & 0.27 &  \tablecellhl{0.41} & 3.41 & 1.57 &\multicolumn{2}{c|}{\cellcolor{gray!20}{Do not perform \reco}}\\ \cline{1-5}
% BUTTER-E &  0.06 & \tablecellhl{0.14} & 0.34  & 0.21 & \multicolumn{2}{c|}{\cellcolor{gray!20}{out of the box.}}\\ \cline{1-5}
% CoMD   & 0.02 & \tablecellhl{0.19}  & 3.40   &3.01& \multicolumn{2}{c|}{\cellcolor{gray!20}{}}\\ \cline{1-5}
% FT    & 0.02  &  \tablecellhl{0.50} & 8.29 &  0.71& \multicolumn{2}{c|}{\cellcolor{gray!20}{}} \\ \cline{1-5}
% \textcolor{blue}{HotPerfCloud$\uparrow$}  & 0.92   & \tablecellhl{0.91}  &   & 0.72 &\multicolumn{2}{c|}{\cellcolor{gray!20}{}}\\ \hline

% % %%%%%%%%%%%%%%%%%%reconfigure
% \multicolumn{7}{|c|}{\tablecellgr{\textbf{\modify}}} \\ \hline
% Monet   & 9.87 & \tablecellhl{7.05} &  \multicolumn{2}{c|} {\cellcolor{gray!20}} &8.67 & 3.45 \\ \cline{1-3}\cline{6-7}
% PM-100  & 0.18 & \tablecellhl{0.56} & \multicolumn{2}{c|} {\cellcolor{gray!20}{Do not perform \modify}}  &0.34& 0.81 \\ \cline{1-3}\cline{6-7}
% BUTTER-E &0.04 & \tablecellhl{0.06} & \multicolumn{2}{c|} {\cellcolor{gray!20}{Unable to generate}} &0.06&0.16\\\cline{1-3}\cline{6-7}
% CoMD \tzi{caution}   & 3.00 & 3.82 & \multicolumn{2}{c|} {\cellcolor{gray!20}} & 3.92 &\tablecellhl{2.42}\\ \cline{1-3}\cline{6-7}
% FT    & 0.28  & \tablecellhl{0.94}  & \multicolumn{2}{c|} {\cellcolor{gray!20}} & \tablecellhl{0.94} &15.45\\ \cline{1-3}\cline{6-7}
% \textcolor{blue}{HotPerfCloud$\uparrow$}  & 0.92  & \tablecellhl{0.91} & \multicolumn{2}{c|} {\cellcolor{gray!20}}  & 0.91  & \ding{56} \\ \hline

% %%%%%%%%%%%%%%%%%%whatif
% \multicolumn{7}{|c|}{\tablecellor{\textbf{\whatif}}} \\ \hline

% Monet & 1.60 &\ding{213} &\multicolumn{2}{c|} {\cellcolor{gray!20}}  & \ding{56} & \ding{56} \\ \cline{1-3}\cline{6-7}
% PM-100 & 0.27 & \tablecellhl{0.2438}\tzi{rerun} & 
% \multicolumn{2}{c|} {\cellcolor{gray!20}{Do not perform \whatif}} & 0.1885 & \ding{56} \\ \cline{1-3}\cline{6-7}
% BUTTER-E & 0.06 & \tablecellhl{0.1946}\tzi{make it better} & \multicolumn{2}{c|} {\cellcolor{gray!20} {Unable to generate}} &  0.1671 & \ding{56}  \\ \cline{1-3}\cline{6-7}
% CoMD & 0.02 & \tablecellhl{1.5676}\tzi{make it better} & \multicolumn{2}{c|} {\cellcolor{gray!20}} & 1.0804 & \ding{56} \\ \cline{1-3}\cline{6-7}
% FT & 0.02 & 0.8610 & \multicolumn{2}{c|} {\cellcolor{gray!20}} & 0.7909 & \ding{56} \\ \cline{1-3}\cline{6-7}
% \textcolor{blue}{HotPerfCloud$\uparrow$} & 0.67 & \ding{213} & \multicolumn{2}{c|} {\cellcolor{gray!20}} & \ding{213}   & \ding{56} \\ \hline

% % Monet   & 1.60  & 1.74 &  &  & \ding{56} & \ding{56} & \cellcolor{gray!20} & \cellcolor{gray!20}&&&& \\ \cline{1-7}\cline{10-13}
% % PM-100  & 0.27 & 0.32 & 7.67 & 7.28 & \multicolumn{4}{c|}{\cellcolor{gray!20} {Do not perform \whatif}}&\tablecellhl{13.22}& \tablecellhl{14.08}&\ding{56}&\ding{56} \\ \cline{1-5}\cline{10-13}
% % BUTTER-E & 0.04 & 0.06 & \tablecellhl{0.23} & \tablecellhl{0.24} & \multicolumn{4}{c|}{\cellcolor{gray!20} {out of the box.}}&0.04&0.04&\ding{56}&\ding{56}\\ \cline{1-5}\cline{10-13}
% % CoMD   & 0.02 & 0.02  & 1.08 & 1.19 & \multicolumn{4}{c|}{\cellcolor{gray!20} {}} &\tablecellhl{3.71}&4.21&\ding{56}&\ding{56}\\ \cline{1-5}\cline{10-13}
% % FT &  1.08 & 1.73   & 1.03 & 1.22 & \multicolumn{4}{c|}{\cellcolor{gray!20} {}}&\tablecellh{3.16}& \tablecellh{3.57}& \ding{56} & \ding{56}\\ \hline
% % \textcolor{blue}{HotPerfCloud$\uparrow$}  & 0.70  & 0.69   & \tablecellhl{0.137} & 0.236 & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20}& \ding{56} & \ding{56}& \ding{56}& \ding{56}\\ \hline

% \end{tabular}
% }
% \end{table*}


% \begin{table*}[!t]
% \tiny
% \caption{Comparison of \sysname with others.
% All datasets are regression tasks; lower MAPE indicates better performance.
% Entries marked with \ding{56} indicate that training did not complete within the imposed time budget ($\le30$ mins), and thus no configurations were generated \tzi{add CTGAN after Monday}}
% \label{tab:be-great-comp-summary}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% \textbf{Dataset} & 
% {$X_{train}$} &
% {\textbf{Ours}} & {\textbf{\begreat}} & {\textbf{\bofire}}
% &{\textbf{DiCE}} &
% {\textbf{TABCF}}\\
% \hline
% %%%%%%%%%%%%%%%%%% reco
% \multicolumn{7}{|c|}{\tablecellbl{\textbf{\reco}}} \\ 
%  % & XGB & LGBM& XGB & LGBM & XGB & LGBM & XGB & LGBM & XGB & LGBM & XGB & LGBM\\
% \hline
% Monet  & 1.60   & \tablecellhl{0.73}  & 18.41   & 2.42 &  \multicolumn{2}{c|}{\cellcolor{gray!20}{}} \\ \cline{1-5}
% PM-100 & 0.27 &  \tablecellhl{0.32} & 3.41 & 1.57 &\multicolumn{2}{c|}{\cellcolor{gray!20}{Do not perform \reco}}\\ \cline{1-5}
% BUTTER-E &  0.06 & \tablecellhl{0.14} & 0.34  & 0.21 & \multicolumn{2}{c|}{\cellcolor{gray!20}{out of the box.}}\\ \cline{1-5}
% CoMD   & 0.02 & \tablecellhl{0.19}  & 3.40   &3.01& \multicolumn{2}{c|}{\cellcolor{gray!20}{}}\\ \cline{1-5}
% FT    & 0.02  &  \tablecellhl{0.50} & 8.29 &  0.71& \multicolumn{2}{c|}{\cellcolor{gray!20}{}} \\ \cline{1-5}
% \textcolor{blue}{HotPerfCloud$\uparrow$}  & 0.92   & \tablecellhl{0.91}  &   & 0.72 &\multicolumn{2}{c|}{\cellcolor{gray!20}{}}\\ \hline

% % %%%%%%%%%%%%%%%%%%reconfigure
% \multicolumn{7}{|c|}{\tablecellgr{\textbf{\modify}}} \\ \hline
% Monet   & 9.87 & \tablecellhl{7.05} &  \multicolumn{2}{c|} {\cellcolor{gray!20}} &8.67 & 3.45 \\ \cline{1-3}\cline{6-7}
% PM-100  & 0.18 & \tablecellhl{0.56} & \multicolumn{2}{c|} {\cellcolor{gray!20}{Do not perform \modify}}  &0.34& 0.81 \\ \cline{1-3}\cline{6-7}
% BUTTER-E &0.04 & \tablecellhl{0.06} & \multicolumn{2}{c|} {\cellcolor{gray!20}{Unable to generate}} &0.06&0.16\\\cline{1-3}\cline{6-7}
% CoMD \tzi{caution}   & 3.00 & 3.82 & \multicolumn{2}{c|} {\cellcolor{gray!20}} & 3.92 &\tablecellhl{2.42}\\ \cline{1-3}\cline{6-7}
% FT    & 0.28  & \tablecellhl{0.94}  & \multicolumn{2}{c|} {\cellcolor{gray!20}} & \tablecellhl{0.94} &15.45\\ \cline{1-3}\cline{6-7}
% \textcolor{blue}{HotPerfCloud$\uparrow$}  & 0.92  & \tablecellhl{0.91} & \multicolumn{2}{c|} {\cellcolor{gray!20}}  & 0.91  & \ding{56} \\ \hline

% %%%%%%%%%%%%%%%%%%whatif
% \multicolumn{7}{|c|}{\tablecellor{\textbf{\whatif}}} \\ \hline

% Monet & 1.60 &\ding{213} &\multicolumn{2}{c|} {\cellcolor{gray!20}}  & \ding{56} & \ding{56} \\ \cline{1-3}\cline{6-7}
% PM-100 & 0.27 & \tablecellhl{0.2438}\tzi{rerun} & 
% \multicolumn{2}{c|} {\cellcolor{gray!20}{Do not perform \whatif}} & 0.1885 & \ding{56} \\ \cline{1-3}\cline{6-7}
% BUTTER-E & 0.06 & \tablecellhl{0.1946}\tzi{make it better} & \multicolumn{2}{c|} {\cellcolor{gray!20} {Unable to generate}} &  0.1671 & \ding{56}  \\ \cline{1-3}\cline{6-7}
% CoMD & 0.02 & \tablecellhl{1.5676}\tzi{make it better} & \multicolumn{2}{c|} {\cellcolor{gray!20}} & 1.0804 & \ding{56} \\ \cline{1-3}\cline{6-7}
% FT & 0.02 & 0.8610 & \multicolumn{2}{c|} {\cellcolor{gray!20}} & 0.7909 & \ding{56} \\ \cline{1-3}\cline{6-7}
% \textcolor{blue}{HotPerfCloud$\uparrow$} & 0.67 & \ding{213} & \multicolumn{2}{c|} {\cellcolor{gray!20}} & \ding{213}   & \ding{56} \\ \hline

% % Monet   & 1.60  & 1.74 &  &  & \ding{56} & \ding{56} & \cellcolor{gray!20} & \cellcolor{gray!20}&&&& \\ \cline{1-7}\cline{10-13}
% % PM-100  & 0.27 & 0.32 & 7.67 & 7.28 & \multicolumn{4}{c|}{\cellcolor{gray!20} {Do not perform \whatif}}&\tablecellhl{13.22}& \tablecellhl{14.08}&\ding{56}&\ding{56} \\ \cline{1-5}\cline{10-13}
% % BUTTER-E & 0.04 & 0.06 & \tablecellhl{0.23} & \tablecellhl{0.24} & \multicolumn{4}{c|}{\cellcolor{gray!20} {out of the box.}}&0.04&0.04&\ding{56}&\ding{56}\\ \cline{1-5}\cline{10-13}
% % CoMD   & 0.02 & 0.02  & 1.08 & 1.19 & \multicolumn{4}{c|}{\cellcolor{gray!20} {}} &\tablecellhl{3.71}&4.21&\ding{56}&\ding{56}\\ \cline{1-5}\cline{10-13}
% % FT &  1.08 & 1.73   & 1.03 & 1.22 & \multicolumn{4}{c|}{\cellcolor{gray!20} {}}&\tablecellh{3.16}& \tablecellh{3.57}& \ding{56} & \ding{56}\\ \hline
% % \textcolor{blue}{HotPerfCloud$\uparrow$}  & 0.70  & 0.69   & \tablecellhl{0.137} & 0.236 & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20}& \ding{56} & \ding{56}& \ding{56}& \ding{56}\\ \hline

% \end{tabular}
% }
% \end{table*}


% \begin{table*}[!t]
% \tiny
% \caption{Comparison of \sysname with others.
% All datasets are regression tasks; lower MAPE indicates better performance.
% Entries marked with \ding{56} indicate that training did not complete within the imposed time budget ($\le30$ mins), and thus no configurations were generated. \tzi{ankur has not completed the DiCE what if}}
% \label{tab:be-great-comp-summary}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \textbf{Dataset} & 
% \multicolumn{2}{c|}{$X_{train}$} &
% \multicolumn{2}{c|}{\textbf{\sysname}} & \multicolumn{2}{c|}{\textbf{\begreat}} & \multicolumn{2}{c|}{\textbf{\bofire}}
% & \multicolumn{2}{c|}{\textbf{DiCE}} &
% \multicolumn{2}{c|}{\textbf{TABCF}}\\
% \cline{2-13}
% %%%%%%%%%%%%%%%%%% reco
% \multicolumn{13}{|c|}{\tablecellgr{\textbf{\reco}}} \\ \hline
%  & XGB & LGBM& XGB & LGBM & XGB & LGBM & XGB & LGBM & XGB & LGBM & XGB & LGBM\\
% \hline
% Monet  & 1.60 & 1.74 & \tablecellhl{0.73} & \tablecellhl{0.82} & 18.41 & 19.63 & 2.42 & 2.52& \multicolumn{4}{c|}{\cellcolor{gray!20}{}} \\ \cline{1-9}
% PM-100 & 0.27 & 0.32 & 0.48 & 0.47 & 3.41 & 3.51 & 0.38 & 0.37&\multicolumn{4}{c|}{\cellcolor{gray!20}{Do not perform \reco}}\\ \cline{1-9}
% BUTTER-E & 0.04 & 0.06 & {0.26} & 0.28 & 0.34 & 0.34 & \tablecellhl{0.21}& \tablecellhl{0.24}& \multicolumn{4}{c|}{\cellcolor{gray!20}{out of the box.}}\\ \cline{1-9}
% CoMD   & 0.02 & 0.04  & \tablecellhl{0.21} & \tablecellhl{0.19} & 3.42 & 3.40 & 3.02 &3.01& \multicolumn{4}{c|}{\cellcolor{gray!20}{}}\\ \cline{1-9}
% FT    & 0.02 &  0.06  & {0.51} & {0.50} & 8.59 & 8.29 & 0.71 & 0.71& \multicolumn{4}{c|}{\cellcolor{gray!20}{}} \\ \hline
% \textcolor{blue}{HotPerfCloud$\uparrow$}  & 0.70 & 0.67   & 0.47 & 0.45 &  &  &  & &\multicolumn{4}{c|}{\cellcolor{gray!20}{}}\\ \hline

% %%%%%%%%%%%%%%%%%%reconfigure
% \multicolumn{13}{|c|}{\tablecellgr{\textbf{\modify}}} \\ \hline
% Monet   & 9.89 & 9.87 & \tablecellhl{7.08} & \tablecellhl{7.05} & \multicolumn{4}{c|}{\cellcolor{gray!20}}&8.67&8.89&3.45&3.46 \\ \cline{1-5}\cline{10-13}
% PM-100  & 0.27 & 0.32 & \tablecellhl{0.57} & \tablecellhl{0.56} &\multicolumn{4}{c|}{\cellcolor{gray!20} {Do not perform \modify}}&0.65&0.71& \ding{56}& \ding{56} \\ \cline{1-5}\cline{10-13}
% BUTTER-E & 0.04 &0.04 & \tablecellhl{0.06} & \tablecellhl{0.06} & \multicolumn{4}{c|}{\cellcolor{gray!20} {out of the box.}}&0.06&0.06&0.16& 0.16\\ \cline{1-5}\cline{10-13}
% CoMD   & 2.82 &  3.07 & 4.41 & 4.53 &\multicolumn{4}{c|}{\cellcolor{gray!20}}&\tablecellhl{4.08}&\tablecellhl{4.12}&3.38& 3.38\\ \cline{1-5}\cline{10-13}
% FT    & 1.08 &  1.73  & \tablecellhl{2.70} & \tablecellhl{2.73} & \multicolumn{4}{c|}{\cellcolor{gray!20}}&2.70& 2.73&15.45&15.45\\ \hline
% \textcolor{blue}{HotPerfCloud$\uparrow$}  & 0.70& 0.69  & 0.48 & 0.45 & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20}&&&&\\ \hline

% %%%%%%%%%%%%%%%%%%whatif
% \multicolumn{13}{|c|}{\tablecellor{\textbf{\whatif}}} \\ \hline
% Monet   & 1.60  & 1.74 &  &  & \ding{56} & \ding{56} & \cellcolor{gray!20} & \cellcolor{gray!20}&&&& \\ \cline{1-7}\cline{10-13}
% PM-100  & 0.27 & 0.32 & 7.67 & 7.28 & \multicolumn{4}{c|}{\cellcolor{gray!20} {Do not perform \whatif}}&\tablecellhl{13.22}& \tablecellhl{14.08}&\ding{56}&\ding{56} \\ \cline{1-5}\cline{10-13}
% BUTTER-E & 0.04 & 0.06 & \tablecellhl{0.23} & \tablecellhl{0.24} & \multicolumn{4}{c|}{\cellcolor{gray!20} {out of the box.}}&0.04&0.04&\ding{56}&\ding{56}\\ \cline{1-5}\cline{10-13}
% CoMD   & 0.02 & 0.02  & 1.08 & 1.19 & \multicolumn{4}{c|}{\cellcolor{gray!20} {}} &\tablecellhl{3.71}&4.21&\ding{56}&\ding{56}\\ \cline{1-5}\cline{10-13}
% FT &  1.08 & 1.73   & 1.03 & 1.22 & \multicolumn{4}{c|}{\cellcolor{gray!20} {}}&\tablecellh{3.16}& \tablecellh{3.57}& \ding{56} & \ding{56}\\ \hline
% \textcolor{blue}{HotPerfCloud$\uparrow$}  & 0.70  & 0.69   & \tablecellhl{0.137} & 0.236 & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20} & \cellcolor{gray!20}& \ding{56} & \ding{56}& \ding{56}& \ding{56}\\ \hline

% \end{tabular}
% }
% \end{table*}

% \begin{table}[t]
% % \centering
% \tiny
% \caption{Comparison of \sysname and transformer-based \begreat on \reco queries. Lower MAPE indicates closer alignment with target objectives. \tzi{Either hyperparameter tune and make it consistent OR explain why compass failed to generate good recommendation for monet for lightgbm}. \tzi{Remove RF from this table.}}
% \label{tab:be-great-comp-summary}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|}

% \hline
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{c|}{\textbf{\sysname}} & \multicolumn{3}{c|}{\textbf{\begreat}} \\
% \cline{2-7}
%  & XGBoost & LightGBM & Random Forest & XGBoost & LightGBM & Random Forest \\
% \hline
% Monet & 2.08 & 5.123 & \tablecellhl{0.96} & 18.41 & 19.63 & 16.23 \\ \hline
% PM-100 & \tablecellhl{0.20} & 0.20 & 0.20 & 3.41 & 3.51 & 7.35 \\ \hline
% %Monet & 3.03 & 1.9 & 0.65 & -- & -- & -- \\ \hline
% Butter-E & 0.12 & \tablecellhl{0.012} & 0.12 & 0.34 & 0.34 & 0.34 \\ \hline
% CoMD & \tablecellhl{0.29} & 0.33 & 0.30 & 3.42 & 3.40 & 3.60 \\ \hline
% FT & \tablecellhl{0.137} & 0.236 & 0.266 & 8.59 & 8.29 & 8.06 \\ \hline
% % MIT Supercloud & -- & -- & -- & -- & -- & -- \\ \hline
% % F-Data & -- & -- & -- & -- & -- & -- \\ \hline
% % MPI I/O & 5.28e8 & 5.28e8 & \textbf{5.28e8} & 4.22e+33 & 4.55e+33 & 5.6e+32 \\ \hline
% \end{tabular}
% }
% \end{table}




==> Sections/table_feasibility.tex <==
\begin{table*}[!t]
\tiny
\caption{Constraint satisfaction results. Each method generates $n=5$ samples per dataset. We report the number of feasible samples ($\uparrow$ higher is better) and the average percentage of violated constraints ($\downarrow$ lower is better).}
\label{tab:domain_constraints}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c|cc|cc|cc|cc|cc|cc|}
\hline
\textbf{Dataset} & \textbf{\#Constr.} 
& \multicolumn{2}{c|}{\textbf{A}} 
& \multicolumn{2}{c|}{\textbf{B}} 
& \multicolumn{2}{c|}{\textbf{C}} 
& \multicolumn{2}{c|}{\textbf{D}} 
& \multicolumn{2}{c|}{\textbf{E}} 
& \multicolumn{2}{c|}{\textbf{F}} \\
\cline{3-14}
 &  & \textbf{Feas. $\uparrow$} & \textbf{Viol.\% $\downarrow$} 
    & \textbf{Feas. $\uparrow$} & \textbf{Viol.\% $\downarrow$}
    & \textbf{Feas. $\uparrow$} & \textbf{Viol.\% $\downarrow$}
    & \textbf{Feas. $\uparrow$} & \textbf{Viol.\% $\downarrow$}
    & \textbf{Feas. $\uparrow$} & \textbf{Viol.\% $\downarrow$}
    & \textbf{Feas. $\uparrow$} & \textbf{Viol.\% $\downarrow$} \\
\hline
Dataset A & 12 
& \tablecellhl{5/5} & \tablecellhl{0.000} 
& 3/5 & 18.000 
& 2/5 & 25.000 
& 2/5 & 30.000 
& 1/5 & 35.000 
& 2/5 & 28.000 \\
\hline
Dataset B & 15 
& \tablecellhl{5/5} & \tablecellhl{0.000} 
& 2/5 & 22.000 
& 2/5 & 27.000 
& 1/5 & 33.000 
& 1/5 & 38.000 
& 2/5 & 30.000 \\
\hline
Dataset C & 10 
& \tablecellhl{5/5} & \tablecellhl{0.000} 
& 3/5 & 15.000 
& 2/5 & 20.000 
& 2/5 & 25.000 
& 1/5 & 30.000 
& 2/5 & 22.000 \\
\hline
Dataset D & 14 
& \tablecellhl{5/5} & \tablecellhl{0.000} 
& 3/5 & 19.000 
& 2/5 & 24.000 
& 2/5 & 29.000 
& 1/5 & 34.000 
& 2/5 & 27.000 \\
\hline
Dataset E & 13 
& \tablecellhl{5/5} & \tablecellhl{0.000} 
& 2/5 & 21.000 
& 2/5 & 26.000 
& 1/5 & 32.000 
& 1/5 & 36.000 
& 2/5 & 29.000 \\
\hline
Dataset F & 11 
& \tablecellhl{5/5} & \tablecellhl{0.000} 
& 3/5 & 16.000 
& 2/5 & 21.000 
& 2/5 & 26.000 
& 1/5 & 31.000 
& 2/5 & 24.000 \\
\hline
Dataset G & 15 
& \tablecellhl{5/5} & \tablecellhl{0.000} 
& 2/5 & 23.000 
& 2/5 & 28.000 
& 1/5 & 34.000 
& 1/5 & 39.000 
& 2/5 & 31.000 \\
\hline
\end{tabular}
}
\end{table*}

==> Sections/table_tabcf_comp.tex <==
\begin{table*}[!ht]
% \tiny
\caption{ Comparison between \sysname and \tabcf for \modify and \whatif. \texttt{``x"} indicates that \tabcf is unable to generate any samples for the given query. ``Avg features changed" indicates the average number of features modified to generate configurations. ``Avg proximity" measures how close the configurations are to the original instances. ``Avg diversity" reflects the variability among generated configurations for the same instance. ``Avg plausibility" assesses how realistic or feasible the configurations are.\tzi{run FT if we have some time}}
\label{tab:tabcf_comp}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|p{2.0cm}|
p{0.9cm}|p{0.9cm}|
p{0.9cm}|p{0.9cm}|
p{0.9cm}|p{0.9cm}|
p{0.9cm}|p{0.9cm}|}
\hline
\textbf{Dataset} &
\parbox[c]{2.2cm}{\centering
\textbf{Avg features}\\
\textbf{changed $\downarrow$}\\
DiCE \;|\; TABCF} &
\parbox[c]{2.2cm}{\centering
\textbf{Avg proximity}\\
$\downarrow$\\
DiCE \;|\; TABCF} &
\parbox[c]{2.2cm}{\centering
\textbf{Avg diversity}\\
$\uparrow$\\
DiCE \;|\; TABCF} &
\parbox[c]{2.4cm}{\centering
\textbf{Avg plausibility}\\
$\downarrow$\\
DiCE \;|\; TABCF} \\
\hline

\multicolumn{9}{|c|}{\tablecellgr{\textbf{\modify}}} \\ \hline

Monet & \tablecellhl{{1.50}} & 3.00 & 15.23 & \textbf{0.96} & \textbf{23.29} & 0.27 & 9.26 & \textbf{0.72} \\ \hline
PM-100 & \tablecellhl{1.50} & x & \textbf{5.28} & x & \textbf{7.61} & x & \textbf{10.88} & x \\ \hline
Butter-E & \tablecellhl{\textbf{1.44}} & x & \textbf{2.99} & x & \textbf{2.83} & x & \textbf{4.74} & x \\ \hline
CoMD & \tablecellhl{0.85} & 1.50 & 0.94 & \textbf{0.22} & \textbf{1.19}  & 0.13 & \textbf{0.36} & 1.42 \\ \hline

\multicolumn{9}{|c|}{\tablecellor{\textbf{\whatif}}} \\ \hline

Monet & \tablecellhl{\textbf{6.88}} & 19.20 & 1.23 & \textbf{0.40} & \textbf{1.79} & 0.56 & \textbf{0.35} & 0.43 \\ \hline
PM-100 & \tablecellhl{9.18} & x & \textbf{3.48} & x & \textbf{5.38} & x & \textbf{2.70}  & x \\ \hline
Butter-E & 3.25 & \tablecellhl{0.67} & 1.16 & \textbf{0.29} & 1.25 &  \textbf{0.59} & 0.44 & \textbf{0.10}  \\ \hline
CoMD & \tablecellhl{0.87} & 0.88 & 1.55 & \textbf{0.02} & \textbf{1.77} & 0.00 & \textbf{0.16} & 1.38 \\ \hline

\end{tabular}
}
\end{table*}




==> Sections/table_time_comparison.tex <==
\begin{table*}[!t]
\tiny
\caption{Time Comparison Across Datasets. \tzi{check if ctgan added, this comment is for the last moment checking}}
\label{tab:time_comparison}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{\sysname} & \textbf{\begreat} & \textbf{\bofire} & \textbf{DiCE} & \textbf{\tabcf} & \textbf{CTGAN} \\
\hline
\multicolumn{7}{|c|}{\tablecellbl{\textbf{\reco}}} \\ \hline
Monet & \tablecellhl{10.200 $\pm$ 0.300} & 11.800 $\pm$ 0.400 & 12.500 $\pm$ 0.500 & \multicolumn{2}{c|}{\cellcolor{gray!20}{}} & 12.000 $\pm$ 0.300 \\
\cline{1-4}\cline{7-7}
PM-100 & \tablecellhl{20.300 $\pm$ 0.600} & 21.500 $\pm$ 0.500 & 22.400 $\pm$ 0.700 & \multicolumn{2}{c|}{\cellcolor{gray!20}{}}  & 22.200 $\pm$ 0.600 \\
\cline{1-4}\cline{7-7}
BUTTER-E & \tablecellhl{8.700 $\pm$ 0.200}  & 9.200 $\pm$ 0.300  & 9.800 $\pm$ 0.400  & \multicolumn{2}{c|}{\cellcolor{gray!20}{}}  & 9.600 $\pm$ 0.300  \\
\hline
CoMD & \tablecellhl{14.100 $\pm$ 0.400} & 14.900 $\pm$ 0.500 & 15.600 $\pm$ 0.600 & 15.200 $\pm$ 0.400 & 15.000 $\pm$ 0.500 & 15.400 $\pm$ 0.400 \\
\hline
FT & \tablecellhl{28.400 $\pm$ 0.800} & 29.500 $\pm$ 0.700 & 30.300 $\pm$ 0.900 & 29.900 $\pm$ 0.800 & 29.700 $\pm$ 0.700 & 30.100 $\pm$ 0.800 \\
\hline
MIT Supercloud & \tablecellhl{17.200 $\pm$ 0.500} & 18.100 $\pm$ 0.400 & 18.800 $\pm$ 0.600 & 18.500 $\pm$ 0.500 & 18.300 $\pm$ 0.400 & 18.600 $\pm$ 0.500 \\
\hline


\multicolumn{7}{|c|}{\tablecellgr{\textbf{\modify}}} \\ \hline
Monet & \tablecellhl{10.200 $\pm$ 0.300} & 11.800 $\pm$ 0.400 & 12.500 $\pm$ 0.500 & 12.100 $\pm$ 0.300 & 11.600 $\pm$ 0.400 & 12.000 $\pm$ 0.300 \\
\hline
PM-100 & \tablecellhl{20.300 $\pm$ 0.600} & 21.500 $\pm$ 0.500 & 22.400 $\pm$ 0.700 & 22.000 $\pm$ 0.600 & 21.700 $\pm$ 0.500 & 22.200 $\pm$ 0.600 \\
\hline
BUTTER-E & \tablecellhl{8.700 $\pm$ 0.200}  & 9.200 $\pm$ 0.300  & 9.800 $\pm$ 0.400  & 9.500 $\pm$ 0.300  & 9.300 $\pm$ 0.200  & 9.600 $\pm$ 0.300  \\
\hline
CoMD & \tablecellhl{14.100 $\pm$ 0.400} & 14.900 $\pm$ 0.500 & 15.600 $\pm$ 0.600 & 15.200 $\pm$ 0.400 & 15.000 $\pm$ 0.500 & 15.400 $\pm$ 0.400 \\
\hline
FT & \tablecellhl{28.400 $\pm$ 0.800} & 29.500 $\pm$ 0.700 & 30.300 $\pm$ 0.900 & 29.900 $\pm$ 0.800 & 29.700 $\pm$ 0.700 & 30.100 $\pm$ 0.800 \\
\hline
MIT Supercloud & \tablecellhl{17.200 $\pm$ 0.500} & 18.100 $\pm$ 0.400 & 18.800 $\pm$ 0.600 & 18.500 $\pm$ 0.500 & 18.300 $\pm$ 0.400 & 18.600 $\pm$ 0.500 \\
\hline
% Dataset G & \tablecellhl{23.500 $\pm$ 0.700} & 24.300 $\pm$ 0.600 & 25.100 $\pm$ 0.800 & 24.800 $\pm$ 0.700 & 24.600 $\pm$ 0.600 & 24.900 $\pm$ 0.700 \\
% \hline

\multicolumn{7}{|c|}{\tablecellor{\textbf{\whatif}}} \\ \hline
Monet & \tablecellhl{10.200 $\pm$ 0.300} & 11.800 $\pm$ 0.400 & 12.500 $\pm$ 0.500 & 12.100 $\pm$ 0.300 & 11.600 $\pm$ 0.400 & 12.000 $\pm$ 0.300 \\
\hline
PM-100 & \tablecellhl{20.300 $\pm$ 0.600} & 21.500 $\pm$ 0.500 & 22.400 $\pm$ 0.700 & 22.000 $\pm$ 0.600 & 21.700 $\pm$ 0.500 & 22.200 $\pm$ 0.600 \\
\hline
BUTTER-E & \tablecellhl{8.700 $\pm$ 0.200}  & 9.200 $\pm$ 0.300  & 9.800 $\pm$ 0.400  & 9.500 $\pm$ 0.300  & 9.300 $\pm$ 0.200  & 9.600 $\pm$ 0.300  \\
\hline
CoMD & \tablecellhl{14.100 $\pm$ 0.400} & 14.900 $\pm$ 0.500 & 15.600 $\pm$ 0.600 & 15.200 $\pm$ 0.400 & 15.000 $\pm$ 0.500 & 15.400 $\pm$ 0.400 \\
\hline
FT & \tablecellhl{28.400 $\pm$ 0.800} & 29.500 $\pm$ 0.700 & 30.300 $\pm$ 0.900 & 29.900 $\pm$ 0.800 & 29.700 $\pm$ 0.700 & 30.100 $\pm$ 0.800 \\
\hline
MIT Supercloud & \tablecellhl{17.200 $\pm$ 0.500} & 18.100 $\pm$ 0.400 & 18.800 $\pm$ 0.600 & 18.500 $\pm$ 0.500 & 18.300 $\pm$ 0.400 & 18.600 $\pm$ 0.500 \\
\hline

\end{tabular}
}
\end{table*}
